The Gateaux Derivative of Map over Division Ring

I consider differential of mapping $f$ of continuous division ring as linear mapping the most close to mapping $f$. Different expressions which correspond to known deffinition of derivative are supplementary. I explore the Gateaux derivative of higher order and Taylor series. The Taylor series allow solving of simple differential equations. As an example of solution of differential equation I considered a model of exponent. I considered application of obtained theorems to complex field and quaternion algebra. In contrast to complex field in quaternion algebra congugation is linear function of original number \bar a=a+iai+jaj+kak . In quaternion algebra this difference leads to the absence of analogue of the Cauchy Riemann equations that are well known in the theory of complex function.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{texSpaceTime}{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
}%

\BiblioItem{texSpaceTime}{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{texSpaceTime}{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{texSpaceTime}{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{texSpaceTime}{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{texSpaceTime}{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{texSpaceTime}{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{texSpaceTime}{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{texSpaceTime}{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{texGenRelativity}{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{texGenRelativity}{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{texAffine,texGeomObject}{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{texAffine}{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{texAffine}{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{texAffine}{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{texAffine}{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{texTidal,texAffine,texGeomObject}{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{texTidal,texNewton}{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{texNewton}{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{texNewton}{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{texLagrange}{Weinberg}
{
Steven Weinberg. The Quantum Theory of Fields. Cambridge university press.
}%

\BiblioItem{texLagrange}{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{texLagrange}{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{texTidal}{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{texPrefaceTidal,texPrefaceRefernceFrame}{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{texTidal}{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{texDifferential,texReferenceFrame,texFiberedAlgebra,texVocab,texAdditiveMap,texDivisionRing}
{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{texFiberedAlgebra,texTstarMorphism}{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{texGeomObject}{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{texBundle}{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин,
Элементы теории функций и функционального анализа,
М., Наука, 1976
}%

\BiblioItem{}{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem{texAffine,texRepresentation,texTstarRepresentation,texRingAdditiveMap,texPolyvector,texAffineSpace}
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem{texBiadditiveMap}
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem{texPolyvector}{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{texDrcBasis,texBasis}{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{texBundle}{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{texPrefaceRefernceFrame}{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{texPrefaceRefernceFrame}{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{texPrefaceRefernceFrame}{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{texPrefaceRefernceFrame}{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{texPrefaceRefernceFrame}{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{texPrefaceRefernceFrame}{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texPrefaceRefernceFrame}{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texPrefaceRefernceFrame,texPrefaceTidal}{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{texBiring,texVectorSpace}{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{texBiring,texVectorSpace}
{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{texVectorSpace}{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{texVectorSpace}{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

%\BiblioItem{texVectorSpace}{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{texVectorSpace}{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\ifx\PrintBook\Defined
\else
\BiblioItem{texDrcReferenceFrame,texRefernceFrame,texLie,texLieRepresentation}{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2004)
}%
\fi

\BiblioItem{}{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2004)
}%

\BiblioItem{}{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2004)
}%

\BiblioItem{texFiberedAlgebra,texBundleRelation,texDrcLie}{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2007)
}%

\BiblioItem{texBundleRelation,texPrefaceRelation,IntroCalculusBook}{0702.561}
{
Александр Клейн,
Расслоенная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

%\BiblioItem{texBasis,texLinearMap}{math.RA-0501237}
%{
%Александр Клейн,
%Векторное пространство над телом,\\
%eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2005)
%}%

\BiblioItem{texPolymodule}{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\ifx\texBiring\Defined
\else
\BiblioItem{texVectorSpace,texFiberedAlgebra}{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2006)
}%
\fi

\ifx\texBundleRelation\Defined
\else
\BiblioItem{texFiberedMorphism}{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%
\fi

\ifx\PrintBook\Defined
\BiblioItem{texPrefaceRelation}{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%
\fi

\BiblioItem{texLie}{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2008)
}%

\BiblioItem{EprintCalculus}{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2008)
}%

\BiblioItem{texHomotopy,texTowerRepresentation,texPrefaceIntroGeometry}{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{texPrefaceRelation}{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem{texBundleRelation,texPrefaceRelation,texTstarMorphism,texBundle}
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem{texBundle}
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{texFiberedAlgebra}{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{texBundleRelation}{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{texBundle,texCartesian,texFiberedAlgebra,texBundleRelation,texFiberedMorphism}
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{texDifferential,texSecondDifferential}{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{texSecondDifferential}{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{texDifferential}{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem{texVocab,texDiffEq,texDrcDiffEq,texPrefaceLie}
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М. Иностранная литература, 1947
}

\BiblioItem{texVocab}
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{texFiberedMorphism}{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{texSecondDifferential,texDifferential}{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{texFiberedAlgebra,texFiberedMorphism}{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{texFiberedMorphism}{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{texFiberedMorphism}{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{texPolyvector}{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{texQuaternion}{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{texAffineSpace}{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{texPrefaceIntroCalculus}{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\CloseBiblio



==> Convention.Russian.tex <==
%auto-ignore

\section{Соглашения}

\begin{enumerate}

\item Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции.
%Однако мы можем рассматривать свободную
%алгебру как векторное пространство над полем.
%Так как нежелательно одно и тоже соответствие называть то функцией, то
%отображением, я буду пользоваться термином линейная функция алгебры.

\item
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
При этом подразумевается, что отображение мультипликативно над
максимально возможным полем. В частности, линейное отображение
тела $D$ мультипликативно над центром $Z(D)$. Это не противоречит
определению линейного отображения поля, так как для поля $F$ справедливо
$Z(F)=F$.
Если поле $F$ отлично
от максимально возможного, то я это явно указываю в тексте.

\item
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
Запись \Ds линейно зависимые векторы можно прочесть
как D\Hyph star\Hyph линейно зависимые векторы либо
как векторы, линейно зависимые слева.

\end{enumerate}



==> Differential.Russian.tex <==
%auto-ignore
\def\texDifferential{}

\input{Differential.Eq}

\ifx\PrintBook\undefined
\else
	\chapter{Дифференцируемые отображения}
	\label{chapter: Differentiable maps}
\fi
\section{Топологическое тело}
\label{section: Topological Division Ring}

\begin{definition}
Тело $D$ называется 
\AddIndex{топологическим телом}{topological division ring}\footnote{Определение
дано согласно
определению из \citeBib{Pontryagin: Topological Group},
глава 4},
если $D$ является топологическим пространством, и алгебраические операции,
определённые в $D$, непрерывны в топологическом пространстве $D$.
\qed
\end{definition}

Согласно определению, для произвольных элементов $a, b\in D$
и для произвольных окрестностей $W_{a-b}$ элемента $a-b$,
$W_{ab}$ элемента $ab$ существуют такие окрестности $W_a$
элемента $a$ и $W_b$ элемента $b$, что $W_a-W_b\subset W_{a-b}$,
$W_aW_b\subset W_{ab}$. Если $a\ne 0$, то для произвольной
окрестности $W_{a^{-1}}$ существует окрестность $W_a$ элемента $a$,
удовлетворяющая условию $W_a^{-1}\subset W_{a^{-1}}$.

\begin{definition}
\label{definition: absolute value on division ring}
\AddIndex{Норма на теле}
{absolute value on division ring} $D$\footnote{Определение
дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2} - это отображение
\[d\in D\rightarrow |d|\in R\]
такое, что
\begin{itemize}
\item $|a|\ge 0$
\item $|a|=0$ равносильно $a=0$
\item $|ab|=|a|\ |b|$
\item $|a+b|\le|a|+|b|$
\end{itemize}

Тело $D$, наделённое структурой, определяемой заданием на
$D$ нормы, называется \AddIndex{нормированным телом}{valued division ring}.
\qed
\end{definition}

Инвариантное расстояние на аддитивной группе тела $D$
\[d(a,b)=|a-b|\]
определяет топологию метрического пространства,
согласующуюся со структурой тела в $D$.

\begin{definition}
\label{definition: limit of sequence, valued division ring}
Пусть $D$ - нормированное тело.
Элемент $a\in D$ называется 
\AddIndex{пределом последовательности}{limit of sequence, valued division ring}
$\{a_n\}$
\symb{\lim_{n\rightarrow\infty}a_n}0{limit of sequence, valued division ring}
\[
a=\ShowSymbol{limit of sequence, valued division ring}
\]
если для любого $\epsilon\in R$, $\epsilon>0$
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое,
что $|a_n-a|<\epsilon$ для любого $n>n_0$.
\qed
\end{definition}

\ifx\EprintCalculus\undefined
\begin{theorem}
\label{theorem: limit of sequence, valued division ring, product on scalar}
Пусть $D$ - нормированное тело характеристики $0$ и пусть $d\in D$.
Пусть $a\in D$ - предел последовательности $\{a_n\}$.
Тогда
\[
\lim_{n\rightarrow\infty}(a_nd)=ad
\]
\[
\lim_{n\rightarrow\infty}(da_n)=da
\]
\end{theorem}
\begin{proof}
Утверждение теоремы тривиально, однако я привожу доказательство
для полноты текста. 
Поскольку $a\in D$ - предел последовательности $\{a_n\}$,
то согласно определению \ref{definition: limit of sequence, valued division ring}
для заданного $\epsilon\in R$, $\epsilon>0$,
существует натуральное число $n_0$ такое,
что $|a_n-a|<\epsilon/|d|$ для любого $n>n_0$.
Согласно определению \ref{definition: absolute value on division ring}
утверждение теоремы следует из неравенств
\[
|a_nd-ad|=|(a_n-a)d|=|a_n-a||d|<\epsilon/|d||d|=\epsilon
\]
\[
|da_n-da|=|d(a_n-a)|=|d||a_n-a|<|d|\epsilon/|d|=\epsilon
\]
для любого $n>n_0$.
\end{proof}
\fi

\begin{definition}
Пусть $D$ - нормированное тело.
Последовательность $\{a_n\}$, $a_n\in D$ называется 
\AddIndex{фундаментальной}{fundamental sequence, valued division ring}
или \AddIndex{последовательностью Коши}{Cauchy sequence, valued division ring},
если для любого $\epsilon\in R$, $\epsilon>0$
существует, зависящее от $ \epsilon$, натуральное число $n_0$ такое,
что $|a_p-a_q|<\epsilon$ для любых $p$, $q>n_0$.
\qed
\end{definition}

\begin{definition}
Нормированное тело $D$ называется 
\AddIndex{полным}{complete division ring}
если любая фундаментальная последовательность элементов
данного тела сходится, т. е.
имеет предел в этом теле.
\qed
\end{definition}

\ifx\EprintCalculus\undefined
До сих пор всё было хорошо. Кольцо целых чисел содержится в кольце
характеристики $0$. Поле рациональных чисел содержится в теле
характеристики $0$. Однако это не означает, что поле действительных
чисел содержится в полном теле $D$ характеристики $0$.
Например, мы можем определить норму на теле,
тождественно равную $1$. Эта норма определяет на нормированном
теле дискретную топологию и не представляет для нас интереса,
так как любая фундаментальная последовательность является
постоянным отображением.
\fi

В дальнейшем, говоря о нормированном теле характеристики $0$,
мы будем предполагать, что определён гомеоморфизм поля рациональных чисел $Q$
в тело $D$.

\begin{theorem}
\label{theorem: division ring contains real number}
Полное тело $D$ характеристики $0$
содержит в качестве подполя изоморфный образ поля $R$
действительных чисел.
Это поле обычно отождествляют с $R$.
\end{theorem}
\begin{proof}
Рассмотрим фундаментальную последовательность рациональных чисел $\{p_n\}$.
Пусть $p'$ - предел этой последовательности в теле $D$.
Пусть $p$ - предел этой последовательности в поле $R$.
Так как вложение поля $Q$ в тело $D$ гомеоморфно,
то мы можем отождествить $p'\in D$ и $p\in R$.
\end{proof}

\begin{theorem}
\label{theorem: division ring, real number}
Пусть $D$ - полное тело характеристики $0$ и пусть $d\in D$.
Тогда любое действительное число $p\in R$ коммутирует с $d$.
\end{theorem}
\begin{proof}
Мы можем представить действительное число $p\in R$ в
виде фундаментальной последовательности рациональных чисел $\{p_n\}$.
Утверждение теоремы следует из цепочки равенств
\[
pd=\lim_{n\rightarrow\infty}(p_nd)=\lim_{n\rightarrow\infty}(dp_n)=dp
\]
основанной на утверждении теоремы
\xRef{0812.4763}{theorem: limit of sequence, valued division ring, product on scalar}.
\end{proof}

\begin{theorem}
\label{theorem: real subring of center}
Пусть $D$ - полное тело характеристики $0$.
Тогда поле действительных чисел $R$ является подполем центра $Z(D)$ тела $D$.
\end{theorem}
\begin{proof}
Следствие теоремы \ref{theorem: division ring, real number}.
\end{proof}

\begin{definition}
Пусть $D$ - полное тело характеристики $0$.
Множество элементов $d\in D$, $|d|=1$ называется
\AddIndex{единичной сферой в теле}{unit sphere in division ring} $D$.
\qed
\end{definition}

\begin{definition}
\label{definition: continuous function, division ring}
Пусть $D_1$ - полное тело характеристики $0$ с нормой $|x|_1$.
Пусть $D_2$ - полное тело характеристики $0$ с нормой $|x|_2$.
Функция \[f:D_1\rightarrow D_2\]
называется \AddIndex{непрерывной}{continuous function, division ring}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\[
|x'-x|_1<\delta
\]
влечёт
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\begin{theorem}
\label{theorem: continuous map of division ring}
Пусть $D$ - полное тело характеристики $0$.
Если в разложении
\ifx\IntroCalculusBook\Defined
\eqref{eq: linear map, division ring, canonical morphism}
\else
\ifx\EprintCalculus\Defined
\eqref{eq: linear map, division ring, canonical morphism}
\else
\xEqRef{0701.238}{eq: linear map, division ring, canonical morphism}
\fi
\fi
аддитивного отображения \[f:D\rightarrow D\]
индекс $s$ принимает конечное множество значений,
то аддитивное отображение $f$
непрерывно.
\end{theorem}
\begin{proof}
Положим $x'=x+a$. Тогда
\[
f(x')-f(x)=f(x+a)-f(x)=f(a)=\pC{s}{0}f\ a\ \pC{s}{1}f
\]
\[
|f(x')-f(x)|=|\pC{s}{0}f\ a\ \pC{s}{1}f|<(|\pC{s}{0}f|\ |\pC{s}{1}f|)|a|
\]
Положим $F=|\pC{s}{0}f|\ |\pC{s}{1}f|$. Тогда
\[
|f(x')-f(x)|<F|a|
\]
Выберем $\epsilon>0$ и положим $\displaystyle a=\frac{\epsilon}Fe$.
Тогда $\displaystyle\delta=|a|=\frac{\epsilon}F$.
Согласно определению \ref{definition: continuous function, division ring}
аддитивное отображение $f$ непрерывно.
\end{proof}

\ifx\EprintCalculus\undefined
Аналогично, если индекс $s$ принимает счётное множество значений,
то для непрерывности аддитивного отображения $f$ мы требуем, что бы ряд
$|\pC{s}{0}f|\ |\pC{s}{1}f|$ сходился.
Если индекс $s$ принимает непрерывное множество значений,
то для непрерывности аддитивного отображения $f$ мы требуем, что бы интеграл
$\int|\pC{s}{0}f|\ |\pC{s}{1}f|ds$ существовал.
\fi

\begin{definition}
\label{definition: norm of map, division ring}
Пусть
\[f:D_1\rightarrow D_2\]
отображение полного тела $D_1$ характеристики $0$ с нормой $|x|_1$
в полное тело $D_2$ характеристики $0$ с нормой $|y|_2$.
Величина \symb{\|f\|}0{norm of map, division ring}
\begin{equation}
\ShowSymbol{norm of map, division ring}=
\text{sup}\frac{|f(x)|_2}{|x|_1}
\label{eq: norm of map, division ring}
\end{equation}
называется
\AddIndex{нормой отображения $f$}
{norm of map, division ring}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: norm of multiplicative map, division ring}
Пусть $D_1$ - полное тело характеристики $0$ с нормой $|x|_1$.
Пусть $D_2$ - полное тело характеристики $0$ с нормой $|x|_2$.
Пусть
\[f:D_1\rightarrow D_2\]
отображение, мультипликативное над полем $R$.
Тогда
\begin{equation}
\|f\|=\text{sup}\{|f(x)|_2:|x|_1=1\}
\label{eq: norm of multiplicative map, division ring}
\end{equation}
\end{theorem}
\begin{proof}
Согласно определению
\ifx\IntroCalculusBook\Defined
\ref{definition: map multiplicative over commutative ring, ring}
\else
\ifx\EprintCalculus\Defined
\ref{definition: map multiplicative over commutative ring, ring}
\else
\xRef{0701.238}{definition: map multiplicative over commutative ring, ring}
\fi
\fi
\[
\frac{|f(x)|_2}{|x|_1}=\frac{|f(rx)|_2}{|rx|_1}
\]
Полагая $\displaystyle r=\frac 1{|x|_1}$, мы получим
\begin{equation}
\frac{|f(x)|_2}{|x|_1}=\left|f\left(\frac x{|x|_1}\right)\right|_2
\label{eq: norm of multiplicative map, division ring, 1}
\end{equation}
Равенство \eqref{eq: norm of multiplicative map, division ring}
следует из равенств \eqref{eq: norm of multiplicative map, division ring, 1}
и \eqref{eq: norm of map, division ring}.
\end{proof}

\begin{theorem}
\label{theorem: continuity of additive map, finite norm, division ring}
Пусть
\[f:D_1\rightarrow D_2\]
аддитивное отображение полного тела $D_1$
в полное тело $D_2$.
Отображение $f$ непрерывно, если $\|f\|<\infty$.
\end{theorem}
\begin{proof}
Поскольку отображение $f$ аддитивно, то
согласно определению \ref{definition: norm of map, division ring}
\[
|f(x)-f(y)|_2=|f(x-y)|_2\le \|f\|\ |x-y|_1
\]
Возьмём произвольное $\epsilon>0$. Положим $\displaystyle\delta=\frac\epsilon{\|f\|}$.
Тогда из неравенства
\[
|x-y|_1<\delta
\]
следует
\[
|f(x)-f(y)|_2\le \|f\|\ \delta=\epsilon
\]
Согласно определению \ref{definition: continuous function, division ring}
отображение $f$ непрерывно.
\end{proof}

\ifx\texFuture\Defined
\begin{theorem}
\label{theorem: continuity of map, norm, division ring}
Пусть
\[f:D_1\rightarrow D_2\]
отображение полного тела $D_1$
в полное тело $D_2$.
Отображение $f$ непрерывно, если $\|f\|<\infty$.
\end{theorem}
\begin{proof}
Поскольку отображение $f$ аддитивно, то
согласно определению \ref{definition: norm of map, division ring}
\[
|f(x)-f(y)|_2=|f(x-y)|_2\le \|f\|\ |x-y|_1
\]
Возьмём произвольное $\epsilon>0$. Положим $\displaystyle\delta=\frac\epsilon{\|f\|}$.
Тогда из неравенства
\[
|x-y|_1<\delta
\]
следует
\[
|f(x)-f(y)|_2\le \|f\|\ \delta=\epsilon
\]
Согласно определению \ref{definition: continuous function, division ring}
отображение $f$ непрерывно.
\end{proof}
\fi

\begin{theorem}
\label{theorem: projective map in 0, division ring}
Пусть $D$ - полное тело характеристики $0$.
Либо непрерывное отображение $f$ тела, проективное над полем $P$,
не зависит от направления над полем $P$,
либо значение $f(0)$ не определено.
\end{theorem}
\begin{proof}
Согласно определению
\ifx\IntroCalculusBook\Defined
\ref{definition: map projective over commutative ring, ring},
\else
\xRef{0701.238}{definition: map projective over commutative ring, ring},
\fi
отображение $f$
постоянно на направлении $Pa$. Так как $0\in Pa$,
то естественно положить по непрерывности
\[
f(0)=f(a)
\]
Однако это приводит к неопределённости значения
отображения $f$ в направлении $0$,
если отображение $f$ имеет разное значение для разных направлений $a$.
\end{proof}

Если проективная над полем $R$ функция $f$ непрерывна,
то мы будем говорить, что функция $f$ \AddIndex{непрерывна
по направлению над полем $R$}
{projective function is continuous in direction over field R, division ring}.
Поскольку для любого $a\in D$, $a\ne 0$ мы можем выбрать
$a_1=|a|^{-1}a$, $f(a_1)=f(a)$, то мы можем сделать определение более точным.

\begin{definition}
\label{definition: projective function is continuous in direction over field R, division ring}
Пусть $D$ - полное тело характеристики $0$.
Проективная над полем $R$ функция $f$ непрерывна
по направлению над полем $R$, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\[
|x'-x|_1<\delta\ \ \ |x'|_1=|x|_1=1
\]
влечёт
\[
|f(x')-f(x)|_2<\epsilon
\]
\qed
\end{definition}

\begin{theorem}
\label{theorem: projective function is continuous in direction over field R, division ring}
Пусть $D$ - полное тело характеристики $0$.
Проективная над полем $R$ функция $f$ непрерывна
по направлению над полем $R$ тогда и только тогда, когда
эта функция непрерывна на единичной сфере тела $D$.
\end{theorem}
\begin{proof}
Следствие определений \ref{definition: continuous function, division ring},
\ifx\IntroCalculusBook\Defined
\ref{definition: map projective over commutative ring, ring},
\else
\xRef{0701.238}{definition: map projective over commutative ring, ring},
\fi
\ref{definition: projective function is continuous in direction over field R, division ring}.
\end{proof}

\section{Дифференцируемое отображение тела}
\label{section: Differentiable maps of Division Ring}

\ifx\IntroCalculusBook\Defined
\def\texFrechet{}
\begin{definition}
\label{definition: differentiable functions, division ring}
Пусть $D$ - нормированное тело.\footnote{Определение
дано согласно
определению \citeBib{Lebedev Vorovich}-3.1.1,
стр. 256.}
Функция \[f:D\rightarrow D\] называется
\AddIndex{\Ds дифференцируемой по Фреше}
{function Dstar differentiable in Frechet sense, division ring}
на множестве $U\subset D$\footnote{Так же как в замечании
\xRef{0701.238}{remark: drc linear map}
мы можем определить \Ds дифференцируемость отображения \[f:S\rightarrow D\]
нормированного тела $S$
в нормированное тело $D$ согласно правилу
\[
f(x+h)-f(x)
=F(h)\frac{d f(x)}{d_*x}
+o(h)
\]
где \[F:S\rightarrow D\] гомоморфизм тел.
Однако, опираясь на теоремы об изоморфизмах, мы можем ограничиться случаем
отображений тела $D$ в $D$.},
если в каждой точке $x\in U$ изменение функции $f$ может быть представлено в виде
\symb{\frac{d f(x)}{d_*x}}0{Frechet Dstar derivative of map, division ring}
\begin{equation}
\label{eq: Dstar derivative, division ring}
f(x+h)-f(x)
=h\ShowSymbol{Frechet Dstar derivative of map, division ring}
+o(h)
\end{equation}
где $o$ - такое непрерывное отображение
\[o:D\rightarrow D\]
что
\begin{equation}
\label{eq: infinitesimal, division ring}
\lim_{h\rightarrow 0}\frac{|o(h)|}{|h|}=0
\end{equation}
\qed
\end{definition}

Согласно определению \ref{definition: differentiable functions, division ring},
\AddIndex{\Ds производная Фреше отображения $f$ в точке $x$}
{Frechet Dstar derivative of map, division ring}
\[
\ShowSymbol{Frechet Dstar derivative of map, division ring}\in {}_*\mathcal L(D,D)
\]
порождает гомоморфизм
\[
\Delta f
=\Delta x\frac{d f(x)}{d_*x}
\]
отображающий приращение аргумента в приращение функции.

Если мы умножим обе части равенства
\eqref{eq: Dstar derivative, division ring}
на $h^{-1}$, то мы получим равенство
\begin{equation}
\label{eq: Dstar derivative, division ring, 1}
h^{-1}(f(x+h)-f(x))
=\frac{d f(x)}{d_*x}
+h^{-1}o(h)
\end{equation}
Из равенств \eqref{eq: Dstar derivative, division ring, 1} и
\eqref{eq: infinitesimal, division ring} следует
альтернативное определение \Ds производной Фреше
\begin{equation}
\label{eq: Dstar derivative, division ring, 2}
\frac{d f(x)}{d_*x}
=\lim_{h\rightarrow 0}(h^{-1}(f(x+h)-f(x)))
\end{equation}

Отличие \Ds производной Фреше отображения тела $D$ от производной отображения
поля $F$ состоит в том, что прежде всего \Ds производная Фреше не является
линейным отображением. Более точно, \Ds производная Фреше является \sD
линейным отображением, однако, вообще говоря, не является \Ds
линейным отображением. Действительно,
\[
f(x+h)a-f(x)a=h\frac{df}{d_*x}a+o(h)
\]
\begin{equation}
\label{eq: Dstar derivative, division ring, 3}
af(x+h)-af(x)=ah\frac{df}{d_*x}+o(h)
\end{equation}
Однако, вообще говоря,
\[
ah\frac{df}{d_*x}\ne ha\frac{df}{d_*x}
\]

Подобная проблема возникает при дифференцировании произведения функций.
Согласно определению \ref{definition: differentiable functions, division ring}
\begin{equation}
f(x+h)g(x+h)-f(x)g(x)
=h\frac{df(x)g(x)}{d_*x}+o(h)
\label{eq: product of maps, derivative, 0}
\end{equation}
Выражение в левой части можно представить в виде
\begin{align}
&f(x+h)g(x+h)-f(x)g(x)\nonumber\\
\label{eq: product of maps, derivative, 1}
=&f(x+h)g(x+h)-f(x)g(x+h)+f(x)g(x+h)-f(x)g(x)\\
=&(f(x+h)-f(x))g(x+h)+f(x)(g(x+h)-g(x))\nonumber
\end{align}
Согласно определению \ref{definition: differentiable functions, division ring},
мы можем представить \eqref{eq: product of maps, derivative, 1} в виде
\begin{align}
&f(x+h)g(x+h)-f(x)g(x)\nonumber\\
\label{eq: product of maps, derivative, 2}
=&\left(h\frac{df(x)}{d_*x}+o(h)\right)
\left(g(x)+h\frac{dg(x)}{d_*x}+o(h)\right)\\
+&f(x)\left(h\frac{dg(x)}{d_*x}+o(h)\right)\nonumber
\end{align}
Так как, вообще говоря,
\[
f(x)h\frac{dg}{d_*x}\ne hf(x)\frac{dg}{d_*x}
\]
то естественно ожидать, что функция $f(x)g(x)$
не является \Ds дифференцируемой по Фреше.

Таким образом, определение \Ds производной Фреше весьма ограничено
и не удовлетворяет стандартному определению операции дифференцирования.
Чтобы найти решение проблемы дифференцирования,
рассмотрим эту проблему с другой стороны.
\fi

\begin{example}
\label{example: differential dxx}
Рассмотрим приращение функции $f(x)=x^2$.
\begin{align*}
f(x+h)-f(x)
&=(x+h)^2-x^2
\\
&=xh+hx+h^2
\\
&=xh+hx+o(h)
\end{align*}
Как мы видим компонента приращения функции $f(x)=x^2$, линейно зависящая
от приращения аргумента, имеет вид
\[
xh+hx
\]
Так как произведение некомутативно,
то мы не можем представить приращение функции $f(x+h)-f(x)$
в виде $Ah$ или $hA$,
где $A$ не зависит от $h$.
Следствием этого является непредсказуемость поведения приращения функции $f(x)=x^2$,
когда приращение аргумента стремится к $0$.
Однако, если бесконечно малая величина $h$ будет бесконечно малой величиной
вида $h=ta$, $a\in D$, $t\in R$, $t\rightarrow 0$, то ответ становится
более определённым
\[
(xa+ax)t
\]
\qed
\end{example}

\begin{definition}
\label{definition: function differentiable in Gateaux sense, division ring}
Пусть $D$ - полное тело характеристики $0$.\footnote{Определение
дано согласно
определению \citeBib{Lebedev Vorovich}-3.1.2,
стр. 256.}
Функция \[f:D\rightarrow D\]
\AddIndex{дифференцируема по Гато}
{function differentiable in Gateaux sense, division ring} на множестве $U\subset D$,
если в каждой точке $x\in U$
изменение функции $f$ может быть представлено в виде
\symb{\partial f(x)}
0{Gateaux derivative of map, division ring}
\symb{\frac{\partial f(x)}{\partial x}}
0{Gateaux derivative of map, fraction, division ring}
\begin{equation}
\label{eq: Gateaux differential of map, division ring}
f(x+a)-f(x)
=\ShowSymbol{Gateaux derivative of map, division ring}(a)
+o(a)
=\ShowSymbol{Gateaux derivative of map, fraction, division ring}(a)
+o(a)
\end{equation}
где
\AddIndex{производная Гато
$\ShowSymbol{Gateaux derivative of map, division ring}$
отображения $f$}
{Gateaux derivative of map, division ring}
- линейное отображение приращения $a$ и
$o:D\rightarrow D$ - такое непрерывное отображение, что
\[
\lim_{a\rightarrow 0}\frac{|o(a)|}{|a|}=0
\]
\qed
\end{definition}

\begin{remark}
\label{remark: differential L(D,D)}
Согласно определению
\ref{definition: function differentiable in Gateaux sense, division ring}
при заданном $x$ производная Гато $\partial f(x)\in\mathcal L(D;D)$.
Следовательно, производная Гато отображения $f$ является отображением
\ShowEq{differential L(D,D)}
Выражения $\partial f(x)$ и $\displaystyle\frac{\partial f(x)}{\partial x}$
являются разными обозначениями одной и той же функции.
Мы будем пользоваться обозначением $\displaystyle\frac{\partial f(x)}{\partial x}$,
если хотим подчеркнуть, что мы берём производную Гато по переменной $x$.
\qed
\end{remark}

\begin{theorem}
\label{theorem: function differentiable in Gateaux sense, division ring}
\symb{\partial f(x)(a)}
0{Gateaux differential of map, division ring}
Мы можем представить \AddIndex{дифференциал Гато
$\ShowSymbol{Gateaux differential of map, division ring}$
отображения $f$}
{Gateaux differential of map, division ring}
в виде
\begin{equation}
\ShowSymbol{Gateaux differential of map, division ring}
=\frac{\pC{s}{0}\partial f(x)}{\partial x}
\ a
\ \frac{\pC{s}{1}\partial f(x)}{\partial x}
\label{eq: Gateaux differential, representation}
\end{equation}
\end{theorem}
\begin{proof}
Следствие определения \ref{definition: function differentiable in Gateaux sense, division ring}
и теоремы
\ifx\IntroCalculusBook\Defined
\ref{theorem: linear map, division ring, canonical morphism}.
\else
\ifx\EprintCalculus\Defined
\ref{theorem: linear map, division ring, canonical morphism}.
\else
\xRef{0701.238}{theorem: linear map, division ring, canonical morphism}.
\fi
\fi
\end{proof}

\begin{definition}
Выражение
\symb{\frac{\pC{s}{p}\partial f(x)}{\partial x}}0
{component of Gateaux derivative of map, division ring}
$\displaystyle\ShowSymbol{component of Gateaux derivative of map, division ring}$,
$p=0$, $1$, называется
\AddIndex{компонентой производной Гато отображения $f(x)$}
{component of Gateaux derivative of map, division ring}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: Gateaux derivative is multiplicative over field R, division ring}
Пусть $D$ - тело характеристики $0$.
Производная Гато
функции \[f:D\rightarrow D\]
мультипликативна над полем $R$.
\end{theorem}
\begin{proof}
Следствие теорем
\ref{theorem: real subring of center},
\ifx\IntroCalculusBook\Defined
\ref{theorem: additive map, division ring, center}
\else
\ifx\EprintCalculus\Defined
\ref{theorem: additive map, division ring, center}
\else
\xRef{0701.238}{theorem: additive map, division ring, center}
\fi
\fi
и
определения \ref{definition: function differentiable in Gateaux sense, division ring}.
\end{proof}

Из теоремы \ref{theorem: Gateaux derivative is multiplicative over field R, division ring}
следует
\begin{equation}
\label{eq: Gateaux differential is multiplicative over field R, division ring}
\partial f(x)(ra)
=
r\partial f(x)(a)
\end{equation}
для любых $r\in R$, $r\ne 0$ и $a\in D$, $a\ne 0$.
Комбинируя равенство \eqref{eq: Gateaux differential is multiplicative over field R, division ring}
и определение
\ref{definition: function differentiable in Gateaux sense, division ring},
мы получим знакомое определение дифференциала
Гато
\begin{equation}
\partial f(x)(a)=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}(f(x+ta)-f(x)))
\label{eq: Gateaux differential, representation, 2}
\end{equation}
Определения производной Гато \eqref{eq: Gateaux differential of map, division ring}
и \eqref{eq: Gateaux differential, representation, 2}
эквивалентны. На основе этой эквивалентности мы будем говорить,
что отображение $f$
дифференцируемо по Гато на множестве $U\subset D$,
если в каждой точке $x\in U$
изменение функции $f$ может быть представлено в виде
\begin{equation}
\label{eq: Gateaux differential of map, t, division ring}
f(x+ta)-f(x)
=t\partial f(x)(a)
+o(t)
\end{equation}
где
$o:R\rightarrow D$ - такое непрерывное отображение, что
\[
\lim_{t\rightarrow 0}\frac{|o(t)|}{|t|}=0
\]

Если бесконечно малая $ta$ является дифференциалом $dx$,
то равенство
\eqref{eq: Gateaux differential, representation}
примет вид
\begin{equation}
\partial f(x)(dx)
=\frac{\pC{s}{0}\partial f(x)}{\partial x}
dx
\frac{\pC{s}{1}\partial f(x)}{\partial x}
\label{eq: Gateaux differential, form}
\end{equation}

\begin{theorem}
\label{theorem: Gateaux differential, standard form, division ring}
Пусть $D$ - тело характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над центром $Z(D)$ тела $D$.
\symb{\StandPartial{f(x)}{x}{ij}}0
{standard component of Gateaux differential, division ring}
\AddIndex{Стандартное представление дифференциала Гато
\eqref{eq: Gateaux differential, representation}
отображения\[f:D\rightarrow D\]}
{Gateaux differential, standard representation, division ring}
имеет вид
\begin{equation}
\partial f(x)(a)
=\ShowSymbol{standard component of Gateaux differential, division ring}
\ {}_{\gi i}\Vector e\ a\ {}_{\gi j}\Vector e
\label{eq: Gateaux differential, division ring, standard representation}
\end{equation}
Выражение
$\displaystyle\ShowSymbol{standard component of Gateaux differential, division ring}$
в равенстве \eqref{eq: Gateaux differential, division ring, standard representation}
называется \AddIndex{стандартной компонентой дифференциала Гато отображения $f$}
{standard component of Gateaux differential, division ring}.
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теоремы
\ifx\IntroCalculusBook\Defined
\ref{theorem: linear map, standard form, division ring}.
\else
\ifx\EprintCalculus\Defined
\ref{theorem: linear map, standard form, division ring}.
\else
\xRef{0701.238}{theorem: linear map, standard form, division ring}.
\fi
\fi
\end{proof}

\begin{theorem}
Пусть $D$ - тело характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над центром $Z(D)$ тела $D$.
Тогда дифференциал Гато отображения
\[
f:D\rightarrow D
\]
можно записать в виде
\begin{equation}
\partial f(x)(a)=a^{\gi i}\ \frac{\partial f^{\gi j}}{\partial x^{\gi i}}
\ {}_{\gi j}\Vector e
\label{eq: Gateaux differential and jacobian, division ring}
\end{equation}
где $a\in D$ имеет разложение
\[
\begin{array}{ccc}
a=a^{\gi i}\ {}_{\gi i}\Vector e&&a^{\gi i}\in F
\end{array}
\]
относительно базиса $\Basis e$ и якобиан отображения $f$ имеет вид
\begin{equation}
\label{eq: standard components and jacobian, division ring}
\frac{\partial f^{\gi j}}{\partial x^{\gi i}}=
\StandPartial{f(x)}{x}{kr}\ {}_{\gi{ki}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi j}
\end{equation}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием теоремы
\ifx\IntroCalculusBook\Defined
\ref{theorem: linear map over field, division ring}.
\else
\ifx\EprintCalculus\Defined
\ref{theorem: linear map over field, division ring}.
\else
\xRef{0701.238}{theorem: linear map over field, division ring}.
\fi
\fi
\end{proof}

\ifx\EprintCalculus\undefined
Чтобы найти конструкцию, подобную производной в коммутативном случае.
мы должны выделить производную из дифференциала
отображения. Для этого мы должны вынести приращение аргумента за
скобки.\footnote{Это возможно в том случае, если все
$\displaystyle \frac{\pC{s}{0}\partial f(x)}{\partial x}=e$
либо все
$\displaystyle \frac{\pC{s}{1}\partial f(x)}{\partial x}=e$.
Поэтому определение \citeBib{Lebedev Vorovich}-3.1.2,
стр. 256, приводит нас либо к определению
\Ds производной Фреше,
либо к определению
\sD производной Фреше.}
Мы можем вынести $a$ за скобки,
опираясь на равенства
\[
\frac{\pC{s}{0}\partial f(x)}{\partial x}a
\frac{\pC{s}{1}\partial f(x)}{\partial x}
=\frac{\pC{s}{0}\partial f(x)}{\partial x}a
\frac{\pC{s}{1}\partial f(x)}{\partial x}a^{-1}a
\]
\[
\frac{\pC{s}{0}\partial f(x)}{\partial x}a
\frac{\pC{s}{1}\partial f(x)}{\partial x}
=aa^{-1}\frac{\pC{s}{0}\partial f(x)}{\partial x}a
\frac{\pC{s}{1}\partial f(x)}{\partial x}
\]
\fi

\begin{definition}
\label{definition: Gateaux Dstar derivative, division ring}
Пусть $D$ - полное тело характеристики $0$
и $a\in D$.
\symb{\frac{\partial f(x)(a)}{\partial_* x}}
0{Gateaux Dstar derivative of map, division ring}
\AddIndex{\Ds производная Гато
$\displaystyle\ShowSymbol{Gateaux Dstar derivative of map, division ring}$
отображения $f:D\rightarrow D$}
{Gateaux Dstar derivative of map, division ring}
определена равенством
\begin{equation}
\label{eq: Gateaux Dstar derivative, division ring}
\partial f(x)(a)
=a\ShowSymbol{Gateaux Dstar derivative of map, division ring}
\end{equation}
\symb{\frac{\partial f(x)(a)}{{}_*\partial x}}
0{Gateaux starD derivative of map, division ring}
\AddIndex{\sD производная Гато
$\displaystyle\ShowSymbol{Gateaux starD derivative of map, division ring}$
отображения $f:D\rightarrow D$}
{Gateaux starD derivative of map, division ring}
определена равенством
\begin{equation}
\label{eq: Gateaux starD derivative, division ring}
\partial f(x)(a)
=\ShowSymbol{Gateaux starD derivative of map, division ring}a
\end{equation}
\qed
\end{definition}

Рассмотрим базис ${}_1e=1$, ${}_2e=i$, ${}_3e=j$, ${}_4e=k$
тела кватернионов над полем действительных чисел.
Из непосредственных вычислений следует, что
стандартное \Ds представление дифференциала Гато отображения $x^2$
имеет вид
\[
\partial x^2(a)=(x+x_1)a+x_2ai+x_3aj+x_4ak
\]

\ifx\EprintCalculus\undefined
Для представления \Ds производной Гато
мы также будем пользоваться записью
\[
\frac{\partial f(x)(a)}{\partial_* x}=\frac{\partial}{\partial_* x} f(x)(a)=\partial_* f(x)(a)
\]

Для представления \sD производной Гато
мы также будем пользоваться записью
\[
\frac{\partial f(x)(a)}{{}_*\partial x}=\frac{\partial}{{}_*\partial x} f(x)(a)={}_*\partial f(x)(a)
\]

Опираясь на принцип двойственности
\xRef{0701.238}{theorem: duality principle, vector space},
мы будем изучать \Ds производную, имея в виду, что двойственное утверждение
справедливо для \sD производной.

Поскольку произведение не коммутативно, понятие дроби не определено в теле.
Мы должны явно указать, с какой стороны знаменатель действует на числитель.
Эту функцию выполняет символ $*$ в знаменателе дроби.
Согласно определению
\[
\frac{\partial f}{\partial_* x}=(\partial_* x)^{-1}\partial f
\]
\[
\frac{\partial f}{{}_*\partial x}=\partial f({}_*\partial x)^{-1}
\]
Таким образом, мы можем представить
\Ds производную Гато функции $f$
как отношение изменения функции к изменению аргумента.
Это замечание не распространяется на
компоненты дифференциала Гато.
В этом случае мы рассматриваем запись
$\displaystyle\frac{\partial}{\partial_* x}$
и $\displaystyle\frac{\partial}{{}_*\partial x}$ не
как дроби, а как символы операторов.

При этом равенство \eqref{eq: Gateaux Dstar derivative, division ring}
можно записать в виде
\begin{equation}
\label{eq: Gateaux differential, division ring, 1}
\partial f(x)(dx)
=dx(\partial_* x)^{-1}\partial f(x)(dx)
\end{equation}
Нетрудно видеть, что в знаменателе дроби в равенстве
\eqref{eq: Gateaux differential, division ring, 1}
мы записали \Ds дифференциал переменной $x$, а умножаем дробь на
дифференциал переменной $x$.
\fi

\begin{theorem}
\label{theorem: Dstar derivative is multiplicative over field R, division ring}
Пусть $D$ - полное тело характеристики $0$.
\Ds производная Гато проективна
над полем действительных чисел $R$.
\end{theorem}
\begin{proof}
Следствие теоремы \ref{theorem: Gateaux derivative is multiplicative over field R, division ring}
и примера
\ifx\IntroCalculusBook\Defined
\ref{example: map projective over commutative ring, ring}.
\else
\ifx\EprintCalculus\Defined
\ref{example: map projective over commutative ring, ring}.
\else
\xRef{0701.238}{example: map projective over commutative ring, ring}.
\fi
\fi
\end{proof}

Из теоремы \ref{theorem: Dstar derivative is multiplicative over field R, division ring}
следует
\begin{equation}
\label{eq: Dstar derivative is multiplicative over field R, division ring}
\frac{\partial f(x)(ra)}{\partial_* x}
=\frac{\partial f(x)(a)}{\partial_* x}
\end{equation}
для любых $r\in R$, $r\ne 0$ и  $a\in D$, $a\ne 0$.
Следовательно, \Ds производная Гато
хорошо определена в направлении $a$ над полем $R$, $a\in D$, $a\ne 0$, 
и не зависит от выбора значения в этом направлении.

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$
и $a\ne 0$.
\Ds производная Гато и \sD производная Гато отображения $f$ тела $D$
связаны соотношением
\begin{equation}
\label{eq: Dstar derivative and starD derivative in direction, division ring}
\frac{\partial f(x)(a)}{{}_*\partial x} 
=a\frac{\partial f(x)(a)}{\partial_* x} a^{-1}
\end{equation}
\end{theorem}
\begin{proof}
Из равенств \eqref{eq: Gateaux Dstar derivative, division ring}
и \eqref{eq: Gateaux starD derivative, division ring}
следует
\[
\frac{\partial f(x)(a)}{{}_*\partial x}
=\partial f(x)(a)a^{-1}
=a\frac{\partial f(x)(a)}{\partial_* x}a^{-1}
\]
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Дифференциал Гато удовлетворяет соотношению
\begin{equation}
\label{eq: Gateaux differential of product, division ring}
\partial (f(x)g(x))(a)
=\partial f(x)(a)\ g(x)+f(x)\ \partial g(x)(a)
\end{equation}
\end{theorem}
\begin{proof}
Равенство \eqref{eq: Gateaux differential of product, division ring}
следует из цепочки равенств
\begin{align*}
\partial (f(x)g(x))(a)
&=\lim_{t\rightarrow 0}(t^{-1}(f(x+ta)g(x+ta)-f(x)g(x)))
\\
&=\lim_{t\rightarrow 0}(t^{-1}(f(x+ta)g(x+ta)-f(x)g(x+ta)))
\\
&+\lim_{t\rightarrow 0}(t^{-1}(f(x)g(x+ta)-f(x)g(x)))
\\
&=\lim_{t\rightarrow 0}(t^{-1}(f(x+ta)-f(x)))g(x)
\\
&+f(x)\lim_{t\rightarrow 0}(t^{-1}(g(x+ta)-g(x)))
\end{align*}
основанной на определении \eqref{eq: Gateaux differential, representation, 2}.
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Допустим дифференциал Гато
отображения $f:D\rightarrow D$
имеет разложение
\begin{equation}
\label{eq: Gateaux differential of f, division ring}
\partial f(x)(a)
=\frac{\pC{s}{0}\partial f(x)}{\partial x}
a
\frac{\pC{s}{1}\partial f(x)}{\partial x}
\end{equation}
Допустим дифференциал Гато
отображения $g:D\rightarrow D$
имеет разложение
\begin{equation}
\label{eq: Gateaux differential of g, division ring}
\partial g(x)(a)
=\frac{\pC{t}{0}\partial g(x)}{\partial x}
a
\frac{\pC{t}{1}\partial g(x)}{\partial x}
\end{equation}
Компоненты дифференциала Гато отображения $f(x)g(x)$
имеют вид
\begin{align}
\label{eq: 0 component of Gateaux derivative, fg, division ring}
\frac{\pC{s}{0}\partial f(x)g(x)}{\partial x}
&
=\frac{\pC{s}{0}\partial f(x)}{\partial x}
&
\frac{\pC{t}{0}\partial f(x)g(x)}{\partial x}
&
=f(x)\frac{\pC{t}{0}\partial g(x)}{\partial x}
\\
\label{eq: 1 component of Gateaux derivative, fg, division ring}
\frac{\pC{s}{1}\partial f(x)g(x)}{\partial x}
&
=\frac{\pC{s}{1}\partial f(x)}{\partial x}
g(x)
&
\frac{\pC{t}{1}\partial f(x)g(x)}{\partial x}
&
=\frac{\pC{t}{1}\partial g(x)}{\partial x}
\end{align}
\end{theorem}
\begin{proof}
Подставим \eqref{eq: Gateaux differential of f, division ring}
и \eqref{eq: Gateaux differential of g, division ring}
в равенство \eqref{eq: Gateaux differential of product, division ring}
\begin{align}
\label{eq: Gateaux differential of fg, division ring}
\partial (f(x) g(x))(a)
&=\partial f(x)(a)\ g(x)+f(x)\ \partial g(x)(a)
\\ \nonumber
&=\frac{\pC{s}{0}\partial f(x)}{\partial x}a
\frac{\pC{s}{1}\partial f(x)}{\partial x}
g(x)
+f(x)\frac{\pC{t}{0}\partial g(x)}{\partial x}a
\frac{\pC{t}{1}\partial g(x)}{\partial x}
\end{align}
Опираясь на \eqref{eq: Gateaux differential of fg, division ring},
мы определяем равенства
\eqref{eq: 0 component of Gateaux derivative, fg, division ring},
\eqref{eq: 1 component of Gateaux derivative, fg, division ring}.
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
\Ds производная Гато удовлетворяет соотношению
\begin{equation}
\label{eq: Gateaux Dstar derivative of product, division ring}
\frac{\partial f(x)g(x)}{\partial_* x}(a)
=\frac{\partial f(x)(a)}{\partial_* x}g(x)+a^{-1}f(x)a\frac{\partial g(x)(a)}{\partial_* x}
\end{equation}
\end{theorem}
\begin{proof}
Равенство \eqref{eq: Gateaux Dstar derivative of product, division ring}
следует из цепочки равенств
\begin{align*}
\frac{\partial f(x)g(x)}{\partial_* x}(a)
&=a^{-1}\partial f(x)g(x)(a)
\\
&=a^{-1}(\partial f(x)(a)g(x)+f(x)\partial g(x)(a))
\\
&=a^{-1}\partial f(x)(a)g(x)+a^{-1}f(x)aa^{-1}\partial g(x)(a)
\\
&=\frac{\partial f(x)(a)}{\partial_* x}g(x)+a^{-1}f(x)a\frac{\partial g(x)(a)}{\partial_* x}
\end{align*}
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Либо \Ds производная Гато не зависит от направления,
либо \Ds производная Гато в направлении $0$ не определена.
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием
теоремы \ref{theorem: Dstar derivative is multiplicative over field R, division ring}
и теоремы \ref{theorem: projective map in 0, division ring}.
\end{proof}

\begin{theorem}
\label{theorem: norm of Gateaux differential, division ring}
Пусть $D$ - полное тело характеристики $0$.
Пусть единичная сфера тела $D$ - компактна.
Если \Ds производная Гато
$\displaystyle\frac{\partial f(x)(a)}{\partial_* x}$
существует в точке $x$ и непрерывна по направлению над полем $R$,
то существует норма $\|\partial f(x)\|$ дифференциала Гато.
\end{theorem}
\begin{proof}
Из определения \ref{definition: Gateaux Dstar derivative, division ring}
следует
\begin{equation}
\label{eq: norm of Gateaux differential, division ring, 1}
|\partial f(x)(a)|
=|a|\ \left|\frac{\partial f(x)(a)}{\partial_* x}\right|
\end{equation}
Из теорем
\xRef{0812.4763}{theorem: projective function is continuous in direction over field R, division ring},
\ref{theorem: Dstar derivative is multiplicative over field R, division ring}
следует, что \Ds производная Гато непрерывна
на единичной сфере.
Так как единичная сфера компактна, то множество значений
\Ds производной Гато функции $f$ в точке $x$ ограниченно
\[
\left|
\frac{\partial f(x)(a)}{\partial_* x}
\right|
<F=\text{sup}\left|
\frac{\partial f(x)(a)}{\partial_* x}
\right|
\]
Согласно определению \ref{definition: norm of map, division ring}
\[
\|\partial f(x)\|=F
\]
\end{proof}

\begin{theorem}
\label{theorem: Dstar derivative and continuos function, division ring}
Пусть $D$ - полное тело характеристики $0$.
Пусть единичная сфера тела $D$ - компактна.
Если \Ds производная Гато
$\displaystyle\frac{\partial f(x)(a)}{\partial_* x}$
существует в точке $x$ и непрерывна по направлению над полем $R$,
то отображение $f$ непрерывно в точке $x$.
\end{theorem}
\begin{proof}
Из теоремы \ref{theorem: norm of Gateaux differential, division ring}
следует
\begin{equation}
\label{eq: Dstar derivative and continuos function, division ring, 1}
|\partial f(x)(a)|
\le\|\partial f(x)\| |a|
\end{equation}
Из \eqref{eq: Gateaux differential of map, division ring},
\eqref{eq: Dstar derivative and continuos function, division ring, 1}
следует
\begin{equation}
\label{eq: Dstar derivative and continuos function, division ring, 2}
|f(x+a)-f(x)|<|a|\ \|\partial f(x)\|
\end{equation}
Возьмём произвольное $\epsilon>0$. Положим
\[\delta=\frac\epsilon{\|\partial f(x)\|}\]
Тогда из неравенства
\[
|a|<\delta
\]
следует
\[
|f(x+a)-f(x)|\le \|\partial f(x)\|\ \delta=\epsilon
\]
Согласно определению \ref{definition: continuous function, division ring}
отображение $f$ непрерывно в точке $x$.
\end{proof}

\ifx\EprintCalculus\undefined
Теорема \ref{theorem: Dstar derivative and continuos function, division ring}
имеет интересное обобщение. Если единичная сфера тела $D$ не является компактной,
то мы можем рассмотреть компактное множество направлений вместо единичной сферы.
В этом случае, мы можем говорить о непрерывности функции $f$ вдоль заданного множества
направлений.
\fi

\section{Таблица производных Гато отображения тела}

\begin{theorem}
\label{theorem: Gateaux differential of const, division ring}
Пусть $D$ - полное тело характеристики $0$.
Тогда для любого $b\in D$
\begin{equation}
\label{eq: Gateaux differential of const, division ring}
\partial (b)(a)
=0
\end{equation}
\end{theorem}
\begin{proof}
Непосредственное следствие определения
\ref{definition: function differentiable in Gateaux sense, division ring}.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux differential, product over constant, division ring}
Пусть $D$ - полное тело характеристики $0$.
Тогда для любых $b$, $c\in D$
\begin{align}
\label{eq: Gateaux differential, product over constant, division ring}
\partial (bf(x)c)(a)
&=b\partial f(x)(a)c
\\
\label{eq: 0 component of Gateaux differential, product over constant, division ring}
\frac{\pC{s}{0}\partial bf(x)c}{\partial x}
&=b\frac{\pC{s}{0}\partial f(x)}{\partial x}
\\
\label{eq: 1 component of Gateaux differential, product over constant, division ring}
\frac{\pC{s}{1}\partial bf(x)c}{\partial x}
&=\frac{\pC{s}{1}\partial f(x)}{\partial x}c
\\
\label{eq: Gateaux derivative, product over constant, division ring}
\frac{\partial bf(x)c}{\partial_* x}(a)
&=a^{-1}ba\frac{\partial f(x)(a)}{\partial_* x}c
\end{align}
\end{theorem}
\begin{proof}
Непосредственное следствие равенств
\eqref{eq: Gateaux differential of product, division ring},
\eqref{eq: 0 component of Gateaux derivative, fg, division ring},
\eqref{eq: 1 component of Gateaux derivative, fg, division ring},
\eqref{eq: Gateaux Dstar derivative of product, division ring},
так как $\partial b=\partial c=0$.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux differential, product over constant, fx=x, division ring}
Пусть $D$ - полное тело характеристики $0$.
Тогда для любых $b$, $c\in D$
\begin{align}
\label{eq: Gateaux differential, product over constant, fx=x, division ring}
\partial (bxc)(h)
&=bhc
\\
\label{eq: 0 component of Gateaux differential, product over constant, fx=x, division ring}
\frac{\pC{1}{0}\partial bxc}{\partial x}
&=b
\\
\label{eq: 1 component of Gateaux differential, product over constant, fx=x, division ring}
\frac{\pC{1}{1}\partial bxc}{\partial x}
&=c
\\
\label{eq: Gateaux derivative, product over constant, fx=x, division ring}
\frac{\partial bf(x)c}{\partial_* x}(h)
&=h^{-1}bhc
\end{align}
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: Gateaux differential, product over constant, division ring},
когда $f(x)=x$.
\end{proof}

\begin{theorem}
%\label{theorem: Gateaux differential, product over constant, fx=x, division ring}
Пусть $D$ - полное тело характеристики $0$.
Тогда для любого $b\in D$
\begin{align}
\label{eq: Gateaux differential, xb-bx, division ring}
\partial (xb-bx)(h)
&=hb-bh
\\
\nonumber
\frac{\pC{1}{0}\partial (xb-bx)}{\partial x}
&=1
&
\frac{\pC{1}{1}\partial (xb-bx)}{\partial x}
&=b
\\
\nonumber
\frac{\pC{2}{0}\partial (xb-bx)}{\partial x}
&=-b
&
\frac{\pC{2}{1}\partial (xb-bx)}{\partial x}
&=1
\\
\nonumber
\frac{\partial (xb-bx)}{\partial_* x}(h)
&=h^{-1}bhc
\end{align}
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: Gateaux differential, product over constant, division ring},
когда $f(x)=x$.
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Тогда
\begin{equation}
 \begin{array}{rl}
\partial (x^2)(a)&=xa+ax
\\
\displaystyle\frac{\partial x^2}{\partial_*x}(a)
&=a^{-1}xa+x
\end{array}
\label{eq: derivative x2, division ring}
\end{equation}
\begin{equation}
 \begin{array}{ccc}
\displaystyle\frac{\pC{1}{0}\partial x^2}{\partial x}=x
&
\displaystyle\frac{\pC{1}{1}\partial x^2}{\partial x}=e
\\ \\
\displaystyle\frac{\pC{2}{0}\partial x^2}{\partial x}=e
&
\displaystyle\frac{\pC{2}{1}\partial x^2}{\partial x}=x
\end{array}
\label{eq: derivative x2, component of Gateaux differential, division ring}
\end{equation}
\end{theorem}
\begin{proof}
\eqref{eq: derivative x2, division ring} следует из примера \ref{example: differential dxx}
и определения \ref{definition: Gateaux Dstar derivative, division ring}.
\eqref{eq: derivative x2, component of Gateaux differential, division ring}
следует из примера \ref{example: differential dxx}
и равенства \eqref{eq: Gateaux differential, form}.
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Тогда
\begin{align}
\partial (x^{-1})(h)&=-x^{-1}hx^{-1}
\label{eq: derivative x power -1, division ring}
\\
\displaystyle\frac{\partial x^{-1}}{\partial_*x}(h)
&=-h^{-1}x^{-1}hx^{-1}
\nonumber
\end{align}
\[
 \begin{array}{ccc}
\displaystyle\frac{\pC{1}{0}\partial x^{-1}}{\partial x}=-x^{-1}
&
\displaystyle\frac{\pC{1}{1}\partial x^{-1}}{\partial x}=x^{-1}
\end{array}
\]
\end{theorem}
\begin{proof}
Подставим $f(x)=x^{-1}$ в определение \eqref{eq: Gateaux differential, representation, 2}.
\begin{align}
\partial f(x)(h)
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}((x+th)^{-1}-x^{-1}))
\nonumber
\\
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}((x+th)^{-1}-x^{-1}(x+th)(x+th)^{-1}))
\nonumber
\\
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}(1-x^{-1}(x+th))(x+th)^{-1})
\label{eq: derivative x power -1, division ring, 1}
\\
&=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}(1-1-x^{-1}th)(x+th)^{-1})
\nonumber
\\
&=\lim_{t\rightarrow 0,\ t\in R}(-x^{-1}h(x+th)^{-1})
\nonumber
\end{align}
Равенство \eqref{eq: derivative x power -1, division ring}
следует из цепочки равенств
\eqref{eq: derivative x power -1, division ring, 1}.
\end{proof}

\begin{theorem}
Пусть $D$ - полное тело характеристики $0$.
Тогда
\begin{align}
\partial (xax^{-1})(h)&=hax^{-1}-xax^{-1}hx^{-1}
\label{eq: derivative xax power -1, division ring}
\\
\displaystyle\frac{\partial xax^{-1}}{\partial_*x}(h)
&=ax^{-1}-h^{-1}xax^{-1}hx^{-1}
\nonumber
\end{align}
\[
 \begin{array}{lll}
\displaystyle\frac{\pC{1}{0}\partial x^{-1}}{\partial x}=1
&
\displaystyle\frac{\pC{1}{1}\partial x^{-1}}{\partial x}=ax^{-1}
\\
\displaystyle\frac{\pC{2}{0}\partial x^{-1}}{\partial x}=-xax^{-1}
&
\displaystyle\frac{\pC{2}{1}\partial x^{-1}}{\partial x}=x^{-1}
\end{array}
\]
\end{theorem}
\begin{proof}
Равенство \eqref{eq: derivative xax power -1, division ring}
является следствием равенств \eqref{eq: Gateaux differential of product, division ring},
\eqref{eq: Gateaux differential, product over constant, fx=x, division ring},
\eqref{eq: derivative xax power -1, division ring}.
\end{proof}

\section{Производная второго порядка отображения тела}

Пусть $D$ - нормированное тело характеристики $0$.
Пусть
\[f:D\rightarrow D\]
функция, дифференцируемая по Гато.
Согласно замечанию \ref{remark: differential L(D,D)}
производная Гато является отображением
\ShowEq{differential L(D,D)}
Согласно теоремам
\ifx\IntroCalculusBook\Defined
\ref{theorem: sum of additive maps, ring},
\ref{theorem: additive map times constant, ring}
\else
\ifx\EprintCalculus\Defined
\ref{theorem: sum of additive maps, ring},
\ref{theorem: additive map times constant, ring}
\else
\xRef{0701.238}{theorem: sum of additive maps, ring},
\xRef{0701.238}{theorem: additive map times constant, ring}
\fi
\fi
и определению \ref{definition: norm of map, division ring}
множество $\mathcal L(D;D)$ является
нормированным $D$\Hyph векторным пространством.
Следовательно, мы можем рассмотреть вопрос,
является ли отображение $\partial f$ дифференцируемым по Гато.

Согласно определению
\xRef{0812.4763}{definition: function differentiable in Gateaux sense, D vector space}
\ShowEq{Gateaux differential of map df, division ring}
где
\ShowEq{Gateaux differential of map df, division ring, o2}
- такое непрерывное отображение, что
\ShowEq{Gateaux differential of map df, division ring, o2 lim}
Согласно определению
\xRef{0812.4763}{definition: function differentiable in Gateaux sense, D vector space}
отображение $\partial(\partial f(x)(a_1))(a_2)$
линейно по переменной $a_2$. Из равенства
\eqref{eq: Gateaux differential of map df, division ring}
следует, что отображение
$\partial(\partial f(x)(a_1))(a_2)$
линейно по переменной $a_1$.

\begin{definition}
\label{definition: Gateaux Differential of Second Order, division ring}
Полилинейное отображение
\symb{\partial^2 f(x)}
0{Gateaux derivative of Second Order, division ring}
\symb{\frac{\partial^2 f(x)}{\partial x^2}}
0{Gateaux derivative of Second Order, fraction, division ring}
\begin{equation}
\label{eq: Gateaux derivative of Second Order, division ring}
\ShowSymbol{Gateaux derivative of Second Order, division ring}(a_1;a_2)
=\ShowSymbol{Gateaux derivative of Second Order, fraction, division ring}(a_1;a_2)
=\partial(\partial f(x)(a_1))(a_2)
\end{equation}
называется
\AddIndex{производной Гато второго порядка отображения $f$}
{Gateaux derivative of Second Order, division ring}
\qed
\end{definition}

\begin{remark}
\label{remark: differential L(D,D;D)}
Согласно определению
\ref{definition: Gateaux Differential of Second Order, division ring}
при заданном $x$ дифференциал Гато второго порядка
\ShowEq{differential L(D,D;D), 1}.
Следовательно, дифференциал Гато второго порядка отображения $f$ является отображением
\ShowEq{differential L(D,D;D)}
\end{remark}

\begin{theorem}
\label{theorem: Gateaux Differential of Second Order, division ring}
\symb{\partial^2 f(x)(a_1;a_2)}
0{Gateaux differential of Second Order, division ring}
Мы можем представить \AddIndex{дифференциал Гато второго порядка отображения $f$}
{Gateaux differential of Second Order, division ring}
в виде
\ShowEq{Differential of Second Order, division ring, representation}
\end{theorem}
\begin{proof}
Следствие определения \ref{definition: Gateaux Differential of Second Order, division ring}
и теоремы
\ifx\IntroCalculusBook\Defined
\ref{theorem: polyadditive map, D vector space}.
\else
\xRef{0701.238}{theorem: polyadditive map, D vector space}.
\fi
\end{proof}

\begin{definition}
Мы будем называть выражение\footnote{Мы полагаем
\[
\frac{\pC{s}{p}\partial^2 f(x)}{\partial x^2}=\frac{\pC{s}{p}\partial^2 f(x)}{\partial x\partial x}
\]}
\symb{\frac{\pC{s}{p}\partial^2 f(x)}{\partial x^2}}0
{component of Gateaux derivative of Second Order, division ring}
$\displaystyle\ShowSymbol{component of Gateaux derivative of Second Order, division ring}$,
$p=0$, $1$,
\AddIndex{компонентой производной Гато отображения $f(x)$}
{component of Gateaux derivative of Second Order, division ring}.
\qed
\end{definition}

По индукции, предполагая, что определена производная Гато
$\partial^{n-1} f(x)$ порядка $n-1$, мы определим
\symb{\partial^n f(x)}
0{Gateaux derivative of Order n, division ring}
\symb{\frac{\partial^n f(x)}{\partial x^n}}
0{Gateaux derivative of Order n, fraction, division ring}
\begin{equation}
\label{eq: Gateaux derivative of Order n, division ring}
\ShowSymbol{Gateaux derivative of Order n, division ring}(a_1;...;a_n)
=\ShowSymbol{Gateaux derivative of Order n, fraction, division ring}(a_1;...;a_n)
=\partial(\partial^{n-1} f(x)(a_1;...;a_{n-1}))(a_n)
\end{equation}
\AddIndex{производную Гато порядка $n$ отображения $f$}
{Gateaux derivative of Order n, division ring}.
Мы будем также полагать $\partial^0 f(x)=f(x)$.

\section{Ряд Тейлора}
\label{section: Taylor Series}

Рассмотрим многочлен одной переменной над телом $D$ степени $n$, $n>0$. Нас
интересует структура одночлена $p_k(x)$ многочлена степени $k$.

Очевидно, что одночлен степени $0$ имеет вид $a_0$, $a_0\in D$.
Пусть $k>0$. Докажем, что
\[
p_k(x)=p_{k-1}(x)xa_k
\]
где $a_k\in D$.
Действительно, последний множитель одночлена $p_k(x)$ является либо $a_k\in D$,
либо имеет вид $x^l$, $l\ge 1$.
В последнем случае мы положим $a_k=1$.
Множитель, предшествующий $a_k$, имеет вид $x^l$, $l\ge 1$.
Мы можем представить этот множитель в виде $x^{l-1}x$.
Следовательно, утверждение доказано.

В частности, одночлен степени $1$ имеет вид $p_1(x)=a_0xa_1$.

Не нарушая общности, мы можем положить $k=n$.

\begin{theorem}
\label{theorem: Gateaux derivative of f(x)x, division ring}
Для произвольного $m>0$ справедливо равенство
\begin{align}
&\partial^m (f(x)x)(h_1;...;h_m)
\nonumber \\
=&\partial^m f(x)(h_1;...;h_m)x
+\partial^{m-1} f(x)(h_1;...;h_{m-1})h_m
\label{eq: Gateaux derivative of f(x)x, division ring}
\\ \nonumber
+&\partial^{m-1} f(x)(\widehat{h_1};...;h_{m-1};h_m)h_1
+...
\\ \nonumber
+&\partial^{m-1} f(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}
\end{align}
где символ $\widehat{h^i}$ означает отсутствие переменной $h^i$ в списке.
\end{theorem}
\begin{proof}
Для $m=1$ - это следствие равенства \eqref{eq: Gateaux differential of product, division ring}
\[
\partial (f(x)x)(h_1)=\partial f(x)(h_1)x+
f(x)h_1
\]
Допустим, \eqref{eq: Gateaux derivative of f(x)x, division ring} справедливо
для $m-1$. Тогда
\begin{align}
&\partial^{m-1} (f(x)x)(h_1;...;h_{m-1})
\nonumber \\
=&\partial^{m-1} f(x)(h_1;...;h_{m-1})x
+\partial^{m-2} f(x)(h_1;...;h_{m-2})h_{m-1}
\label{eq: Gateaux derivative of f(x)x, m-1, division ring}
\\ \nonumber
+&\partial^{m-2} f(x)(\widehat{h_1},...,h_{m-2},h_{m-1})h_1
+...
\\ \nonumber
+&\partial^{m-2} f(x)(h_1,...,\widehat{h_{m-2}},h_{m-1})h_{m-2}
\end{align}
Пользуясь равенствами \eqref{eq: Gateaux differential of product, division ring}
и \eqref{eq: Gateaux differential, product over constant, division ring}
получим
\begin{align}
&\partial^m (f(x)x)(h_1;...;h_{m-1};h_m)
\nonumber \\
=&\partial^m f(x)(h_1;...;h_{m-1};h_m)x
+\partial^{m-1} f(x)(h_1;...;h_{m-2};h_{m-1})h_m
\nonumber \\
+&\partial^{m-1} f(x)(h_1;...;h_{m-2};\widehat{h_{m-1}};h_m)h_{m-1}
\label{eq: Gateaux derivative of f(x)x, m, division ring}
\\ \nonumber
+&\partial^{m-2} f(x)(\widehat{h_1},...,h_{m-2},h_{m-1};h_m)h_1
+...
\\ \nonumber
+&\partial^{m-2} f(x)(h_1,...,\widehat{h_{m-2}},h_{m-1};h_m)h_{m-2}
\end{align}
Равенства \eqref{eq: Gateaux derivative of f(x)x, division ring} и
\eqref{eq: Gateaux derivative of f(x)x, m, division ring}
отличаются только формой записи.
Теорема доказана.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn is simetric, m less than n, division ring}
Производная Гато $\partial^m p_n(x)(h_1,...,h_m)$
является симметричным многочленом по переменным $h_1$, ..., $h_m$.
\end{theorem}
\begin{proof}
Для доказательства теоремы мы рассмотрим алгебраические свойства
производной Гато и дадим эквивалентное определение.
Мы начнём с построения одночлена.
Для произвольного одночлена $p_n(x)$ мы построим симметричный
многочлен $r_n(x)$ согласно следующим правилам
\begin{itemize}
\item Если $p_1(x)=a_0xa_1$, то $r_1(x_1)=a_0x_1a_1$
\item Если $p_n(x)=p_{n-1}(x)a_n$, то
\[
r_n(x_1,...,x_n)=r_{n-1}(x_{[1},...,x_{n-1})x_{n]}a_n
\]
где квадратные скобки выражают симметризацию выражения
по переменным $x_1$, ..., $x_n$.
\end{itemize}
Очевидно, что
\[
p_n(x)=r_n(x_1,...,x_n)\ \ \ x_1=...=x_n=x
\]
Мы определим производную Гато порядка $k$ согласно правилу
\begin{equation}
\partial^k p_n(x)(h_1,...,h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\label{eq: Gateaux derivative of monomial, algebraic definition, division ring}
\end{equation}
Согласно построению многочлен $r_n(h_1,...,h_k,x_{k+1},...,x_n)$
симметричен по переменным $h_1$, ..., $h_k$, $x_{k+1}$, ..., $x_n$.
Следовательно, многочлен
\eqref{eq: Gateaux derivative of monomial, algebraic definition, division ring}
симметричен по переменным $h_1$, ..., $h_k$.

При $k=1$ мы докажем, что определение
\eqref{eq: Gateaux derivative of monomial, algebraic definition, division ring}
производной Гато совпадает с определением
\eqref{eq: Gateaux Dstar derivative, division ring}.

Для $n=1$, $r_1(h_1)=a_0h_1a_1$. Это выражение совпадает
с выражением производной Гато в теореме
\ref{theorem: Gateaux differential, product over constant, fx=x, division ring}.

Пусть утверждение справедливо для $n-1$.
Справедливо равенство
\begin{equation}
r_n(h_1,x_2,...,x_n)=r_{n-1}(h_1,x_{[2},...,x_{n-1})x_{n]}a_n+r_{n-1}(x_2,...,x_n)h_1a_n
\label{eq: Gateaux derivative of monomial, n, division ring}
\end{equation}
Положим $x_2=...=x_n=x$. 
Согласно предположению индукции, из равенств
\eqref{eq: Gateaux derivative of monomial, algebraic definition, division ring},
\eqref{eq: Gateaux derivative of monomial, n, division ring}
следует
\[
r_n(h_1,x_2,...,x_n)=\partial p_{n-1}(x)(h_1)xa_n+p_{n-1}(x)h_1a_n
\]

Согласно теореме
\ref{theorem: Gateaux derivative of f(x)x, division ring}
\[
r_n(h_1,x_2,...,x_n)=\partial p_n(x)(h_1)
\]
что доказывает равенство
\eqref{eq: Gateaux derivative of monomial, algebraic definition, division ring}
для $k=1$.

Докажем теперь, что определение
\eqref{eq: Gateaux derivative of monomial, algebraic definition, division ring}
производной Гато совпадает с определением
\eqref{eq: Gateaux derivative of Order n, division ring} для $k>1$.

Пусть равенство
\eqref{eq: Gateaux derivative of monomial, algebraic definition, division ring}
верно для $k-1$.
Рассмотрим произвольное слагаемое многочлена $r_n(h_1,...,h_{k-1},x_k,...,x_n)$.
Отождествляя переменные $h_1$, ..., $h_{k-1}$
с элементами тела $D$, мы рассмотрим многочлен
\begin{equation}
R_{n-k}(x_k,...,x_n)=r_n(h_1,...,h_{k-1},x_k,...,x_n)
\label{eq: reduced polynom, division ring}
\end{equation}
Положим $P_{n-k}(x)=R_{n-k}(x_k,...,x_n)$, $x_k=...=x_n=x$.
Следовательно
\[
P_{n-k}(x)=\partial^{k-1} p_n(x)(h_1;...;h_{k-1})
\]
Согласно определению
\eqref{eq: Gateaux derivative of Order n, division ring}
производной Гато
\begin{align}
\partial P_{n-k}(x)(h_k)
=&\partial(\partial^{k-1} p_n(x)(h_1;...;h_{k-1}))(h_k)
\nonumber\\
=&\partial^k p_n(x)(h_1;...;h_{k-1};h_k)
\label{eq: Gateaux derivative of Order n, 1, division ring}
\end{align}
Согласно определению производной Гато
\eqref{eq: Gateaux derivative of monomial, algebraic definition, division ring}
\begin{equation}
\partial P_{n-k}(x)(h_k)=R_{n-k}(h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\label{eq: Gateaux derivative of monomial, algebraic definition, 1, division ring}
\end{equation}
Согласно определению \eqref{eq: reduced polynom, division ring},
из равенства
\eqref{eq: Gateaux derivative of monomial, algebraic definition, 1, division ring}
следует
\begin{equation}
\partial P_{n-k}(x)(h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\label{eq: Gateaux derivative of monomial, algebraic definition, 2, division ring}
\end{equation}
Из сравнения равенств \eqref{eq: Gateaux derivative of Order n, 1, division ring}
и \eqref{eq: Gateaux derivative of monomial, algebraic definition, 2, division ring}
следует
\[
\partial^k p_n(x)(h_1;...;h_k)=r_n(h_1,...,h_k,x_{k+1},...,x_n)\ \ \ x_{k+1}=x_n=x
\]
Следовательно равенсто
\eqref{eq: Gateaux derivative of monomial, algebraic definition, division ring}
верно для любых $k$ и $n$.

Утверждение теоремы доказано.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn equal 0, division ring}
Для произвольного $n\ge 0$ справедливо равенство
\begin{equation}
\label{eq: Gateaux derivative n1 of pn, division ring}
\partial^{n+1} p_n(x)(h_1;...;h_{n+1})=0
\end{equation}
\end{theorem}
\begin{proof}
Так как $p_0(x)=a_0$, $a_0\in D$, то при $n=0$ теорема является следствием
теоремы \ref{theorem: Gateaux differential of const, division ring}.
Пусть утверждение теоремы верно для $n-1$. Согласно теореме
\ref{theorem: Gateaux derivative of f(x)x, division ring}
при условии $f(x)=p_{n-1}(x)$ мы имеем
\begin{align*}
\partial^{n+1} p_n(x)(h_1;...;h_{n+1})
=&\partial^{n+1}(p_{n-1}(x)xa_n)(h_1;...;h_{n+1})
\\
=&\partial^{n+1} p_{n-1}(x)(h_1;...;h_m)xa_n
\\
+&\partial^n p_{n-1}(x)(h_1;...;h_{m-1})h_ma_n
\\
+&\partial^n p_{n-1}(x)(\widehat{h_1};...;h_{m-1};h_m)h_1a_n
+...
\\
+&\partial^{m-1} p_{n-1}(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}a_n
\end{align*}
Согласно предположению индукции все одночлены равны $0$.
\end{proof}

\begin{theorem}
\label{theorem: Gateaux derivative of pn equal 0, m less than n, division ring}
Если $m<n$, то справедливо равенство
\begin{equation}
\partial^m p_n(0)(h)=0
\label{eq: m Gateaux derivative of polinom pn, division ring}
\end{equation}
\end{theorem}
\begin{proof}
Для $n=1$ справедливо равенство
\[
\partial^0 p_1(0)=a_0xa_1=0
\]
Допустим, утверждение справедливо
для $n-1$. Тогда согласно теореме \ref{theorem: Gateaux derivative of f(x)x, division ring}
\begin{align*}
&\partial^m (p_{n-1}(x)xa_n)(h_1;...;h_m)
\\
=&\partial^m p_{n-1}(x)(h_1;...;h_m)xa_n
+\partial^{m-1} p_{n-1}(x)(h_1;...;h_{m-1})h_ma_n
\\
+&\partial^{m-1} p_{n-1}(x)(\widehat{h_1};...;h_{m-1};h_m)h_1a_n
+...
\\
+&\partial^{m-1} p_{n-1}(x)(h_1;...;\widehat{h_{m-1}};h_m)h_{m-1}a_n
\end{align*}
Первое слагаемое равно $0$ так как $x=0$.
Так как $m-1<n-1$, то
остальные слагаемые равны $0$ согласно предположению индукции.
Утверждение теоремы доказано.
\end{proof}

Если $h_1=...=h_n=h$, то мы положим
\[
\partial^nf(x)(h)=\partial^nf(x)(h_1;...;h_n)
\]
Эта запись не будет приводить к неоднозначности, так как по числу аргументов
ясно, о какой функции идёт речь.

\begin{theorem}
\label{theorem: n Gateaux derivative of polinom pn, division ring}
Для произвольного $n>0$ справедливо равенство
\begin{equation}
\partial^n p_n(x)(h)=n!p_n(h)
\label{eq: n Gateaux derivative of polinom pn, division ring}
\end{equation}
\end{theorem}
\begin{proof}
Для $n=1$ справедливо равенство
\[
\partial p_1(x)(h)=\partial (a_0xa_1)(h)=a_0ha_1=1!p_1(h)
\]
Допустим, утверждение справедливо
для $n-1$. Тогда согласно теореме \ref{theorem: Gateaux derivative of f(x)x, division ring}
\begin{align}
\label{eq: n Gateaux derivative of polinom pn, 1, division ring}
\partial^n p_n(x)(h)
=&\partial^n p_{n-1}(x)(h)xa_n
+\partial^{n-1} p_{n-1}(x)(h)ha_n
\\ \nonumber
+&...
+\partial^{n-1} p_{n-1}(x)(h)ha_n
\end{align}
Первое слагаемое равно $0$ согласно теореме
\ref{theorem: Gateaux derivative of pn equal 0, division ring}.
Остальные $n$ слагаемых равны, и согласно предположению индукции
из равенства \eqref{eq: n Gateaux derivative of polinom pn, 1, division ring}
следует
\[
\partial^n p_n(x)(h)
=n\partial^{n-1} p_{n-1}(x)(h)ha_n=n(n-1)!p_{n-1}(h)ha_n=n!p_n(h)
\]
Следовательно, утверждение теоремы верно для любого $n$.
\end{proof}

Пусть $p(x)$ - многочлен степени $n$.\footnote{Я рассматриваю
формулу Тейлора для многочлена по аналогии с
построением формулы Тейлора в \citeBib{Fihtengolts: Calculus volume 1}, с. 246.}
\[
p(x)=p_0+p_{1i_1}(x)+...+p_{ni_n}(x)
\]
Мы предполагаем сумму по индексу $i_k$, который нумерует слагаемые
степени $k$.
Согласно теоремам \ref{theorem: Gateaux derivative of pn equal 0, division ring},
\ref{theorem: Gateaux derivative of pn equal 0, m less than n, division ring},
\ref{theorem: n Gateaux derivative of polinom pn, division ring}
\[
\partial^k p(x)(h_1;...;h_k)=k!p_{ki_k}(x)
\]
Следовательно, мы можем записать
\[
p(x)=p_0+(1!)^{-1}\partial p(0)(x)+(2!)^{-1}\partial^2 p(0)(x)+...+(n!)^{-1}\partial^n p(0)(x)
\]
Это представление многочлена называется
\AddIndex{формулой Тейлора для многочлена}{Taylor polynomial, division ring}.
Если рассмотреть замену переменных $x=y-y_0$, то рассмотренное построение
остаётся верным для многочлена
\[
p(y)=p_0+p_{1i_1}(y-y_0)+...+p_{ni_n}(y-y_0)
\]
откуда следует
\[
p(y)=p_0+(1!)^{-1}\partial p(y_0)(y-y_0)+(2!)^{-1}\partial^2 p(y_0)(y-y_0)+...+(n!)^{-1}\partial^n p(y_0)(y-y_0)
\]

Предположим, что функция $f(x))$ в точке $x_0$ дифференцируема в смысле Гато
до любого порядка.\footnote{Я рассматриваю
построение ряда Тейлора по аналогии с
построением ряда Тейлора в \citeBib{Fihtengolts: Calculus volume 1}, с. 248, 249.}

\begin{theorem}
\label{theorem: n Gateaux derivative equal 0, division ring}
Если для функции $f(x)$ выполняется условие
\begin{equation}
f(x_0)=\partial f(x_0)(h)=...=\partial^n f(x_0)(h)=0
\label{eq: n Gateaux derivatives of function, division ring}
\end{equation}
то при $t\rightarrow 0$ выражение $f(x+th)$ является бесконечно малой порядка
выше $n$ по сравнению с $t$
\[
f(x_0+th)=o(t^n)
\]
\end{theorem}
\begin{proof}
При $n=1$ это утверждение следует из равенства
\eqref{eq: Gateaux differential of map, t, division ring}.

Пусть утверждение справедливо для $n-1$.
Для отображения
\[
f_1(x)=\partial f(x)(h)
\]
выполняется условие
\[
f_1(x_0)=\partial f_1(x_0)(h)=...=\partial^{n-1} f_1(x_0)(h)=0
\]
Согласно предположению индукции
\[
f_1(x_0+th)=o(t^{n-1})
\]
Тогда равенство \eqref{eq: Gateaux differential, representation, 2}
примет вид
\[
o(t^{n-1})=\lim_{t\rightarrow 0,\ t\in R}(t^{-1}f(x+th))
\]
Следовательно,
\[
f(x+th)=o(t^n)
\]
\end{proof}

Составим многочлен
\begin{equation}
\label{eq: Taylor polynomial, f(x), division ring}
p(x)=f(x_0)+(1!)^{-1}\partial f(x_0)(x-x_0)+...+(n!)^{-1}\partial^n f(x_0)(x-x_0)
\end{equation}
Согласно теореме \ref{theorem: n Gateaux derivative equal 0, division ring}
\[
f(x_0+t(x-x_0))-p(x_0+t(x-x_0))=o(t^n)
\]
Следовательно, полином $p(x)$ является хорошей апроксимацией отображения $f(x)$.

Если отображение $f(x)$ имеет производную Гато любого порядка, то переходя к пределу
$n\rightarrow\infty$, мы получим разложение в ряд
\[
f(x)=\sum_{n=0}^{\infty}(n!)^{-1}\partial^n f(x_0)(x-x_0)
\]
который называется \AddIndex{рядом Тейлора}{Taylor series, division ring}.

\section{Интеграл}

Понятие интеграла имеет разные аспекты. В этом разделе мы рассмотрим
интегрирование, как операцию, обратную дифференцированию.
По сути дела, мы рассмотрим процедуру решения обыкновенного дифференциального
уравнения
\[
\partial f(x)(h)=F(x;h)
\]

\begin{example}
Я начну с примера дифференциального уравнения над полем действительных чисел.
\begin{equation}
\label{eq: differential equation y=xx, 1, real number}
y'=3x^2
\end{equation}
\begin{equation}
\label{eq: differential equation y=xx, initial, real number}
\begin{matrix}
x_0=0&y_0=0
\end{matrix}
\end{equation}
Последовательно дифференцируя равенство \eqref{eq: differential equation y=xx, 1, real number},
мы получаем цепочку уравнений
\begin{align}
\label{eq: differential equation y=xx, 2, real number}
y''&=6x
\\
\label{eq: differential equation y=xx, 3, real number}
y'''&=6
\\
\label{eq: differential equation y=xx, 4, real number}
y^{(n)}&=0&n&>3
\end{align}
Из уравнений
\eqref{eq: differential equation y=xx, 1, real number},
\eqref{eq: differential equation y=xx, initial, real number},
\eqref{eq: differential equation y=xx, 2, real number},
\eqref{eq: differential equation y=xx, 3, real number},
\eqref{eq: differential equation y=xx, 4, real number}
следует разложение в ряд Тейлора
\[
y=x^3
\]
\qed
\end{example}

\begin{example}
Рассмотрим аналогичное уравнение над телом
\begin{equation}
\label{eq: differential equation y=xx, 1, division ring}
\partial (y)(h)=hx^2+xhx+x^2h
\end{equation}
\begin{equation}
\label{eq: differential equation y=xx, initial, division ring}
\begin{matrix}
x_0=0&y_0=0
\end{matrix}
\end{equation}
Последовательно дифференцируя равенство
\eqref{eq: differential equation y=xx, 1, division ring},
мы получаем цепочку уравнений
\ShowEq{differential equation y=xx, division ring}
Из уравнений
\eqref{eq: differential equation y=xx, 1, division ring},
\eqref{eq: differential equation y=xx, initial, division ring},
\eqref{eq: differential equation y=xx, 2, division ring},
\eqref{eq: differential equation y=xx, 3, division ring},
\eqref{eq: differential equation y=xx, 4, division ring}
следует разложение в ряд Тейлора
\[
y=x^3
\]
\qed
\end{example}

\begin{remark}
Дифференциальное уравнение
\begin{equation}
\label{eq: differential equation y=xx, 1, a, division ring}
\partial (y)(h)=3hx^2
\end{equation}
\begin{equation}
\label{eq: differential equation y=xx, initial, a, division ring}
\begin{matrix}
x_0=0&y_0=0
\end{matrix}
\end{equation}
так же приводит к решению $y=x^3$. Очевидно, что это
отображение не удовлетворяет дифференциальному уравнению.
Однако, вопреки теореме
\ref{theorem: Gateaux derivative of pn is simetric, m less than n, division ring}
вторая производная не
является симметричным многочленом. Это говорит о том,
что уравнение \eqref{eq: differential equation y=xx, 1, a, division ring}
не имеет решений.
\qed
\end{remark}

\begin{example}
\label{example: differential equation, additive function, division ring}
Очевидно, если функция удовлетворяет дифференциальному уравнению
\ShowEq{differential equation, additive function, division ring}
то вторая производная Гато
\[
\partial^2 f(x)(h_1;h_2)=0
\]
Следовательно, если задано начальное условие $y(0)=0$,
то дифференциальное уравнение
\eqref{eq: differential equation, additive function, division ring} имеет решение
\ShowEq{differential equation, additive function, solution, division ring}
\qed
\end{example}

\section{Экспонента}

В этом разделе мы рассмотрим одну из возможных моделей
построения экспоненты.

В поле мы можем определить экспоненту как решение дифференциального
уравнения
\ShowEq{exponent over field}
Очевидно, что мы не можем записать подобное уравнения для тела.
Однако мы можем воспользоваться равенством
\ShowEq{derivative over field}
Из уравнений
\eqref{eq: exponent over field}, \eqref{eq: derivative over field}
следует
\ShowEq{exponent derivative over field}
Это уравнение уже ближе к нашей цели,
однако остаётся открытым вопрос в каком порядке
мы должны перемножать $y$ и $h$.
Что бы ответить на этот вопрос, мы изменим запись уравнения
\ShowEq{exponent derivative over division ring}
Следовательно, наша задача - решить дифференциальное уравнение
\eqref{eq: exponent derivative over division ring}
при начальном условии $y(0)=1$.

Для формулировки и доказательства теоремы
\ref{theorem: exponent derivative n over division ring}
я введу следующее обозначение.
Пусть
\ShowEq{exponent derivative, transposition n}
перестановка кортежа переменных
\ShowEq{exponent transposition tuple 1}
Обозначим $p_{\sigma}(h_i)$ позицию, которую занимает
переменная $h_i$ в кортеже
\ShowEq{exponent transposition tuple 2}
Например, если перестановка $\sigma$ имеет вид
\ShowEq{exponent transposition tuple 3}
то следующие кортежи равны
\ShowEq{exponent transposition tuple 4}

\begin{theorem}
\label{theorem: exponent derivative n over division ring}
Производная Гато порядка $n$ функции $y$, удовлетворяющей дифференциальному уравнению
\eqref{eq: exponent derivative over division ring}
имеет вид
\ShowEq{exponent derivative n over division ring}
где сумма выполнена по перестановкам
\ShowEq{exponent derivative, transposition n}
множества переменных $y$, $h_1$, ..., $h_n$.
Перестановка $\sigma$ обладает следующими свойствами
\begin{enumerate}
\item Если существуют $i$, $j$, $i\ne j$, такие, что
$p_{\sigma}(h_i)$ располагается в произведении
\eqref{eq: exponent derivative n over division ring}
левее $p_{\sigma}(h_j)$ и $p_{\sigma}(h_j)$ располагается
левее $p_{\sigma}(y)$, то $i<j$.
\label{enumerate: exponent derivative, transposition n, left}
\item Если существуют $i$, $j$, $i\ne j$, такие, что
$p_{\sigma}(h_i)$ располагается в произведении
\eqref{eq: exponent derivative n over division ring}
правее $p_{\sigma}(h_j)$ и $p_{\sigma}(h_j)$ располагается
правее $p_{\sigma}(y)$, то $i>j$.
\label{enumerate: exponent derivative, transposition n, right}
\end{enumerate}
\end{theorem}
\begin{proof}
Мы докажем это утверждение индукцией.
Для $n=1$ утверждение верно, так как это дифференциальное уравнение
\eqref{eq: exponent derivative over division ring}.
Пусть утверждение верно для $n=k-1$.
Следовательно
\ShowEq{exponent derivative n=k-1 over division ring}
где сумма выполнена по перестановкам
\ShowEq{exponent derivative, transposition n=k-1}
множества переменных $y$, $h_1$, ..., $h_{k-1}$.
Перестановка $\sigma$ удовлетворяет условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.
Согласно определению
\eqref{eq: Gateaux derivative of Order n, division ring}
производная Гато` порядка $k$ имеет вид
\ShowEq{exponent derivative n=k over division ring, 1}
Из равенств
\eqref{eq: exponent derivative over division ring},
\eqref{eq: exponent derivative n=k over division ring, 1}
следует
\ShowEq{exponent derivative n=k over division ring, 2}
Нетрудно видеть, что произвольная перестановка $\sigma$
из суммы
\eqref{eq: exponent derivative n=k over division ring, 2}
порождает две перестановки
\ShowEq{exponent derivative, transposition n=k}
Из \eqref{eq: exponent derivative n=k over division ring, 2}
и \eqref{eq: exponent derivative, transposition n=k}
следует
\ShowEq{exponent derivative n=k over division ring, 3}
В выражении
\eqref{eq: exponent derivative n=k over division ring, 3}
$p_{\tau_1}(h_k)$ записано непосредственно перед $p_{\tau_1}(y)$.
Так как $k$ - самое большое значение индекса,
то перестановка $\tau_1$ удовлетворяет условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.
В выражении
\eqref{eq: exponent derivative n=k over division ring, 3}
$p_{\tau_2}(h_k)$ записано непосредственно после $p_{\tau_2}(y)$.
Так как $k$ - самое большое значение индекса,
то перестановка $\tau_2$ удовлетворяет условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.

Нам осталось показать, что в выражении
\eqref{eq: exponent derivative n=k over division ring, 3}
перечислены все перестановки $\tau$, удовлетворяющие условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме.
Так как $k$ - самый большой индекс, то согласно условиям
\eqref{enumerate: exponent derivative, transposition n, left},
\eqref{enumerate: exponent derivative, transposition n, right},
сформулированным в теореме, $\tau(h_k)$
записано непосредственно перед или непосредственно после $\tau(y)$.
Следовательно, любая перестановка $\tau$ имеет
либо вид $\tau_1$, либо вид $\tau_2$.
Пользуясь равенством
\eqref{eq: exponent derivative, transposition n=k},
мы можем для заданной перестановки $\tau$ найти соответствующую
перестановку $\sigma$.
Следовательно, утверждение теоремы верно для $n=k$.
Теорема доказана.
\end{proof}

\begin{theorem}
Решением дифференциального уравнения
\eqref{eq: exponent derivative over division ring}
при начальном условии $y(0)=1$
является экспонента
\ShowEq{exponent over division ring}
которая имеет следующее разложение в ряд Тейлора
\ShowEq{exponent Taylor series over division ring}
\end{theorem}
\begin{proof}
Производная Гато порядка $n$ содержит $2^n$ слагаемых.
Действительно, производная Гато порядка $1$ содержит $2$ слагаемых,
и каждое дифференцирование увеличивает число слагаемых вдвое.
Из начального условия $y(0)=1$ и теоремы
\ref{theorem: exponent derivative n over division ring}
следует, что производная Гато порядка $n$ искомого решения имеет вид
\ShowEq{exponent derivative n over division ring, x=0}
Из равенства
\eqref{eq: exponent derivative n over division ring, x=0}
следует разложение
\eqref{eq: exponent Taylor series over division ring}.
в ряд Тейлора.
\end{proof}

\begin{theorem}
\label{theorem: exponent of sum}
Равенство
\ShowEq{exponent of sum}
справедливо тогда и только тогда, когда
\ShowEq{exponent of sum, 1}
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно рассмотреть ряды Тейлора
\ShowEq{exponent a b a+b}
Перемножим выражения
\eqref{eq: exponent a} и \eqref{eq: exponent b}.
Сумма одночленов порядка $3$ имеет вид
\ShowEq{exponent ab 3}
и не совпадает, вообще говоря, с выражением
\ShowEq{exponent a+b 3}
Доказательство утверждения, что
\eqref{eq: exponent of sum} следует из \eqref{eq: exponent of sum, 1}
тривиально.
\end{proof}

Смысл теоремы \ref{theorem: exponent of sum}
становится яснее, если мы вспомним, что существует две
модели построения экспоненты. Первая модель - это
решение дифференциального уравнения
\eqref{eq: exponent derivative over division ring}.
Вторая - это изучение однопараметрической группы преобразований.
В случае поля обе модели приводят к одной и той же функции.
Я не могу этого утверждать сейчас в общем случае. Это вопрос отдельного
исследования. Но если вспомнить, что кватернион является аналогом
преобразования трёхмерного пространства, то утверждение теоремы
становится очевидным.


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index{texLinearMap}%1%0
   {$1$-\drc форма}%
   {1-drc form, vector spaces}%
\SetIndexSpace%
\Index{texBundleRelation}%2%0
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index{texBiring}%A%0
   {$(^a_b)$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index{texBiring}%A%0
   {$(^a_b)$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant}%
\Index{texSecondDifferential}%A%0
   {$A$\Hyph значная функция}%
   {A valued function}%
\SetIndexSpace%
\Index{texBiring}%C%0
   {\subs строка матрицы}%
   {c row}%
\Index{texVectorSpace}%C%0
   {\CR матричная группа}%
   {cr-matrix group}%
\Index{texBiring}%C%0
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index{texBiring}%C%0
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index{texBiring}%C%0
   {\CR степень}%
   {cr power}%
\Index{texVectorSpace}%C%0
   {\crd векторное пространство}%
   {crd vector space}%
\Index{texBiring}%C%0
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index{texSecondDifferential}%D%0
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Index{texSecondDifferential}%D%0
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index{texLinearMap}%D%0
   {$D$\hyph векторное пространство}%
   {D vector space}%
\Index{texVectorSpace}%D%0
   {\dcr базис векторного пространства \subs строк}%
   {dcr basis, c rows vector space}%
\Index{texVectorSpace}%D%0
   {\dcr вектор}%
   {dcr vector}%
\Index{texVectorSpace}%D%0
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index{texVectorSpace}%D%0
   {\dcr векторное пространство \subs строк}%
   {subs rows dcr vector space}%
\Index{texVectorField}%D%0
   {\Drc  линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index{texVectorSpace}%D%0
   {\drc  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index{texVectorSpace}%D%0
   {\drc автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index{texAffineSpace}%D%0
   {\drc аффинное пространство}%
   {drc affine space}%
\Index{texVectorSpace}%D%0
   {\drc базис в векторном пространстве}%
   {drc basis, vector space}%
\Index{texVectorSpace}%D%0
   {\drc базис в векторном пространстве \sups строк}%
   {drc basis, r rows vector space}%
\Index{texVectorField}%D%0
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index{texVectorSpace}%D%0
   {\drc вектор}%
   {drc vector}%
\Index{texVectorSpace}%D%0
   {\drc векторное пространство}%
   {drc vector space}%
\Index{texVectorSpace}%D%0
   {\drc векторное пространство \sups строк}%
   {sups rows drc vector space}%
\Index{texSecondDifferential}%D%0
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index{texVectorSpace}%D%0
   {\drc изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index{texVectorSpace}%D%0
   {\drc линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index{texVectorField}%D%0
   {\Drc линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index{texVectorSpace}%D%0
   {\drc линейно независимые векторы}%
   {linearly independent, vector space}%
\Index{texDrcMorphism}%D%0
   {\drc линейное отображение векторных пространств}%
   {drc linear map of vector spaces}%
\Index{texVectorField}%D%0
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index{texDrcBasis}%D%0
   {\drc линейным \sT представление группы}%
   {drc linear starT representation of group}%
\Index{texSecondDifferential}%D%0
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Index{texVectorField}%D%0
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index{texVectorSpace}%D%0
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index{texVectorField}%D%0
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index{texLinearMap}%D%0
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Index{texVectorField}%D%0
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index{texVectorSpace}%D%0
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index{texVectorField}%D%0
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index{texDifferential}%D%0
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index{texFrechet}%D%0
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index{texSecondDifferential}%D%0
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index{texLinearMap}%D%0
   {\rcd базис, дуальный \drc базису в векторном пространстве}%
   {basis dual to basis, drc vector space}%
\SetIndexSpace%
\Index{texELie}%E%0
   {enhanced Lie group}%
   {enhanced Lie group}%
\Index{texDiffEq}%E%0
   {essential parameters}%
   {essential parameters}%
\SetIndexSpace%
\Index{texRefernceFrame}%G%0
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index{texBasis}%G%0
   {\Gbasis\ векторного пространства}%
   {G-basis}%
\Index{texBasis}%G%0
   {\Gcoords ы базиса}%
   {G-coordinates}%
\Index{texBasis}%G%0
   {\Gspace о}%
   {GSpace}%
\SetIndexSpace%
\Index{texPolyvector}%M%0
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\Index{texPolyvector}%M%0
   {$m$\Hyph вектор}%
   {m-vector}%
\SetIndexSpace%
\Index{texBundleRelation}%N%0
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index{texBiring}%R%0
   {\sups строка матрицы}%
   {r row}%
\Index{texVectorSpace}%R%0
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index{texVectorSpace}%R%0
   {\RC главный минор}%
   {RC-major minor}%
\Index{texBiring}%R%0
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index{texVectorSpace}%R%0
   {\RC матричная группа}%
   {rc-matrix group}%
\Index{texVectorSpace}%R%0
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index{texBiring}%R%0
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index{texBiring}%R%0
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index{texVectorSpace}%R%0
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index{texBiring}%R%0
   {\RC степень}%
   {rc power}%
\Index{texVectorSpace}%R%0
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index{texDrcBasis}%R%0
   {\rcd представление группы}%
   {rcd linear representation of group}%
\Index{texVectorSpace}%R%0
   {$R\star$\Hyph модуль}%
   {Rstar-module}%
\Index{texBiring}%R%0
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index{texDrcMorphism}%S%0
   {$(S\RCstar,T\RCstar)$\Hyph линейное отображение векторных пространств}%
   {src trc linear map of vector spaces}%
\Index{texVectorField}%S%0
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index{texLinearMap}%S%0
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%
\Index{texDifferential}%S%0
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index{texLinearMap}%S%0
   {$\star D$\Hyph произведением \drc линейного отображения $A$ на скаляр}%
   {starD product of drc linear map over scalar}%
\Index{texVectorSpace}%S%0
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index{texVectorSpace}%S%0
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index{texTstarRepresentation}%S%0
   {\sT сдвиг}%
   {starT shift}%
\Index{texFiberedGroup}%S%0
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\Index{texTstarMorphism}%S%0
   {\sT представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {starT representation of algebra}%
\Index{texFiberedAlgebra}%S%0
   {\sT представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {starT representation of fibered F-algebra}%
\Index{texFiberedGroup}%S%0
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index{texTstarMorphism}%S%0
   {\sT преобразование}%
   {starT transformation}%
\Index{texFiberedAlgebra}%S%0
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\SetIndexSpace%
\Index{texVectorSpace}%T%0
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index{texVectorSpace}%T%0
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index{texTstarRepresentation}%T%0
   {\Ts сдвиг}%
   {Tstar shift}%
\Index{texTstarMorphism}%T%0
   {\Ts представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {Tstar representation of algebra}%
\Index{texFiberedAlgebra}%T%0
   {\Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {Tstar representation of fibered F-algebra}%
\Index{texTstarMorphism}%T%0
   {\Ts преобразование}%
   {Tstar transformation}%
\Index{texFiberedAlgebra}%T%0
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\SetIndexSpace%
\Index{texTstarMorphism}%А%0
   {автоморфизм представления $f$}%
   {automorphism of representation f}%
\Index{texAffine}%А%0
   {автопараллельная кривая}%
   {auto parallel line}%
\Index{texAdditiveMap}%А%0
   {аддитивное отображение $D$\Hyph векторных пространств}%
   {additive map of D vector spaces}%
\Index{texAdditiveMap}%А%0
   {аддитивное отображение кольца}%
   {Additive map of Ring}%
\Index{texRingAdditiveMap}%А%0
   {аддитивное отображение тела, порождённое отображением $G$}%
   {additive map generated by map, division ring}%
\Index{texDrcBasis}%А%0
   {активное \sT представление}%
   {active representation, vector space}%
\Index{texBasis}%А%0
   {активное представление}%
   {active representation}%
\Index{texBasis}%А%0
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index{texDrcBasis}%А%0
   {активное преобразование на множестве \drc базисов}%
   {active transformation, vector space}%
\Index{texAdditiveMap}%А%0
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index{texLie}%А%0
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index{texBiring}%А%0
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index{texFiberedGroup}%А%0
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index{texBundleRelation}%А%0
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index{texFiberedAlgebra}%А%0
   {арность операции}%
   {arity of operation}%
\Index{texBasis}%А%0
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index{texBasis}%А%0
   {аффинный базис}%
   {Affine Basis}%
\Index{texAffineSpace}%А%0
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index{texPolymodule}%Б%0
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index{texBundle}%Б%0
   {база отображения}%
   {base of map}%
\Index{texBundleRelation}%Б%0
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index{texBasis}%Б%0
   {базис векторного пространства}%
   {Basis}%
\Index{texLieRepresentation}%Б%0
   {базовый вектор \sT представления}%
   {basis vector of starT representation}%
\Index{texLieRepresentation}%Б%0
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation}%
\Index{texLie}%Б%0
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index{texTowerRepresentation}%Б%0
   {башня представлений $\mathfrak{F}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index{texFiberedMorphism}%Б%0
   {башня расслоений}%
   {tower of bundles}%
\Index{texLieRepresentation}%Б%0
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index{texBiring}%Б%0
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index{texDiffProperty}%В%0
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index{texRepresentation}%В%0
   {вектор\hyph столбец}%
   {column vector}%
\Index{texFiberedAlgebra}%В%0
   {векторное расслоение}%
   {vector bundle}%
\Index{texNewton}%В%0
   {векторный потенциал}%
   {vector potential}%
\Index{texRepresentation}%В%0
   {вектор\hyph строка}%
   {row vector}%
\Index{texDiffEq}%В%0
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index{texNewton}%В%0
   {второй закон Ньютона}%
   {Second Newton law}%
\Index{texAdditiveMap}%В%0
   {вырожденное аддитивное отображение $D$\Hyph векторного пространства}%
   {singular additive map, D vector space}%
\Index{texAdditiveMap}%В%0
   {вырожденное аддитивное отображение тела}%
   {singular additive map, division ring}%
\SetIndexSpace%
\Index{texBasis}%Г%0
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%
\Index{texBasis}%Г%0
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Index{texDrcBasis}%Г%0
   {геометрический объект в координатном представлении, определённом в \drc векторном пространстве}%
   {geometrical object, coordinate vector space}%
\Index{texDrcBasis}%Г%0
   {геометрический объект типа $A$}%
   {geometrical object of type A, vector space}%
\Index{texBasis}%Г%0
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometrical object of type A, vector space}%
\Index{texDrcBasis}%Г%0
   {геометрический объект, определённый в \drc векторном пространстве}%
   {geometrical object, vector space}%
\Index{texRefernceFrame}%Г%0
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index{texRefernceFrame}%Г%0
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index{texFiberedAlgebra}%Г%0
   {гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Index{texFiberedGroup}%Г%0
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index{texAffineSpace}%Г%0
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%0
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%0
   {группа симметрии}%
   {symmetry group}%
\Index{texDrcBasis}%Г%0
   {группа симметрии}%
   {SymmetryGroup}%
\Index{texTstarRepresentation}%Г%0
   {группа стабилизации}%
   {stability group}%
\Index{texGroupRing}%Г%0
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index{texAffineSpace}%Д%0
   {движение на многообразии базисов}%
   {movement transformation}%
\Index{texBundle}%Д%0
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index{texBundle}%Д%0
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power A of bundle B}%
\Index{texCartesian}%Д%0
   {декартова степень $n$ расслоения $\mathcal{E}$}%
   {Cartesian power n of bundle E}%
\Index{texCartesian}%Д%0
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index{texCartesian}%Д%0
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index{texBundleRelation}%Д%0
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index{texBundleRelation}%Д%0
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index{texSecondDifferential}%Д%0
   {дифференциал Гато второго порядка отображения $f$}%
   {Gateaux differential of Second Order, division ring}%
\Index{texSecondDifferential}%Д%0
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Index{texSecondDifferential}%Д%0
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Index{texDifferential}%Д%0
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Index{texLinearMap}%Д%0
   {дуальное пространство к \drc векторному пространству}%
   {dual space of drc vector space}%
\SetIndexSpace%
\Index{texDifferential}%Е%0
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\SetIndexSpace%
\Index{texDrcMorphism}%З%0
   {закон ассоциативности для \drc линейных отображений векторных пространств}%
   {associative law for drc linear maps of vector spaces}%
\Index{texVectorField}%З%0
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index{texVectorSpace}%З%0
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index{texVectorField}%З%0
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index{texTstarRepresentation}%З%0
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index{texTstarRepresentation}%З%0
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index{texLinearMap}%З%0
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index{texBundleRelation}%З%0
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index{texVectorSpace}%З%0
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index{texVectorField}%З%0
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index{texVectorSpace}%З%0
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index{texVectorField}%З%0
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\SetIndexSpace%
\Index{texFiberedAlgebra}%И%0
   {изоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {isomorphism of fibered F-algebras}%
\Index{texLinearLie}%И%0
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index{texHomotopy}%К%0
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index{texTstarMorphism}%К%0
   {категория \Ts представлений $\mathfrak{F}$\Hyph алгебры $A$}%
   {category of Tstar representations of F algebra}%
\Index{texTstarMorphism}%К%0
   {категория \Ts представлений $\mathfrak{F}$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of F algebra from category}%
\Index{texBundleRelation}%К%0
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index{texBundleRelation}%К%0
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index{texBasis}%К%0
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index{texAffineSpace}%К%0
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index{texAffineSpace}%К%0
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index{texBasis}%К%0
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index{texTstarRepresentation}%К%0
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index{texFiberedGroup}%К%0
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index{texTstarRepresentation}%К%0
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index{texFiberedGroup}%К%0
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index{texDivisionRing}%К%0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index{texDivisionRing}%К%0
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index{texBundleRelation}%К%0
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index{texBundle}%К%0
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index{texAdditiveMap}%К%0
   {компонента линейного отображения $D$\Hyph векторного пространчства}%
   {component of linear map, D vector space}%
\Index{texRingAdditiveMap}%К%0
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Index{texAdditiveMap}%К%0
   {компонента полиаддитивного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Index{texAdditiveMap}%К%0
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Index{texSecondDifferential}%К%0
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Index{texSecondDifferential}%К%0
   {компонента производной Гато второго порядка отображения тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Index{texDifferential}%К%0
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Index{texSecondDifferential}%К%0
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Index{texFiberedGroup}%К%0
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index{texTstarRepresentation}%К%0
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index{texTstarRepresentation}%К%0
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index{texFiberedGroup}%К%0
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index{texVectorSpace}%К%0
   {координатная матрица вектора в \drc базисе}%
   {coordinate matrix of vector in drc basis}%
\Index{texVectorField}%К%0
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index{texVectorSpace}%К%0
   {координатная матрица множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\Index{texVectorSpace}%К%0
   {координатная матрица множества векторов в векторном пространстве \drc строк}%
   {coordinate matrix of set of vectors, drc vector space}%
\Index{texRefernceFrame}%К%0
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index{texVectorSpace}%К%0
   {координатное \drc векторное пространство}%
   {coordinate drc vector space}%
\Index{texVectorField}%К%0
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index{texBasis}%К%0
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index{texDrcBasis}%К%0
   {координатное представление в \drc векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%0
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texVectorSpace}%К%0
   {координатный \drc изоморфизм}%
   {coordinate drc isomorphism}%
\Index{texBasis}%К%0
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%0
   {координаты вектора в \drc базисе}%
   {coordinates of vector in drc basis}%
\Index{texVectorField}%К%0
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index{texBasis}%К%0
   {координаты геометрического объекта}%
   {coordinates of geometrical object, vector space}%
\Index{texDrcBasis}%К%0
   {координаты геометрического объекта в \drc векторном пространстве}%
   {coordinates of geometrical object, vector space}%
\Index{texDrcBasis}%К%0
   {координаты геометрического объекта в координатном \drc векторном пространстве}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texBasis}%К%0
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texVectorSpace}%К%0
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index{texVectorSpace}%К%0
   {координаты множества векторов в \drc векторном пространстве}%
   {coordinates of set of vectors, drc vector space}%
\Index{texDrcBasis}%К%0
   {координаты представления}%
   {coordinates of representation}%
\Index{texBasis}%К%0
   {координаты представления}%
   {coordinates of representation}%
\Index{texPolyvector}%К%0
   {косое произведение векторов}%
   {skew product of vectors}%
\Index{texAffine}%К%0
   {кривизна Картана}%
   {Cartan curvature}%
\SetIndexSpace%
\Index{texVectorSpace}%Л%0
   {левое векторное пространство}%
   {left vector space}%
\Index{texLie}%Л%0
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index{texRepresentation}%Л%0
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index{texRepresentation}%Л%0
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index{texTstarMorphism}%Л%0
   {левостороннее представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {left-side representation of algebra}%
\Index{texFiberedAlgebra}%Л%0
   {левостороннее представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {left-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%Л%0
   {левостороннее преобразование}%
   {left-side transformation}%
\Index{texFiberedAlgebra}%Л%0
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index{texLie}%Л%0
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index{texVectorSpace}%Л%0
   {левый модуль}%
   {left module}%
\Index{texTstarRepresentation}%Л%0
   {левый сдвиг на группе}%
   {left shift}%
\Index{texRepresentation}%Л%0
   {левый сдвиг на группе}%
   {left shift, group}%
\Index{texFiberedGroup}%Л%0
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index{texAdditiveMap}%Л%0
   {линейное отображение $D$\Hyph векторных пространств}%
   {linear map, vector space}%
\Index{texAdditiveMap}%Л%0
   {линейное отображение $D$\Hyph векторных пространств над полем $F$}%
   {linear map over field, vector space}%
\Index{texRingAdditiveMap}%Л%0
   {линейное отображение тела}%
   {linear map, division ring}%
\Index{texRepresentation}%Л%0
   {линейное представление группы}%
   {linear representation of group}%
\Index{texBundle}%Л%0
   {лифт отображения}%
   {lift of map}%
\Index{texBundleRelation}%Л%0
   {лифт соответствия}%
   {lift of correspondence}%
\Index{texRefernceFrame}%Л%0
   {локальная система отсчёта}%
   {local reference frame}%
\Index{texBundle}%Л%0
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index{texBundle}%Л%0
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index{texTstarRepresentation}%М%0
   {малая группа}%
   {little group}%
\Index{texDrcMorphism}%М%0
   {матрица \drc линейного отображения}%
   {matrix of drc linear map}%
\Index{texVectorField}%М%0
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index{texGeomObject}%М%0
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index{texDrcBasis}%М%0
   {многообразие базисов \drc векторного пространства}%
   {basis manifold of vector space}%
\Index{texBasis}%М%0
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index{texAffineSpace}%М%0
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index{texBasis}%М%0
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index{texBasis}%М%0
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index{texAffineSpace}%М%0
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index{texAffineSpace}%М%0
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texBasis}%М%0
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texDrcReferenceFrame}%М%0
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index{texFiberedMorphism}%М%0
   {морфизм \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {morphism of representations of fibered F algebra}%
\Index{texTowerRepresentation}%М%0
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index{texTstarMorphism}%М%0
   {морфизм представлений $\mathfrak{F}$\Hyph алгебры}%
   {morphism of representations of F algebra}%
\Index{texTstarMorphism}%М%0
   {морфизм представлений $\mathfrak{F}$\Hyph алгебры в $\mathfrak{H}$\Hyph алгебре}%
   {morphism of representations of F algebra in H algebra}%
\Index{texTstarMorphism}%М%0
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index{texFiberedMorphism}%М%0
   {морфизм расслоенных \Ts представлений из $\mathcal{F}$ в $\mathcal{G}$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index{texAdditiveMap}%Н%0
   {направление в $D$\Hyph векторном пространстве $\Vector V$ над полем $P$}%
   {direction over field, D vector space}%
\Index{texAdditiveMap}%Н%0
   {направление в теле $D$ над коммутативным кольцом $P$}%
   {direction over commutative ring, ring}%
\Index{texVectorSpace}%Н%0
   {невырожденная система \drc линейных уравнений}%
   {nonsingular system of linear equations}%
\Index{texRepresentation}%Н%0
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index{texRefernceFrame}%Н%0
   {неголономная координата}%
   {anholonomic coordinate}%
\Index{texRefernceFrame}%Н%0
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index{texRefernceFrame}%Н%0
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index{texRefernceFrame}%Н%0
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index{texGeomObject}%Н%0
   {неметричность}%
   {nonmetricity}%
\Index{texDifferential}%Н%0
   {непрерывная функция тела}%
   {continuous function, division ring}%
\Index{texBundleRelation}%Н%0
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index{texAdditiveMap}%Н%0
   {норма кватерниона}%
   {norm of quaternion}%
\Index{texSecondDifferential}%Н%0
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index{texDifferential}%Н%0
   {норма на теле}%
   {absolute value on division ring}%
\Index{texDifferential}%Н%0
   {норма отображения  тела}%
   {norm of map, division ring}%
\Index{texSecondDifferential}%Н%0
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Index{texSecondDifferential}%Н%0
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index{texDifferential}%Н%0
   {нормированное тело}%
   {valued division ring}%
\SetIndexSpace%
\Index{texRingAdditiveMap}%О%0
   {образующая аддитивного отображения}%
   {generator of additive map, division ring}%
\Index{texBundleRelation}%О%0
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index{texBundleRelation}%О%0
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index{texBiring}%О%0
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index{texRefernceFrame}%О%0
   {объект неголономности}%
   {anholonomity object}%
\Index{texSecondDifferential}%О%0
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index{texTstarRepresentation}%О%0
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texRepresentation}%О%0
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texFiberedGroup}%О%0
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index{texTstarMorphism}%О%0
   {однотранзитивное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index{texRepresentation}%О%0
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index{texFiberedAlgebra}%О%0
   {однотранзитивное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {single transitive representation of fibered F-algebra}%
\Index{texFiberedAlgebra}%О%0
   {операция на расслоении}%
   {operation on bundle}%
\Index{texLie}%О%0
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index{texLie}%О%0
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index{texBiring}%О%0
   {определитель матрицы}%
   {determinant}%
\Index{texTstarRepresentation}%О%0
   {орбита \Ts представления группы}%
   {orbit of representation of group}%
\Index{texRepresentation}%О%0
   {орбита представления группы}%
   {orbit of representation of group}%
\Index{texFiberedGroup}%О%0
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index{texBasis}%О%0
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index{texAffineSpace}%О%0
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index{texTidal}%О%0
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index{texAdditiveMap}%О%0
   {отображение $D$\Hyph векторного пространства, мультипликативное над полем}%
   {map multiplicative over field, D vector space}%
\Index{texAdditiveMap}%О%0
   {отображение $D$\Hyph векторного пространства, проективное над полем}%
   {map projective over field, D vector space}%
\Index{texAdditiveMap}%О%0
   {отображение колец $R_1$, ..., $R_n$, полилинейное над коммутативным кольцом $P$}%
   {map polylinear over commutative ring, ring}%
\Index{texAdditiveMap}%О%0
   {отображение кольца $D$, линейное над коммутативным кольцом $F$}%
   {linear map over commutative ring, ring}%
\Index{texAdditiveMap}%О%0
   {отображение кольца, мультипликативное над коммутативным кольцом}%
   {map multiplicative over commutative ring, ring}%
\Index{texAdditiveMap}%О%0
   {отображение кольца, проективное над коммутативным кольцом}%
   {map projective over commutative ring, ring}%
\Index{texAdditiveMap}%О%0
   {отображение полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index{texDrcReferenceFrame}%О%0
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\SetIndexSpace%
\Index{texGeomObject}%П%0
   {параллелограмм}%
   {parallelogram}%
\Index{texTstarRepresentation}%П%0
   {парные представления группы}%
   {twin representations of group}%
\Index{texFiberedGroup}%П%0
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index{texLinearMap}%П%0
   {парные представления тела}%
   {twin representations of division ring}%
\Index{texDrcBasis}%П%0
   {пассивное \Ts представление}%
   {passive representation}%
\Index{texBasis}%П%0
   {пассивное представление}%
   {passive representation}%
\Index{texBasis}%П%0
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index{texDrcBasis}%П%0
   {пассивное преобразование на множестве \drc базисов}%
   {passive transformation, vector space}%
\Index{texNewton}%П%0
   {первый закон Ньютона}%
   {First Newton law}%
\Index{texAffine}%П%0
   {перенос Картана}%
   {Cartan transport}%
\Index{texAffine}%П%0
   {перенос Френе}%
   {Frenet transport}%
\Index{texBundle}%П%0
   {подрасслоение}%
   {subbundle}%
\Index{texVectorField}%П%0
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index{texAdditiveMap}%П%0
   {полиаддитивное отображение $(n)$\hyph $D$\hyph векторных пространств}%
   {polyadditive map of D vector spaces}%
\Index{texRingAdditiveMap}%П%0
   {полиаддитивное отображение колец}%
   {polyadditive map of rings}%
\Index{texPolyvector}%П%0
   {поливектор}%
   {polyvector}%
\Index{texRingAdditiveMap}%П%0
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric, division ring}%
\Index{texRingAdditiveMap}%П%0
   {полилинейное отображение колец}%
   {polylinear map of rings}%
\Index{texRingAdditiveMap}%П%0
   {полилинейное симметричное отображение}%
   {polylinear map symmetric, division ring}%
\Index{texDiffEq}%П%0
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index{texDifferential}%П%0
   {полное тело}%
   {complete division ring}%
\Index{texEuclideanSpace}%П%0
   {положительно определённое биаддитивное отображение}%
   {positive definite biadditive map}%
\Index{texDifferential}%П%0
   {последовательность Коши в нормированное теле}%
   {Cauchy sequence, valued division ring}%
\Index{texNewton}%П%0
   {потенциальная энергия}%
   {potential energy}%
\Index{texVectorSpace}%П%0
   {правое векторное пространство}%
   {right vector space}%
\Index{texLie}%П%0
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index{texRepresentation}%П%0
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index{texRepresentation}%П%0
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index{texTstarMorphism}%П%0
   {правостороннее представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {right-side representation of algebra}%
\Index{texFiberedAlgebra}%П%0
   {правостороннее представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {right-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%П%0
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texRepresentation}%П%0
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texLie}%П%0
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index{texVectorSpace}%П%0
   {правый модуль}%
   {right module}%
\Index{texTstarRepresentation}%П%0
   {правый сдвиг на группе}%
   {right shift}%
\Index{texRepresentation}%П%0
   {правый сдвиг на группе}%
   {right shift, group}%
\Index{texDifferential}%П%0
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Index{texBundleRelation}%П%0
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index{texBundleRelation}%П%0
   {предел фильтра}%
   {limit of filter}%
\Index{texBundleRelation}%П%0
   {предельное множество фильтра}%
   {limit set of filter}%
\Index{texBasis}%П%0
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texDrcBasis}%П%0
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texTowerRepresentation}%П%0
   {представление $\mathfrak{F}$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of F algebra in category}%
\Index{texTstarMorphism}%П%0
   {представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {representation of algebra}%
\Index{texRepresentation}%П%0
   {представление группы}%
   {representation of group}%
\Index{texRefernceFrame}%П%0
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index{texTstarMorphism}%П%0
   {преобразование множества}%
   {transformation of set}%
\Index{texFiberedAlgebra}%П%0
   {преобразование расслоения}%
   {transformation of bundle}%
\Index{texTstarMorphism}%П%0
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index{texCartesian}%П%0
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index{texCartesian}%П%0
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index{texBundleRelation}%П%0
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {reduced fibered correspondence from A to B}%
\Index{texBundleRelation}%П%0
   {приведенное расслоенное соответствие в $\mathcal{A}$}%
   {reduced fibered correspondence in A}%
\Index{texBiring}%П%0
   {приводимое бикольцо}%
   {reducible biring}%
\Index{texBiring}%П%0
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index{texBiring}%П%0
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index{texDrcBasis}%П%0
   {принцип инвариантности}%
   {invariance principle}%
\Index{texBasis}%П%0
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index{texBundleRelation}%П%0
   {продолжение соответствия}%
   {extension of correspondence}%
\Index{texBundle}%П%0
   {проекция расслоения $\mathcal{E}$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index{texDrcBasis}%П%0
   {произведение геометрического объекта и константы}%
   {product of geometrical object and constant}%
\Index{texBasis}%П%0
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometrical object and constant, vector space}%
\Index{texPolymodule}%П%0
   {произведение групп}%
   {product of groups}%
\Index{texTstarMorphism}%П%0
   {произведение морфизмов представлений $\mathfrak{F}$\Hyph алгебры}%
   {product of morphisms of representations of F algebra}%
\Index{texVectorField}%П%0
   {произведение морфизмов \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {product of morphisms of representations of fibered F algebra}%
\Index{texBundleRelation}%П%0
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index{texBundleRelation}%П%0
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index{texAdditiveMap}%П%0
   {произведением объектов в категории}%
   {product of objects in category}%
\Index{texDifferential}%П%0
   {производная Гато второго порядка отображения $f$}%
   {Gateaux derivative of Second Order, division ring}%
\Index{texDifferential}%П%0
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Index{texSecondDifferential}%П%0
   {производная Гато отображения $\Vector f$ нормированого $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Index{texSecondDifferential}%П%0
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Index{texSecondDifferential}%П%0
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Index{texSecondDifferential}%П%0
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Index{texAffine}%П%0
   {производная Картана}%
   {Cartan derivative}%
\Index{texDiffProperty}%П%0
   {производная Ли}%
   {Lie derivative}%
\Index{texAffine}%П%0
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index{texAffine}%П%0
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index{texPolyvector}%П%0
   {простой поливектор}%
   {simple polyvector}%
\Index{texTstarRepresentation}%П%0
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index{texCartesian}%П%0
   {пространство отображений}%
   {mapping space}%
\Index{texBundleRelation}%П%0
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index{texLieRepresentation}%П%0
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index{texPolymodule}%П%0
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index{texPolymodule}%П%0
   {прямое произведение \drc векторных пространств}%
   {direct product, drc vector space}%
\Index{texTstarRepresentation}%П%0
   {прямое произведение \Ts представлений группы}%
   {direct product of representations of group}%
\Index{texRepresentation}%П%0
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index{texFiberedGroup}%П%0
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index{texPolymodule}%П%0
   {прямое произведение тел}%
   {direct product of division rings}%
\Index{texRefernceFrame}%П%0
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index{texVectorSpace}%Р%0
   {размерность \drc векторного пространства}%
   {dimension of vector space}%
\Index{texFiberedMorphism}%Р%0
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index{texFiberedMorphism}%Р%0
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index{texFiberedAlgebra}%Р%0
   {расслоенная $\mathfrak{F}$\Hyph алгебра}%
   {fibered F-algebra}%
\Index{texFiberedAlgebra}%Р%0
   {расслоенная $\mathfrak{F}$\Hyph подалгебра}%
   {fibered F-subalgebra}%
\Index{texFiberedAlgebra}%Р%0
   {расслоенная группа}%
   {fibered group}%
\Index{texFiberedMorphism}%Р%0
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index{texFiberedMorphism}%Р%0
   {расслоенная малая группа}%
   {fibered little group}%
\Index{texBundleRelation}%Р%0
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index{texBundleRelation}%Р%0
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index{texBundleRelation}%Р%0
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index{texFiberedAlgebra}%Р%0
   {расслоенное кольцо}%
   {fibered ring}%
\Index{texBundle}%Р%0
   {расслоенное подмножество}%
   {fibered subset}%
\Index{texBundleRelation}%Р%0
   {расслоенное соответствие в $\mathcal{A}$}%
   {fibered correspondence in A}%
\Index{texBundleRelation}%Р%0
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index{texBundleRelation}%Р%0
   {расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered correspondence from A to B}%
\Index{texFiberedMorphism}%Р%0
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index{texVectorField}%Р%0
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index{texBundle}%Р%0
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Index{texFiberedMorphism}%Р%0
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index{texVectorSpace}%Р%0
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index{texVectorSpace}%Р%0
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index{texBundleRelation}%Р%0
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index{texSecondDifferential}%Р%0
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index{texTstarRepresentation}%С%0
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index{texFiberedMorphism}%С%0
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index{texAffine}%С%0
   {связность Картана}%
   {Cartan connection}%
\Index{texAffine}%С%0
   {символ Картана}%
   {Cartan symbol}%
\Index{texBiring}%С%0
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index{texBundleRelation}%С%0
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index{texEuclideanSpace}%С%0
   {симметричное биаддитивное отображение}%
   {symmetric biadditive map}%
\Index{texGenRelativity}%С%0
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index{texVectorSpace}%С%0
   {система \drc линейных уравнений}%
   {system of linear equations}%
\Index{texRefernceFrame}%С%0
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index{texNewton}%С%0
   {скалярный потенциал}%
   {scalar potential}%
\Index{texTidal}%С%0
   {скорость отклонения}%
   {speed of deviation}%
\Index{texSecondDifferential}%С%0
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Index{texBundleRelation}%С%0
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index{texBundleRelation}%С%0
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index{texAdditiveMap}%С%0
   {стандартная компонента аддитивного отображения $f$ над полем $F$}%
   {standard component of additive map, division ring}%
\Index{texBiadditiveMap}%С%0
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Index{texDifferential}%С%0
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Index{texBiadditiveMap}%С%0
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Index{texRingAdditiveMap}%С%0
   {стандартная компонента линейного отображения тела}%
   {standard component of linear map, division ring}%
\Index{texRingAdditiveMap}%С%0
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Index{texTensorProduct}%С%0
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%
\Index{texAdditiveMap}%С%0
   {стандартное представление аддитивного отображения тела над полем $F$}%
   {additive map, standard representation, division ring}%
\Index{texBiadditiveMap}%С%0
   {стандартное представление биаддитивного отображения тела над полем $F$}%
   {biadditive map, standard representation, division ring}%
\Index{texBiadditiveMap}%С%0
   {стандартное представление биаддитивного отображения тела над полем}%
   {biadditive map, standard representation, division ring}%
\Index{texDifferential}%С%0
   {стандартное представление дифференциала Гато отображения тела над полем $F$}%
   {Gateaux differential, standard representation, division ring}%
\Index{texBiadditiveMap}%С%0
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index{texRingAdditiveMap}%С%0
   {стандартное представление линейного отображения тела}%
   {linear map, standard representation, division ring}%
\Index{texBiring}%С%0
   {стандартное представление матрицы}%
   {Standard representation}%
\Index{texRingAdditiveMap}%С%0
   {стандартное представление полилинейного отображения тела}%
   {polylinear map, standard representation, division ring}%
\Index{texDrcBasis}%С%0
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBasis}%С%0
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texDivisionRing}%С%0
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%
\Index{texBundleRelation}%С%0
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index{texLinearMap}%С%0
   {сумма \drc линейных отображений}%
   {sum of drc linear maps, drc vector spaces}%
\Index{texDrcBasis}%С%0
   {сумма геометрических объектов}%
   {sum of geometrical objects}%
\Index{texBasis}%С%0
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometrical objects, vector space}%
\SetIndexSpace%
\Index{texGeomObject}%Т%0
   {тензор кручения}%
   {torsion tensor}%
\Index{texNewton}%Т%0
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index{texTensorProduct}%Т%0
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index{texTensorProduct}%Т%0
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index{texTensorProduct}%Т%0
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index{texLie}%Т%0
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index{texTensorProduct}%Т%0
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index{texVectorSpace}%Т%0
   {тип векторного пространства}%
   {vector space type}%
\Index{texSecondDifferential}%Т%0
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index{texSecondDifferential}%Т%0
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index{texDifferential}%Т%0
   {топологическое тело}%
   {topological division ring}%
\Index{texBundleRelation}%Т%0
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index{texTstarMorphism}%Т%0
   {транзитивное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index{texRepresentation}%Т%0
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index{texFiberedAlgebra}%Т%0
   {транзитивное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {transitive representation of fibered F-algebra}%
\SetIndexSpace%
\Index{texDiffProperty}%У%0
   {уравнение Килинга}%
   {Killing equation}%
\Index{texDiffProperty}%У%0
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index{texBiring}%У%0
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index{texFiberedMorphism}%Ф%0
   {фактор расслоение}%
   {quotient bundle}%
\Index{texBundleRelation}%Ф%0
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index{texGeomObject}%Ф%0
   {форма кручение}%
   {torsion form}%
\Index{texSecondDifferential}%Ф%0
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index{texDifferential}%Ф%0
   {фундаментальная последовательность в нормированное теле}%
   {fundamental sequence, valued division ring}%
\Index{texSecondDifferential}%Ф%0
   {функция $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector W$, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, D vector space}%
\Index{texSecondDifferential}%Ф%0
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index{texDifferential}%Ф%0
   {функция проективна над полем $R$ и непрерывна по направлению над полем $R$}%
   {projective function is continuous in direction over field R, division ring}%
\Index{texFrechet}%Ф%0
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index{texDifferential}%Ф%0
   {функция тела, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, division ring}%
\Index{texSecondDifferential}%Ф%0
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index{texDivisionRing}%Ц%0
   {центр кольца $D$}%
   {center of ring}%
\Index{texAffineSpace}%Ц%0
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Index{texBasis}%Ц%0
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index{texSecondDifferential}%Ч%0
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map with respect to variable, D vector space}%
\Index{texSecondDifferential}%Ч%0
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map with respect to variable, D vector space}%
\Index{texSecondDifferential}%Ч%0
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Index{texAdditiveMap}%Ч%0
   {частное аддитивное отображение переменной $v^i$}%
   {partial additive map of variable}%
\SetIndexSpace%
\Index{texVectorField}%Э%0
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index{texAffine}%Э%0
   {экстремальная кривая}%
   {extreme line}%
\Index{texTstarMorphism}%Э%0
   {эффективное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index{texRepresentation}%Э%0
   {эффективное представление группы}%
   {effective representation of group}%
\Index{texTstarRepresentation}%Э%0
   {эффективное представление группы}%
   {effective representation of group}%
\Index{texFiberedAlgebra}%Э%0
   {эффективное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {effective representation of fibered F-algebra}%
\Index{texFiberedGroup}%Э%0
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index{texVectorSpace}%Э%0
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index{texAdditiveMap}%Я%0
   {ядро аддитивного отображения $D$\Hyph векторного пространства}%
   {kernel of additive map, D vector space}%
\Index{texAdditiveMap}%Я%0
   {ядро аддитивного отображения тела}%
   {kernel of additive map, division ring}%
\Index{texTstarRepresentation}%Я%0
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of representation of group}%
\Index{texRepresentation}%Я%0
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index{texFiberedGroup}%Я%0
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index{texSecondDifferential}%Я%0
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%

\CloseIndex


==> Quaternion.Russian.tex <==
%auto-ignore
\def\texQuaternion{}
\ifx\PrintBook\undefined
\else
\chapter{Алгебра кватернионов}
\label{chapter: Quaternion Algebra}
\fi

\input{Quaternion.Eq}

\section{Линейная функция комплексного поля}
\label{section: Linear Function of Complex Field}

\begin{theorem}[Уравнения Коши - Римана]
\label{theorem: complex field over real field}
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим ${}_{\gi 0}\Vector e=1$, ${}_{\gi 1}\Vector e=i$ - базис алгебры $C$.
Тогда в этом базисе структурные константы имеют вид
\[
\begin{matrix}
{}_{\gi{00}}B^{\gi 0}=1&{}_{\gi{01}}B^{\gi 1}=1\ \ 
\\
{}_{\gi{10}}B^{\gi 1}=1&{}_{\gi{11}}B^{\gi 0}=-1
\end{matrix}
\]
Матрица линейной функции
\[
y^{\gi i}=x^{\gi j}\ {}_{\gi j}f^{\gi i}
\]
поля комплексных чисел над полем действительных чисел
удовлетворяет соотношению
\begin{align}
\label{eq: complex field over real field, 0}
{}_{\gi 0}f^{\gi 0}&={}_{\gi 1}f^{\gi 1}
\\
\label{eq: complex field over real field, 1}
{}_{\gi 0}f^{\gi 1}&=-{}_{\gi 1}f^{\gi 0}
\end{align}
\end{theorem}
\begin{proof}
Значение структурных констант следует из равенства $i^2=-1$.
Пользуясь равенством \eqref{eq: linear map over field, division ring, relation}
получаем соотношения
\begin{equation}
\label{eq: complex field over real field, 0, 0}
{}_{\gi 0}f^{\gi 0}=f^{\gi{kr}}\ {}_{\gi{k0}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 0}
=f^{\gi{0r}}\ {}_{\gi{00}}B^{\gi 0}\ {}_{\gi{0r}}B^{\gi 0}+f^{\gi{1r}}\ {}_{\gi{10}}B^{\gi 1}\ {}_{\gi{1r}}B^{\gi 0}
=f^{\gi{00}}-f^{\gi{11}}
\end{equation}
\begin{equation}
\label{eq: complex field over real field, 1, 0}
{}_{\gi 0}f^{\gi 1}=f^{\gi{kr}}\ {}_{\gi{k0}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 1}
=f^{\gi{0r}}\ {}_{\gi{00}}B^{\gi 0}\ {}_{\gi{0r}}B^{\gi 1}+f^{\gi{1r}}\ {}_{\gi{10}}B^{\gi 1}\ {}_{\gi{1r}}B^{\gi 1}
=f^{\gi{01}}+f^{\gi{10}}
\end{equation}
\begin{equation}
\label{eq: complex field over real field, 1, 1}
{}_{\gi 1}f^{\gi 0}=f^{\gi{kr}}\ {}_{\gi{k1}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 0}
=f^{\gi{0r}}\ {}_{\gi{01}}B^{\gi 1}\ {}_{\gi{1r}}B^{\gi 0}+f^{\gi{1r}}\ {}_{\gi{11}}B^{\gi 0}\ {}_{\gi{0r}}B^{\gi 0}
=-f^{\gi{01}}-f^{\gi{10}}
\end{equation}
\begin{equation}
\label{eq: complex field over real field, 0, 1}
{}_{\gi 1}f^{\gi 1}=f^{\gi{kr}}\ {}_{\gi{k1}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 1}
=f^{\gi{0r}}\ {}_{\gi{01}}B^{\gi 1}\ {}_{\gi{1r}}B^{\gi 1}+f^{\gi{1r}}\ {}_{\gi{11}}B^{\gi 0}\ {}_{\gi{0r}}B^{\gi 1}
=f^{\gi{00}}-f^{\gi{11}}
\end{equation}
Из равенств
\eqref{eq: complex field over real field, 0, 0} и
\eqref{eq: complex field over real field, 0, 1}
следует \eqref{eq: complex field over real field, 0}.
Из равенств
\eqref{eq: complex field over real field, 1, 0} и
\eqref{eq: complex field over real field, 1, 1}
следует \eqref{eq: complex field over real field, 1}.
\end{proof}

\begin{remark}
\label{remark: congugate complex and additive map}
Чтобы показать, насколько сложна задача поиска образующих
аддитивного отображения, рассмотрим, как выглядит равенство
\eqref{eq: additive multiplicative map over field, G, division ring, relation}
в случае поля комплексных чисел.
%\[
%\bordermatrix
%{
%&f^{\gi{00}}&f^{\gi{01}}&f^{\gi{10}}&f^{\gi{11}}
%\cr
%{}_{\gi 0}f^{\gi 0}&1&0&0&-1
%\cr
%{}_{\gi 0}f^{\gi 1}&0&1&1&0
%\cr
%{}_{\gi 1}f^{\gi 0}&0&-1&-1&0
%\cr
%{}_{\gi 1}f^{\gi 1}&1&0&0&-1
%}
%\]
%Равенство
%\eqref{eq: additive multiplicative map over field, G, division ring, relation}
%имеет вид
\begin{align*}
{}_{\gi 0}f^{\gi 0}
&
={}_{\gi 0}G^{\gi l}\ f^{\gi{kr}}_G\ {}_{\gi{kl}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 0}
\\
&
={}_{\gi 0}G^{\gi 0}\ f^{\gi{00}}_G\ {}_{\gi{00}}B^{\gi 0}\ {}_{\gi{00}}B^{\gi 0}
+{}_{\gi 0}G^{\gi 1}\ f^{\gi{10}}_G\ {}_{\gi{11}}B^{\gi 0}\ {}_{\gi{00}}B^{\gi 0}
\\
&
+{}_{\gi 0}G^{\gi 1}\ f^{\gi{01}}_G\ {}_{\gi{01}}B^{\gi 1}\ {}_{\gi{11}}B^{\gi 0}
+{}_{\gi 0}G^{\gi 0}\ f^{\gi{11}}_G\ {}_{\gi{10}}B^{\gi 1}\ {}_{\gi{11}}B^{\gi 0}
\\
&
={}_{\gi 0}G^{\gi 0}\ f^{\gi{00}}_G
-{}_{\gi 0}G^{\gi 1}\ f^{\gi{10}}_G
-{}_{\gi 0}G^{\gi 1}\ f^{\gi{01}}_G
-{}_{\gi 0}G^{\gi 0}\ f^{\gi{11}}_G
\\
&
={}_{\gi 0}G^{\gi 0}(f^{\gi{00}}_G-f^{\gi{11}}_G)
-{}_{\gi 0}G^{\gi 1}(f^{\gi{10}}_G+f^{\gi{01}}_G)
\end{align*}

\begin{align*}
{}_{\gi 0}f^{\gi 1}
&
={}_{\gi 0}G^{\gi l}\ f^{\gi{kr}}_G\ {}_{\gi{kl}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 1}
\\
&
={}_{\gi 0}G^{\gi 0}\ f^{\gi{01}}_G\ {}_{\gi{00}}B^{\gi 0}\ {}_{\gi{01}}B^{\gi 1}
+{}_{\gi 0}G^{\gi 1}\ f^{\gi{11}}_G\ {}_{\gi{11}}B^{\gi 0}\ {}_{\gi{01}}B^{\gi 1}
\\
&
+{}_{\gi 0}G^{\gi 1}\ f^{\gi{00}}_G\ {}_{\gi{01}}B^{\gi 1}\ {}_{\gi{10}}B^{\gi 1}
+{}_{\gi 0}G^{\gi 0}\ f^{\gi{10}}_G\ {}_{\gi{10}}B^{\gi 1}\ {}_{\gi{10}}B^{\gi 1}
\\
&
={}_{\gi 0}G^{\gi 0}\ f^{\gi{01}}_G
-{}_{\gi 0}G^{\gi 1}\ f^{\gi{11}}_G
+{}_{\gi 0}G^{\gi 1}\ f^{\gi{00}}_G
+{}_{\gi 0}G^{\gi 0}\ f^{\gi{10}}_G
\\
&
={}_{\gi 0}G^{\gi 0}(f^{\gi{01}}_G+f^{\gi{10}}_G)
+{}_{\gi 0}G^{\gi 1}(f^{\gi{00}}_G-f^{\gi{11}}_G)
\end{align*}

\begin{align*}
{}_{\gi 1}f^{\gi 0}
&
={}_{\gi 1}G^{\gi l}\ f^{\gi{kr}}_G\ {}_{\gi{kl}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 0}
\\
&
={}_{\gi 1}G^{\gi 0}\ f^{\gi{00}}_G\ {}_{\gi{00}}B^{\gi 0}\ {}_{\gi{00}}B^{\gi 0}
+{}_{\gi 1}G^{\gi 1}\ f^{\gi{10}}_G\ {}_{\gi{11}}B^{\gi 0}\ {}_{\gi{00}}B^{\gi 0}
\\
&
+{}_{\gi 1}G^{\gi 1}\ f^{\gi{01}}_G\ {}_{\gi{01}}B^{\gi 1}\ {}_{\gi{11}}B^{\gi 0}
+{}_{\gi 1}G^{\gi 0}\ f^{\gi{11}}_G\ {}_{\gi{10}}B^{\gi 1}\ {}_{\gi{11}}B^{\gi 0}
\\
&
={}_{\gi 1}G^{\gi 0}\ f^{\gi{00}}_G
-{}_{\gi 1}G^{\gi 1}\ f^{\gi{10}}_G
-{}_{\gi 1}G^{\gi 1}\ f^{\gi{01}}_G
-{}_{\gi 1}G^{\gi 0}\ f^{\gi{11}}_G
\\
&
={}_{\gi 1}G^{\gi 0}(f^{\gi{00}}_G-f^{\gi{11}}_G)
-{}_{\gi 1}G^{\gi 1}(f^{\gi{10}}_G+f^{\gi{01}}_G)
\end{align*}

\begin{align*}
{}_{\gi 1}f^{\gi 1}
&
={}_{\gi 1}G^{\gi l}\ f^{\gi{kr}}_G\ {}_{\gi{kl}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 1}
\\
&
={}_{\gi 1}G^{\gi 0}\ f^{\gi{01}}_G\ {}_{\gi{00}}B^{\gi 0}\ {}_{\gi{01}}B^{\gi 1}
+{}_{\gi 1}G^{\gi 1}\ f^{\gi{11}}_G\ {}_{\gi{11}}B^{\gi 0}\ {}_{\gi{01}}B^{\gi 1}
\\
&
+{}_{\gi 1}G^{\gi 1}\ f^{\gi{00}}_G\ {}_{\gi{01}}B^{\gi 1}\ {}_{\gi{10}}B^{\gi 1}
+{}_{\gi 1}G^{\gi 0}\ f^{\gi{10}}_G\ {}_{\gi{10}}B^{\gi 1}\ {}_{\gi{10}}B^{\gi 1}
\\
&
={}_{\gi 1}G^{\gi 0}\ f^{\gi{01}}_G
-{}_{\gi 1}G^{\gi 1}\ f^{\gi{11}}_G
+{}_{\gi 1}G^{\gi 1}\ f^{\gi{00}}_G
+{}_{\gi 1}G^{\gi 0}\ f^{\gi{10}}_G
\\
&
={}_{\gi 1}G^{\gi 0}(f^{\gi{01}}_G+f^{\gi{10}}_G)
+{}_{\gi 1}G^{\gi 1}(f^{\gi{00}}_G-f^{\gi{11}}_G)
\end{align*}
В случае комплексных чисел задачу облегчает наше знание,
что матрица оператора $G$ имеет вид либо
\begin{equation}
G=
\begin{pmatrix}
1&0\\0&1
\end{pmatrix}
\label{eq: additive map generator, complex field 1}
\end{equation}
либо
\begin{equation}
G=
\begin{pmatrix}
1&0\\0&-1
\end{pmatrix}
\label{eq: additive map generator, complex field 2}
\end{equation}
В случае образующей
\eqref{eq: additive map generator, complex field 2}
мы получаем соотношения между координатами преобразования
\[
{}_{\gi 0}f^{\gi 0}=-{}_{\gi 1}f^{\gi 1}
\ \ \ {}_{\gi 0}f^{\gi 1}={}_{\gi 1}f^{\gi 0}
\]
\qed
\end{remark}

\ifx\texFuture\Defined
\begin{theorem}[Уравнения Коши - Римана]
Если матрица
\[
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi 0}}{\partial x^{\gi 0}}
&
\displaystyle\frac{\partial y^{\gi 0}}{\partial x^{\gi 1}} 
\\ \\
\displaystyle\frac{\partial y^{\gi 1}}{\partial x^{\gi 0}}
&
\displaystyle\frac{\partial y^{\gi 1}}{\partial x^{\gi 1}}
\end{pmatrix}
\]
является якобианом функции комплексного переменного
\[
x=x^{\gi 0}+x^{\gi 1}i\rightarrow y=y^{\gi 0}(x^{\gi 0},x^{\gi 1})+y^{\gi 1}(x^{\gi 0},x^{\gi 1})i
\]
над полем действительных чисел,
то
\begin{align*}
\frac{\partial y^{\gi 1}}{\partial x^{\gi 0}}&=-\frac{\partial y^{\gi 0}}{\partial x^{\gi 1}}
\\
\frac{\partial y^{\gi 0}}{\partial x^{\gi 0}}&=\frac{\partial y^{\gi 1}}{\partial x^{\gi 1}}
\end{align*}
\end{theorem}
\begin{proof}
Следствие теоремы
\ifx\IntroCalculusBook\Defined
\ref{theorem: complex field over real field}.
\else
\ifx\EprintCalculus\Defined
\ref{theorem: complex field over real field}.
\else
\xRef{0701.238}{theorem: complex field over real field}.
\fi
\fi
\end{proof}

Рассмотрим функцию $y=x^2$. 
Чтобы увидеть связь производной отображения
\[
\begin{matrix}
\displaystyle\frac{dy}{dx}=2x
& &
\displaystyle\frac{d(y^{\gi 0}+y^{\gi 1}i)}{d(x^{\gi 0}+x^{\gi 1}i)}=2x^{\gi 0}+2x^{\gi 1}i
\end{matrix}
\]
и якобиана отображения над полем действительных чисел
\[
\begin{pmatrix}
2x^{\gi 0}
&
-2x^{\gi 1} 
\\
2x^{\gi 1}
&
2x^{\gi 0}
\end{pmatrix}
\]
рассмотрим дифференциал
\begin{align*}
dy=&2xdx
\\
d(y^{\gi 0}+y^{\gi 1}i)=&(2x^{\gi 0}+2x^{\gi 1}i)d(x^{\gi 0}+x^{\gi 1}i)
\\
=&2x^{\gi 0}dx^{\gi 0}-2x^{\gi 1}dx^{\gi 1}+(2x^{\gi 1}dx^{\gi 0}+2x^{\gi 0}dx^{\gi 1})i
\end{align*}
\fi

\section{Линейная функция тела кватернионов}
\label{section: Linear Function of Division Ring of Quaternions}

		\begin{definition}
Пусть $F$ - поле.
Расширение $F(i,j,k)$ поля $F$ называется
\AddIndex{алгеброй
\symb{E(F)}1{quaternion algebra over the field}
кватернионов над полем $F$}{quaternion algebra over the field}\footnote{Я
буду следовать определению из \citeBib{Izrail M. Gelfand: Quaternion Groups}.},
если произведение в алгебре $E$ определено согласно правилам
\begin{equation}
\begin{array}{c|ccc}
&i&j&k\\
\hline
i&-1&k&-j\\
j&-k&-1&i\\
k&j&-i&-1\\
\end{array}
\label{eq: product of quaternions}
\end{equation}
		\qed
		\end{definition}

Элементы алгебры $E(F)$ имеют вид
	\[
x=x^{\gi 0}+x^{\gi 1}i+x^{\gi 2}j+x^{\gi 3}k
	\]
где $x^{\gi i}\in F$, $\gi i=\gi 0$, $\gi 1$, $\gi 2$, $\gi 3$.
Кватернион
\[
\overline x=x^{\gi 0}-x^{\gi 1}i-x^{\gi 2}j-x^{\gi 3}k
\]
называется сопряжённым кватерниону $x$.
Мы определим \AddIndex{норму кватерниона}{norm of quaternion} $x$ равенством
	\begin{equation}
	\label{eq: norm of quaternion}
|x|^2=x\overline x=(x^{\gi 0})^2+(x^{\gi 1})^2+(x^{\gi 2})^2+(x^{\gi 3})^2
	\end{equation}
Из равенства \eqref{eq: norm of quaternion} следует, что
$E(F)$ является алгеброй с делением.\footnote{Гельфанд в \citeBib{Izrail M. Gelfand: Quaternion Groups}
даёт более общее определение, рассматривая алгебру кватернионов $E(F,a,b)$ с
законом умножения
\[
\begin{array}{c|ccc}
&i&j&k\\
\hline
i&a&k&aj\\
j&-k&b&-bi\\
k&-aj&bi&-ab\\
\end{array}
\]
где $a$, $b\in F$, $ab\ne 0$.
Однако эта алгебра становится телом только когда $a<0$, $b<0$.
Это следует из равенства
\[
x\overline x=(x^{\gi 0})^2-a(x^{\gi 1})^2-b(x^{\gi 2})^2+ab(x^{\gi 3})^2
\]
Тогда мы можем пронормировать базис так, что $a=-1$, $b=-1$.}
При этом обратный элемент имеет вид
	\begin{equation}
	\label{eq: inverce quaternion}
x^{-1}=|x|^{-2}\overline x
	\end{equation}

\begin{theorem}
\label{theorem: Quaternion over real field}
Рассмотрим тело кватернионов $E(F)$ как четырёхмерную алгебру над полем $F$.
Положим ${}_{\gi 0}\Vector e=1$, ${}_{\gi 1}\Vector e=i$, ${}_{\gi 2}\Vector e=j$, ${}_{\gi 3}\Vector e=k$
- базис алгебры $E(F)$.
Тогда в этом базисе структурные константы имеют вид
\ShowEq{structural constants, quaternions}
Стандартные компоненты аддитивной функции над полем $F$
и координаты соответствующего линейного преобразования над полем $F$
удовлетворяют соотношениям
$\\$
\begin{tabular}{l|r}
\begin{minipage}{170pt}
\begin{equation}
\label{eq: quaternion over real field, 1, 0}
\left\{
\begin{matrix}
{}_{\gi 0}f^{\gi 0}=f^{\gi{00}}-f^{\gi{11}}-f^{\gi{22}}-f^{\gi{33}}
\\
{}_{\gi 1}f^{\gi 1}=f^{\gi{00}}-f^{\gi{11}}+f^{\gi{22}}+f^{\gi{33}}
\\
{}_{\gi 2}f^{\gi 2}=f^{\gi{00}}+f^{\gi{11}}-f^{\gi{22}}+f^{\gi{33}}
\\
{}_{\gi 3}f^{\gi 3}=f^{\gi{00}}+f^{\gi{11}}+f^{\gi{22}}-f^{\gi{33}}
\end{matrix}
\right.
\end{equation}
\end{minipage}
&
\begin{minipage}{170pt}
\begin{equation}
\label{eq: quaternion over real field, 2, 0}
\left\{
\begin{matrix}
4\ f^{\gi{00}}={}_{\gi 0}f^{\gi 0}+{}_{\gi 1}f^{\gi 1}+{}_{\gi 2}f^{\gi 2}+{}_{\gi 3}f^{\gi 3}
\\
4\ f^{\gi{11}}=-{}_{\gi 0}f^{\gi 0}-{}_{\gi 1}f^{\gi 1}+{}_{\gi 2}f^{\gi 2}+{}_{\gi 3}f^{\gi 3}
\\
4\ f^{\gi{22}}=-{}_{\gi 0}f^{\gi 0}+{}_{\gi 1}f^{\gi 1}-{}_{\gi 2}f^{\gi 2}+{}_{\gi 3}f^{\gi 3}
\\
4\ f^{\gi{33}}=-{}_{\gi 0}f^{\gi 0}+{}_{\gi 1}f^{\gi 1}+{}_{\gi 2}f^{\gi 2}-{}_{\gi 3}f^{\gi 3}
\end{matrix}
\right.
\end{equation}
\end{minipage}
\end{tabular}
$\\$
\begin{tabular}{l|r}
\begin{minipage}{170pt}
\begin{equation}
\label{eq: quaternion over real field, 1, 1}
\left\{
\begin{matrix}
{}_{\gi 0}f^{\gi 1}=f^{\gi{01}}+f^{\gi{10}}+f^{\gi{23}}-f^{\gi{32}}
\\
{}_{\gi 1}f^{\gi 0}=-f^{\gi{01}}-f^{\gi{10}}+f^{\gi{23}}-f^{\gi{32}}
\\
{}_{\gi 2}f^{\gi 3}=-f^{\gi{01}}+f^{\gi{10}}-f^{\gi{23}}-f^{\gi{32}}
\\
{}_{\gi 3}f^{\gi 2}=f^{\gi{01}}-f^{\gi{10}}-f^{\gi{23}}-f^{\gi{32}}
\end{matrix}
\right.
\end{equation}
\end{minipage}
&
\begin{minipage}{170pt}
\begin{equation}
\label{eq: quaternion over real field, 2, 1}
\left\{
\begin{matrix}
4\ f^{\gi{10}}=-{}_{\gi 1}f^{\gi 0}+{}_{\gi 0}f^{\gi 1}-{}_{\gi 3}f^{\gi 2}+{}_{\gi 2}f^{\gi 3}
\\
4\ f^{\gi{01}}=-{}_{\gi 1}f^{\gi 0}+{}_{\gi 0}f^{\gi 1}+{}_{\gi 3}f^{\gi 2}-{}_{\gi 2}f^{\gi 3}
\\
4\ f^{\gi{32}}=-{}_{\gi 1}f^{\gi 0}-{}_{\gi 0}f^{\gi 1}-{}_{\gi 3}f^{\gi 2}-{}_{\gi 2}f^{\gi 3}
\\
4\ f^{\gi{23}}={}_{\gi 1}f^{\gi 0}+{}_{\gi 0}f^{\gi 1}-{}_{\gi 3}f^{\gi 2}-{}_{\gi 2}f^{\gi 3}
\end{matrix}
\right.
\end{equation}
\end{minipage}
\end{tabular}
$\\$
\begin{tabular}{l|r}
\begin{minipage}{170pt}
\begin{equation}
\label{eq: quaternion over real field, 1, 2}
\left\{
\begin{matrix}
{}_{\gi 0}f^{\gi 2}=f^{\gi{02}}-f^{\gi{13}}+f^{\gi{20}}+f^{\gi{31}}
\\
{}_{\gi 1}f^{\gi 3}=f^{\gi{02}}-f^{\gi{13}}-f^{\gi{20}}-f^{\gi{31}}
\\
{}_{\gi 2}f^{\gi 0}=-f^{\gi{02}}-f^{\gi{13}}-f^{\gi{20}}+f^{\gi{31}}
\\
{}_{\gi 3}f^{\gi 1}=-f^{\gi{02}}-f^{\gi{13}}+f^{\gi{20}}-f^{\gi{31}}
\end{matrix}
\right.
\end{equation}
\end{minipage}
&
\begin{minipage}{170pt}
\begin{equation}
\label{eq: quaternion over real field, 2, 2}
\left\{
\begin{matrix}
4\ f^{\gi{20}}=-{}_{\gi 2}f^{\gi 0}+{}_{\gi 3}f^{\gi 1}+{}_{\gi 0}f^{\gi 2}-{}_{\gi 1}f^{\gi 3}
\\
4\ f^{\gi{31}}=+{}_{\gi 2}f^{\gi 0}-{}_{\gi 3}f^{\gi 1}+{}_{\gi 0}f^{\gi 2}-{}_{\gi 1}f^{\gi 3}
\\
4\ f^{\gi{02}}=-{}_{\gi 2}f^{\gi 0}-{}_{\gi 3}f^{\gi 1}+{}_{\gi 0}f^{\gi 2}+{}_{\gi 1}f^{\gi 3}
\\
4\ f^{\gi{13}}=-{}_{\gi 2}f^{\gi 0}-{}_{\gi 3}f^{\gi 1}-{}_{\gi 0}f^{\gi 2}-{}_{\gi 1}f^{\gi 3}
\end{matrix}
\right.
\end{equation}
\end{minipage}
\end{tabular}
$\\$
\begin{tabular}{l|r}
\begin{minipage}{170pt}
\begin{equation}
\label{eq: quaternion over real field, 1, 3}
\left\{
\begin{matrix}
{}_{\gi 0}f^{\gi 3}=f^{\gi{03}}+f^{\gi{12}}-f^{\gi{21}}+f^{\gi{30}}
\\
{}_{\gi 1}f^{\gi 2}=-f^{\gi{03}}-f^{\gi{12}}-f^{\gi{21}}+f^{\gi{30}}
\\
{}_{\gi 2}f^{\gi 1}=f^{\gi{03}}-f^{\gi{12}}-f^{\gi{21}}-f^{\gi{30}}
\\
{}_{\gi 3}f^{\gi 0}=-f^{\gi{03}}+f^{\gi{12}}-f^{\gi{21}}-f^{\gi{30}}
\end{matrix}
\right.
\end{equation}
\end{minipage}
&
\begin{minipage}{170pt}
\begin{equation}
\label{eq: quaternion over real field, 2, 3}
\left\{
\begin{matrix}
4\ f^{\gi{30}}=-{}_{\gi 3}f^{\gi 0}-{}_{\gi 2}f^{\gi 1}+{}_{\gi 1}f^{\gi 2}+{}_{\gi 0}f^{\gi 3}
\\
4\ f^{\gi{21}}=-{}_{\gi 3}f^{\gi 0}-{}_{\gi 2}f^{\gi 1}-{}_{\gi 1}f^{\gi 2}-{}_{\gi 0}f^{\gi 3}
\\
4\ f^{\gi{12}}={}_{\gi 3}f^{\gi 0}-{}_{\gi 2}f^{\gi 1}-{}_{\gi 1}f^{\gi 2}+{}_{\gi 0}f^{\gi 3}
\\
4\ f^{\gi{03}}=-{}_{\gi 3}f^{\gi 0}+{}_{\gi 2}f^{\gi 1}-{}_{\gi 1}f^{\gi 2}+{}_{\gi 0}f^{\gi 3}
\end{matrix}
\right.
\end{equation}
\end{minipage}
\end{tabular}
\end{theorem}
\begin{proof}
Значение структурных констант следует из таблицы умножения
\eqref{eq: product of quaternions}.
Пользуясь равенством \eqref{eq: linear map over field, division ring, relation}
получаем соотношения
\begin{align*}
{}_{\gi 0}f^{\gi 0}&=f^{\gi{kr}}\ {}_{\gi{k0}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 0}
\\
&=f^{\gi{00}}\ {}_{\gi{00}}B^{\gi 0}\ {}_{\gi{00}}B^{\gi 0}+f^{\gi{11}}\ {}_{\gi{10}}B^{\gi 1}\ {}_{\gi{11}}B^{\gi 0}
+f^{\gi{22}}\ {}_{\gi{20}}B^{\gi 2}\ {}_{\gi{22}}B^{\gi 0}+f^{\gi{33}}\ {}_{\gi{30}}B^{\gi 3}\ {}_{\gi{33}}B^{\gi 0}
\\
&=f^{\gi{00}}-f^{\gi{11}}
-f^{\gi{22}}-f^{\gi{33}}
\end{align*}
\begin{align*}
{}_{\gi 0}f^{\gi 1}&=f^{\gi{kr}}\ {}_{\gi{k0}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 1}
\\
&=f^{\gi{01}}\ {}_{\gi{00}}B^{\gi 0}\ {}_{\gi{01}}B^{\gi 1}+f^{\gi{10}}\ {}_{\gi{10}}B^{\gi 1}\ {}_{\gi{10}}B^{\gi 1}
+f^{\gi{23}}\ {}_{\gi{20}}B^{\gi 2}\ {}_{\gi{23}}B^{\gi 1}+f^{\gi{32}}\ {}_{\gi{30}}B^{\gi 3}\ {}_{\gi{32}}B^{\gi 1}
\\
&=f^{\gi{01}}+f^{\gi{10}}
+f^{\gi{23}}-f^{\gi{32}}
\end{align*}
\begin{align*}
{}_{\gi 0}f^{\gi 2}&=f^{\gi{kr}}\ {}_{\gi{k0}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 2}
\\
&=f^{\gi{02}}\ {}_{\gi{00}}B^{\gi 0}\ {}_{\gi{02}}B^{\gi 2}+f^{\gi{13}}\ {}_{\gi{10}}B^{\gi 1}\ {}_{\gi{13}}B^{\gi 2}
+f^{\gi{20}}\ {}_{\gi{20}}B^{\gi 2}\ {}_{\gi{20}}B^{\gi 2}+f^{\gi{31}}\ {}_{\gi{30}}B^{\gi 3}\ {}_{\gi{31}}B^{\gi 2}
\\
&=f^{\gi{02}}-f^{\gi{13}}
+f^{\gi{20}}+f^{\gi{31}}
\end{align*}
\begin{align*}
{}_{\gi 0}f^{\gi 3}&=f^{\gi{kr}}\ {}_{\gi{k0}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 3}
\\
&=f^{\gi{03}}\ {}_{\gi{00}}B^{\gi 0}\ {}_{\gi{03}}B^{\gi 3}+f^{\gi{12}}\ {}_{\gi{10}}B^{\gi 1}\ {}_{\gi{12}}B^{\gi 3}
+f^{\gi{21}}\ {}_{\gi{20}}B^{\gi 2}\ {}_{\gi{21}}B^{\gi 3}+f^{\gi{30}}\ {}_{\gi{30}}B^{\gi 3}\ {}_{\gi{30}}B^{\gi 3}
\\
&=f^{\gi{03}}+f^{\gi{12}}
-f^{\gi{21}}+f^{\gi{30}}
\end{align*}
\begin{align*}
{}_{\gi 1}f^{\gi 0}&=f^{\gi{kr}}\ {}_{\gi{k1}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 0}
\\
&=f^{\gi{01}}\ {}_{\gi{01}}B^{\gi 1}\ {}_{\gi{11}}B^{\gi 0}+f^{\gi{10}}\ {}_{\gi{11}}B^{\gi 0}\ {}_{\gi{00}}B^{\gi 0}
+f^{\gi{23}}\ {}_{\gi{21}}B^{\gi 3}\ {}_{\gi{33}}B^{\gi 0}+f^{\gi{32}}\ {}_{\gi{31}}B^{\gi 2}\ {}_{\gi{22}}B^{\gi 0}
\\
&=-f^{\gi{01}}-f^{\gi{10}}
+f^{\gi{23}}-f^{\gi{32}}
\end{align*}
\begin{align*}
{}_{\gi 1}f^{\gi 1}&=f^{\gi{kr}}\ {}_{\gi{k1}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 1}
\\
&=f^{\gi{00}}\ {}_{\gi{01}}B^{\gi 1}\ {}_{\gi{10}}B^{\gi 1}+f^{\gi{11}}\ {}_{\gi{11}}B^{\gi 0}\ {}_{\gi{01}}B^{\gi 1}
+f^{\gi{22}}\ {}_{\gi{21}}B^{\gi 3}\ {}_{\gi{32}}B^{\gi 1}+f^{\gi{33}}\ {}_{\gi{31}}B^{\gi 2}\ {}_{\gi{23}}B^{\gi 1}
\\
&=f^{\gi{00}}-f^{\gi{11}}
+f^{\gi{22}}+f^{\gi{33}}
\end{align*}
\begin{align*}
{}_{\gi 1}f^{\gi 2}&=f^{\gi{kr}}\ {}_{\gi{k1}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 2}
\\
&=f^{\gi{03}}\ {}_{\gi{01}}B^{\gi 1}\ {}_{\gi{13}}B^{\gi 2}+f^{\gi{12}}\ {}_{\gi{11}}B^{\gi 0}\ {}_{\gi{02}}B^{\gi 2}
+f^{\gi{21}}\ {}_{\gi{21}}B^{\gi 3}\ {}_{\gi{31}}B^{\gi 2}+f^{\gi{30}}\ {}_{\gi{31}}B^{\gi 2}\ {}_{\gi{20}}B^{\gi 2}
\\
&=-f^{\gi{03}}-f^{\gi{12}}
-f^{\gi{21}}+f^{\gi{30}}
\end{align*}
\begin{align*}
{}_{\gi 1}f^{\gi 3}&=f^{\gi{kr}}\ {}_{\gi{k1}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 3}
\\
&=f^{\gi{02}}\ {}_{\gi{01}}B^{\gi 1}\ {}_{\gi{12}}B^{\gi 3}+f^{\gi{13}}\ {}_{\gi{11}}B^{\gi 0}\ {}_{\gi{03}}B^{\gi 3}
+f^{\gi{20}}\ {}_{\gi{21}}B^{\gi 3}\ {}_{\gi{30}}B^{\gi 3}+f^{\gi{31}}\ {}_{\gi{31}}B^{\gi 2}\ {}_{\gi{21}}B^{\gi 3}
\\
&=f^{\gi{02}}-f^{\gi{13}}
-f^{\gi{20}}-f^{\gi{31}}
\end{align*}
\begin{align*}
{}_{\gi 2}f^{\gi 0}&=f^{\gi{kr}}\ {}_{\gi{k2}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 0}
\\
&=f^{\gi{02}}\ {}_{\gi{02}}B^{\gi 2}\ {}_{\gi{22}}B^{\gi 0}+f^{\gi{13}}\ {}_{\gi{12}}B^{\gi 3}\ {}_{\gi{33}}B^{\gi 0}
+f^{\gi{20}}\ {}_{\gi{22}}B^{\gi 0}\ {}_{\gi{00}}B^{\gi 0}+f^{\gi{31}}\ {}_{\gi{32}}B^{\gi 1}\ {}_{\gi{11}}B^{\gi 0}
\\
&=-f^{\gi{02}}-f^{\gi{13}}
-f^{\gi{20}}+f^{\gi{31}}
\end{align*}
\begin{align*}
{}_{\gi 2}f^{\gi 1}&=f^{\gi{kr}}\ {}_{\gi{k2}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 1}
\\
&=f^{\gi{03}}\ {}_{\gi{02}}B^{\gi 2}\ {}_{\gi{23}}B^{\gi 1}+f^{\gi{12}}\ {}_{\gi{12}}B^{\gi 3}\ {}_{\gi{32}}B^{\gi 1}
+f^{\gi{21}}\ {}_{\gi{22}}B^{\gi 0}\ {}_{\gi{01}}B^{\gi 1}+f^{\gi{30}}\ {}_{\gi{32}}B^{\gi 1}\ {}_{\gi{10}}B^{\gi 1}
\\
&=f^{\gi{03}}-f^{\gi{12}}
-f^{\gi{21}}-f^{\gi{30}}
\end{align*}
\begin{align*}
{}_{\gi 2}f^{\gi 2}&=f^{\gi{kr}}\ {}_{\gi{k2}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 2}
\\
&=f^{\gi{00}}\ {}_{\gi{02}}B^{\gi 2}\ {}_{\gi{20}}B^{\gi 2}+f^{\gi{11}}\ {}_{\gi{12}}B^{\gi 3}\ {}_{\gi{31}}B^{\gi 2}
+f^{\gi{22}}\ {}_{\gi{22}}B^{\gi 0}\ {}_{\gi{02}}B^{\gi 2}+f^{\gi{33}}\ {}_{\gi{32}}B^{\gi 1}\ {}_{\gi{13}}B^{\gi 2}
\\
&=f^{\gi{00}}+f^{\gi{11}}
-f^{\gi{22}}+f^{\gi{33}}
\end{align*}
\begin{align*}
{}_{\gi 2}f^{\gi 3}&=f^{\gi{kr}}\ {}_{\gi{k2}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 3}
\\
&=f^{\gi{01}}\ {}_{\gi{02}}B^{\gi 2}\ {}_{\gi{21}}B^{\gi 3}+f^{\gi{10}}\ {}_{\gi{12}}B^{\gi 3}\ {}_{\gi{30}}B^{\gi 3}
+f^{\gi{23}}\ {}_{\gi{22}}B^{\gi 0}\ {}_{\gi{03}}B^{\gi 3}+f^{\gi{32}}\ {}_{\gi{32}}B^{\gi 1}\ {}_{\gi{12}}B^{\gi 3}
\\
&=-f^{\gi{01}}+f^{\gi{10}}
-f^{\gi{23}}-f^{\gi{32}}
\end{align*}
\begin{align*}
{}_{\gi 3}f^{\gi 0}&=f^{\gi{kr}}\ {}_{\gi{k3}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 0}
\\
&=f^{\gi{03}}\ {}_{\gi{03}}B^{\gi 3}\ {}_{\gi{33}}B^{\gi 0}+f^{\gi{12}}\ {}_{\gi{13}}B^{\gi 2}\ {}_{\gi{22}}B^{\gi 0}
+f^{\gi{21}}\ {}_{\gi{23}}B^{\gi 1}\ {}_{\gi{11}}B^{\gi 0}+f^{\gi{30}}\ {}_{\gi{33}}B^{\gi 0}\ {}_{\gi{00}}B^{\gi 0}
\\
&=-f^{\gi{03}}+f^{\gi{12}}
-f^{\gi{21}}-f^{\gi{30}}
\end{align*}
\begin{align*}
{}_{\gi 3}f^{\gi 1}&=f^{\gi{kr}}\ {}_{\gi{k3}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 1}
\\
&=f^{\gi{02}}\ {}_{\gi{03}}B^{\gi 3}\ {}_{\gi{32}}B^{\gi 1}+f^{\gi{13}}\ {}_{\gi{13}}B^{\gi 2}\ {}_{\gi{23}}B^{\gi 1}
+f^{\gi{20}}\ {}_{\gi{23}}B^{\gi 1}\ {}_{\gi{10}}B^{\gi 1}+f^{\gi{31}}\ {}_{\gi{33}}B^{\gi 0}\ {}_{\gi{01}}B^{\gi 1}
\\
&=-f^{\gi{02}}-f^{\gi{13}}
+f^{\gi{20}}-f^{\gi{31}}
\end{align*}
\begin{align*}
{}_{\gi 3}f^{\gi 2}&=f^{\gi{kr}}\ {}_{\gi{k3}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 2}
\\
&=f^{\gi{01}}\ {}_{\gi{03}}B^{\gi 3}\ {}_{\gi{31}}B^{\gi 2}+f^{\gi{10}}\ {}_{\gi{13}}B^{\gi 2}\ {}_{\gi{20}}B^{\gi 2}
+f^{\gi{23}}\ {}_{\gi{23}}B^{\gi 1}\ {}_{\gi{13}}B^{\gi 2}+f^{\gi{32}}\ {}_{\gi{33}}B^{\gi 0}\ {}_{\gi{02}}B^{\gi 2}
\\
&=f^{\gi{01}}-f^{\gi{10}}
-f^{\gi{23}}-f^{\gi{32}}
\end{align*}
\begin{align*}
{}_{\gi 3}f^{\gi 3}&=f^{\gi{kr}}\ {}_{\gi{k3}}B^{\gi p}\ {}_{\gi{pr}}B^{\gi 3}
\\
&=f^{\gi{00}}\ {}_{\gi{03}}B^{\gi 3}\ {}_{\gi{30}}B^{\gi 3}+f^{\gi{11}}\ {}_{\gi{13}}B^{\gi 2}\ {}_{\gi{21}}B^{\gi 3}
+f^{\gi{22}}\ {}_{\gi{23}}B^{\gi 1}\ {}_{\gi{12}}B^{\gi 3}+f^{\gi{33}}\ {}_{\gi{33}}B^{\gi 0}\ {}_{\gi{03}}B^{\gi 3}
\\
&=f^{\gi{00}}+f^{\gi{11}}
+f^{\gi{22}}-f^{\gi{33}}
\end{align*}

Мы группируем эти соотношения в системы линейных уравнений
\eqref{eq: quaternion over real field, 1, 0},
\eqref{eq: quaternion over real field, 1, 1},
\eqref{eq: quaternion over real field, 1, 2},
\eqref{eq: quaternion over real field, 1, 3}.

\eqref{eq: quaternion over real field, 2, 0} -
это решение системы линейных уравнений
\eqref{eq: quaternion over real field, 1, 0}.

\eqref{eq: quaternion over real field, 2, 1} -
это решение системы линейных уравнений
\eqref{eq: quaternion over real field, 1, 1}.

\eqref{eq: quaternion over real field, 2, 2} -
это решение системы линейных уравнений
\eqref{eq: quaternion over real field, 1, 2}.

\eqref{eq: quaternion over real field, 2, 3} -
это решение системы линейных уравнений
\eqref{eq: quaternion over real field, 1, 3}.
\end{proof}

\begin{theorem}
\label{theorem: Quaternion over real field, matrix}
Рассмотрим тело кватернионов $E(F)$ как четырёхмерную алгебру над полем $F$.
Положим ${}_{\gi 0}\Vector e=1$, ${}_{\gi 1}\Vector e=i$, ${}_{\gi 2}\Vector e=j$, ${}_{\gi 3}\Vector e=k$ - базис алгебры $E(F)$.
Стандартные компоненты аддитивной функции над полем $F$
и координаты этой функции над полем $F$
удовлетворяют соотношениям
\begin{align}
&
\begin{pmatrix}
{}_{\gi 0}f^{\gi 0}&{}_{\gi 0}f^{\gi 1}&{}_{\gi 0}f^{\gi 2}&{}_{\gi 0}f^{\gi 3}
\\
{}_{\gi 1}f^{\gi 1}&{}_{\gi 1}f^{\gi 0}&{}_{\gi 1}f^{\gi 3}&{}_{\gi 1}f^{\gi 2}
\\
{}_{\gi 2}f^{\gi 2}&{}_{\gi 2}f^{\gi 3}&{}_{\gi 2}f^{\gi 0}&{}_{\gi 2}f^{\gi 1}
\\
{}_{\gi 3}f^{\gi 3}&{}_{\gi 3}f^{\gi 2}&{}_{\gi 3}f^{\gi 1}&{}_{\gi 3}f^{\gi 0}
\end{pmatrix}
\nonumber
\\
=&
\begin{pmatrix}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{pmatrix}
\begin{pmatrix}
f^{\gi{00}}&-f^{\gi{32}}&-f^{\gi{13}}&-f^{\gi{21}}
\\
f^{\gi{11}}&-f^{\gi{23}}&-f^{\gi{02}}&-f^{\gi{30}}
\\
f^{\gi{22}}&-f^{\gi{10}}&-f^{\gi{31}}&-f^{\gi{03}}
\\
f^{\gi{33}}&-f^{\gi{01}}&-f^{\gi{20}}&-f^{\gi{12}}
\end{pmatrix}
\label{eq: quaternion over real field, 3}
\end{align}
\end{theorem}
\begin{proof}
Запишем равенство \eqref{eq: quaternion over real field, 1, 0}
в виде произведения матриц
\begin{equation}
\label{eq: quaternion over real field, 3, 0}
\begin{pmatrix}
{}_{\gi 0}f^{\gi 0}
\\
{}_{\gi 1}f^{\gi 1}
\\
{}_{\gi 2}f^{\gi 2}
\\
{}_{\gi 3}f^{\gi 3}
\end{pmatrix}
=
\begin{pmatrix}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{pmatrix}
\begin{pmatrix}
f^{\gi{00}}
\\
f^{\gi{11}}
\\
f^{\gi{22}}
\\
f^{\gi{33}}
\end{pmatrix}
\end{equation}
Запишем равенство \eqref{eq: quaternion over real field, 1, 1}
в виде произведения матриц
\begin{align}
\begin{pmatrix}
{}_{\gi 0}f^{\gi 1}
\\
{}_{\gi 1}f^{\gi 0}
\\
{}_{\gi 2}f^{\gi 3}
\\
{}_{\gi 3}f^{\gi 2}
\end{pmatrix}
&=
\begin{pmatrix}
1&1&1&-1
\\
-1&-1&1&-1
\\
-1&1&-1&-1
\\
1&-1&-1&-1
\end{pmatrix}
\begin{pmatrix}
f^{\gi{01}}
\\
f^{\gi{10}}
\\
f^{\gi{23}}
\\
f^{\gi{32}}
\end{pmatrix}
\nonumber
\\
&=
\begin{pmatrix}
-1&-1&-1&1
\\
1&1&-1&1
\\
1&-1&1&1
\\
-1&1&1&1
\end{pmatrix}
\begin{pmatrix}
{}-f^{\gi{01}}
\\
-f^{\gi{10}}
\\
-f^{\gi{23}}
\\
-f^{\gi{32}}
\end{pmatrix}
\label{eq: quaternion over real field, 3, 1}
\\
&=
\begin{pmatrix}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{pmatrix}
\begin{pmatrix}
-f^{\gi{32}}
\\
-f^{\gi{23}}
\\
-f^{\gi{10}}
\\
-f^{\gi{01}}
\end{pmatrix}
\nonumber
\end{align}
Запишем равенство \eqref{eq: quaternion over real field, 1, 2}
в виде произведения матриц
\begin{align}
\begin{pmatrix}
{}_{\gi 0}f^{\gi 2}
\\
{}_{\gi 1}f^{\gi 3}
\\
{}_{\gi 2}f^{\gi 0}
\\
{}_{\gi 3}f^{\gi 1}
\end{pmatrix}
&=
\begin{pmatrix}
1&-1&1&1
\\
1&-1&-1&-1
\\
-1&-1&-1&1
\\
-1&-1&1&-1
\end{pmatrix}
\begin{pmatrix}
f^{\gi{02}}
\\
f^{\gi{13}}
\\
f^{\gi{20}}
\\
f^{\gi{31}}
\end{pmatrix}
\nonumber
\\
&=
\begin{pmatrix}
-1&1&-1&-1
\\
-1&1&1&1
\\
1&1&1&-1
\\
1&1&-1&1
\end{pmatrix}
\begin{pmatrix}
-f^{\gi{02}}
\\
-f^{\gi{13}}
\\
-f^{\gi{20}}
\\
-f^{\gi{31}}
\end{pmatrix}
\label{eq: quaternion over real field, 3, 2}
\\
&=
\begin{pmatrix}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{pmatrix}
\begin{pmatrix}
-f^{\gi{13}}
\\
-f^{\gi{02}}
\\
-f^{\gi{31}}
\\
-f^{\gi{20}}
\end{pmatrix}
\nonumber
\end{align}
Запишем равенство \eqref{eq: quaternion over real field, 1, 3}
в виде произведения матриц
\begin{align}
\begin{pmatrix}
{}_{\gi 0}f^{\gi 3}
\\
{}_{\gi 1}f^{\gi 2}
\\
{}_{\gi 2}f^{\gi 1}
\\
{}_{\gi 3}f^{\gi 0}
\end{pmatrix}
&=
\begin{pmatrix}
1&1&-1&1
\\
-1&-1&-1&1
\\
1&-1&-1&-1
\\
-1&1&-1&-1
\end{pmatrix}
\begin{pmatrix}
f^{\gi{03}}
\\
f^{\gi{12}}
\\
f^{\gi{21}}
\\
f^{\gi{30}}
\end{pmatrix}
\nonumber
\\
&=
\begin{pmatrix}
-1&-1&1&-1
\\
1&1&1&-1
\\
-1&1&1&1
\\
1&-1&1&1
\end{pmatrix}
\begin{pmatrix}
-f^{\gi{03}}
\\
-f^{\gi{12}}
\\
-f^{\gi{21}}
\\
-f^{\gi{30}}
\end{pmatrix}
\label{eq: quaternion over real field, 3, 3}
\\
&=
\begin{pmatrix}
1&-1&-1&-1
\\
1&-1&1&1
\\
1&1&-1&1
\\
1&1&1&-1
\end{pmatrix}
\begin{pmatrix}
-f^{\gi{21}}
\\
-f^{\gi{30}}
\\
-f^{\gi{03}}
\\
-f^{\gi{12}}
\end{pmatrix}
\nonumber
\end{align}
Мы объединяем равенства
\eqref{eq: quaternion over real field, 3, 0},
\eqref{eq: quaternion over real field, 3, 1},
\eqref{eq: quaternion over real field, 3, 2},
\eqref{eq: quaternion over real field, 3, 3}
в равенстве
\eqref{eq: quaternion over real field, 3}.
\end{proof}

\ifx\texFuture\Defined
\section{Отображения между разными алгебрами}

Для алгебры кватернионов над полем действительных чисел
принято обозначение $H=E(R)$.

\begin{theorem}
Линейная функция
\ShowEq{function from R to H}
удовлетворяет равенству
\end{theorem}
\begin{proof}
Над полем действительных чисел
мы можем представить функцию \eqref{eq: function from R to H}
в виде матрицы
\ShowEq{function from R to H, coordinates}
Если в качестве генератора мы выберем отображение
\ShowEq{function from R to H, generator}
то равенство
\eqref{eq: additive multiplicative map over field, G, division ring, relation}
принимает вид
\ShowEq{function from R to H, relation}
\end{proof}
\fi

\ifx\texDifferential\Defined
\section{Дифференцируемое отображение тела кватернионов}

\begin{theorem}
Если матрица
$\displaystyle
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi i}}{\partial x^{\gi j}}
\end{pmatrix}
$
является якобианом функции
$
x\rightarrow y
$
тела кватернионов над полем действительных чисел,
то
\ShowEq{quaternion over real field, derivative}
\end{theorem}
\begin{proof}
Следствие теоремы
\ifx\IntroCalculusBook\Defined
\ref{theorem: Quaternion over real field}.
\else
\ifx\EprintCalculus\Defined
\ref{theorem: Quaternion over real field}.
\else
\xRef{0701.238}{theorem: Quaternion over real field}.
\fi
\fi
\end{proof}

\begin{theorem}
\label{theorem: quaternion conjugation, derivative}
Отображение кватернионов
\[
f(x)=\overline x
\]
имеет производную Гато
\begin{equation}
\label{eq: quaternion conjugation, derivative}
\partial (\overline x)(h)=-\frac 12(h+ihi+jhj+khk)
\end{equation}
\end{theorem}
\begin{proof}
Якобиан отображения $f$ имеет вид
\[
\begin{pmatrix}
1&0&0&0
\\
0&-1&0&0
\\
0&0&-1&0
\\
0&0&0&-1
\end{pmatrix}
\]
Из равенств
\eqref{eq: quaternion over real field, derivative, 2, 0}
следует
\begin{equation}
\label{eq: quaternion conjugation, derivative, 1}
\StandPartial{y}{x}{00}=
\StandPartial{y}{x}{11}=
\StandPartial{y}{x}{22}=
\StandPartial{y}{x}{33}=
-\frac 12
\end{equation}
Из равенств
\eqref{eq: quaternion over real field, derivative, 2, 1},
\eqref{eq: quaternion over real field, derivative, 2, 2},
\eqref{eq: quaternion over real field, derivative, 2, 3}
следует
\begin{equation}
\label{eq: quaternion conjugation, derivative, 2}
\StandPartial{y}{x}{ij}=0
\ \ \ \gi i\ne\gi j
\end{equation}
Равенство
\eqref{eq: quaternion conjugation, derivative}
следует из равенств
\eqref{eq: Gateaux differential, division ring, standard representation},
\eqref{eq: quaternion conjugation, derivative, 1},
\eqref{eq: quaternion conjugation, derivative, 2}.
\end{proof}

\begin{theorem}
Сопряжение кватернионов удовлетворяет равенству
\[
\overline x=-\frac 12(x+ixi+jxj+kxk)
\]
\end{theorem}
\begin{proof}
Утверждение теоремы следует из теоремы
\ref{theorem: quaternion conjugation, derivative}
и примера \ref{example: differential equation, additive function, division ring}.
\end{proof}

\begin{theorem}
Если матрица
$\displaystyle
\begin{pmatrix}
\displaystyle\frac{\partial y^{\gi i}}{\partial x^{\gi j}}
\end{pmatrix}
$
является якобианом функции
$
x\rightarrow y
$
тела кватернионов над полем действительных чисел,
то
\ShowEq{quaternion over real field, derivative, 1}
\end{theorem}
\begin{proof}
Следствие теоремы
\ifx\IntroCalculusBook\Defined
\ref{theorem: Quaternion over real field, matrix}.
\else
\ifx\EprintCalculus\Defined
\ref{theorem: Quaternion over real field, matrix}.
\else
\xRef{0701.238}{theorem: Quaternion over real field, matrix}.
\fi
\fi
\end{proof}
\fi



==> Ring.Additive.Map.Russian.tex <==
%auto-ignore
\def\texRingAdditiveMap{}
\ifx\PrintBook\undefined
\else
\chapter{Линейное отображение тела}
\label{chapter: Linear map, Division Ring}
\fi

\input{Ring.Additive.Map.Eq}

\section{Аддитивное отображение кольца}

\begin{definition}
\label{definition: Additive map of Ring}
Гомоморфизм \[f:R_1\rightarrow R_2\] аддитивной группы кольца $R_1$
в аддитивную группу кольца $R_2$
называется
\AddIndex{аддитивным отображением
кольца $R_1$ в кольцо $R_2$}{Additive map of Ring}.
\qed
\end{definition} 

Согласно определению гомоморфизма аддитивной группы,
аддитивное отображение $f$ кольца $R_1$ в кольцо $R_2$
удовлетворяет свойству
\begin{equation}
f(a+b)=f(a)+f(b)
\label{eq: additive map, ring}
\end{equation}
\ifx\EprintCalculus\undefined
Мы не требуем, чтобы аддитивное отображение
кольца сохраняло произведение.
\fi

\begin{theorem}
\label{theorem: sum of additive maps, ring}
Рассмотрим кольцо $R_1$ и кольцо $R_2$.
Пусть отображения \[f:R_1\rightarrow R_2\]
\[g:R_1\rightarrow R_2\] являются аддитивными отображениями.
Тогда отображение $f+g$ также является аддитивным.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\begin{align*}
(f+g)(x+y)
=&f(x+y)+g(x+y)
=f(x)+f(y)+g(x)+g(y)
\\
=&(f+g)(x)+(f+g)(y)
\end{align*}
\end{proof}

\begin{theorem}
\label{theorem: additive map times constant, ring}
Рассмотрим кольцо $R_1$ и кольцо $R_2$.
Пусть отображение \[f:R_1\rightarrow R_2\]
является аддитивным отображением.
Тогда отображения $af$, $fb$, $a$, $b\in R_2$, также являются аддитивными.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\begin{align*}
(af)(x+y)
=&a(f(x+y))
=a(f(x)+f(y))
=af(x)+af(y)
\\
=&(af)(x)+(af)(y)
\\
(fb)(x+y)
=&(f(x+y))b
=(f(x)+f(y))b
=f(x)b+f(y)b
\\
=&(fb)(x)+(fb)(y)
\end{align*}
\end{proof}

\begin{theorem}
\label{theorem: additive map, ring, morphism}
Мы можем представить аддитивное отображение кольца $R_1$
в ассоциативное кольцо $R_2$ в виде
\ShowEq{additive map, ring, morphism}
где $G_{(s)}$ - множество аддитивных отображений кольца $R_1$
в кольцо $R_2$.\footnote{Здесь и в дальнейшем мы будем предполагать
сумму по индексу, который записан в скобках и встречвется в произведении несколько раз.
Равенство \eqref{eq: additive map, ring, morphism}
является рекурсивным определением и есть надежда, что мы можем
его упростить.}
\end{theorem}
\begin{proof}
Утверждение теоремы следует из теорем
\ref{theorem: sum of additive maps, ring} и
\ref{theorem: additive map times constant, ring}.
\end{proof}

\begin{definition}
\label{definition: map multiplicative over commutative ring, ring}
Пусть коммутативное кольцо $P$ является подкольцом центра $Z(R)$ кольца $R$.
Отображение
\[f:R\rightarrow R\]
кольца $R$
называется
\AddIndex{мультипликативным над коммутативным кольцом $P$}
{map multiplicative over commutative ring, ring}, если
\[
f(px)=pf(x)
\]
для любого $p\in P$.
\qed
\end{definition}

\begin{definition}
Пусть коммутативное кольцо $F$ является подкольцом центра $Z(D)$ кольца $R$.
Аддитивное, мультипликативное над коммутативным кольцом $F$ отображение
\[
f:R\rightarrow R
\]
называется \AddIndex{линейным отображением над коммутативным кольцом $F$}
{linear map over commutative ring, ring}.
\qed
\end{definition}

\begin{definition}
\label{definition: map projective over commutative ring, ring}
Пусть коммутативное кольцо $P$ является подкольцом центра $Z(R)$ кольца $R$.
Отображение
\[f:R\rightarrow R\]
кольца $R$
называется
\AddIndex{проективным над коммутативным кольцом $P$}
{map projective over commutative ring, ring}, если
\[
f(px)=f(x)
\]
для любого $p\in P$. Множество
\[
Px=\{px:p\in P,x\in R\}
\]
называется
\AddIndex{направлением $x$ над коммутативным кольцом $P$}
{direction over commutative ring, ring}.\footnote{Направление
над коммутативным кольцом $P$ является подможеством кольца $R$.
Однако мы будем обозначать направление $Px$ элементом
$x\in R$, когда это не приводит к неоднозначности.
Мы будем говорить о направлении над коммутативным кольцом $Z(R)$,
если мы явно не указываем коммутативное кольцо $P$.}
\qed
\end{definition}

\begin{example}
\label{example: map projective over commutative ring, ring}
Если отображение $f$
кольца $R$ мультипликативно над коммутативным кольцом $P$,
то отображение
\[
g(x)=x^{-1}f(x)
\]
проективно над коммутативным кольцом $P$.
\qed
\end{example}

\begin{definition}
Обозначим \symb{\mathcal A(R_1;R_2)}1{set additive maps, ring}
множество аддитивных отображений
\[
f:R_1\rightarrow R_2
\]
кольца $R_1$
в кольцо $R_2$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: additive map, ring, integer}
Пусть отображение
\[
f:D\rightarrow D
\]
является аддитивным отображением кольца $R$.
Тогда
\[
f(nx)=nf(x)
\]
для любого целого $n$.
\end{theorem}
\begin{proof}
Мы докажем теорему индукцией по $n$.
При $n=1$ утверждение очевидно, так как
\[
f(1x)=f(x)=1f(x)
\]
Допустим уравнение справедливо при $n=k$. Тогда
\[
f((k+1)x)=f(kx+x)=f(kx)+f(x)=kf(x)+f(x)=(k+1)f(x)
\]
\end{proof}

\section{Аддитивное отображение тела}

\begin{theorem}
\label{theorem: additive map, division ring, rational}
Пусть отображение
\ShowEq{map, division ring D1 D2}
является аддитивным отображением тела $D_1$ в тело $D_2$.
Тогда
\[
f(ax)=af(x)
\]
для любого рационального $a$.
\end{theorem}
\begin{proof}
Запишем $a$ в виде $a=\frac pq$.
Положим $y=\frac 1qx$. Тогда
\begin{equation}
f(x)=f(qy)=qf(y)=qf\left(\frac 1qx\right)
\label{eq: additive map, division ring, rational, 1}
\end{equation}
Из равенства \eqref{eq: additive map, division ring, rational, 1}
следует
\begin{equation}
\frac 1qf(x)=f\left(\frac 1qx\right)
\label{eq: additive map, division ring, rational, 2}
\end{equation}
Из равенства \eqref{eq: additive map, division ring, rational, 2}
следует
\[
f\left(\frac pqx\right)=pf\left(\frac 1qx\right)=\frac pqf(x)
\]
\end{proof}

\begin{theorem}
\label{theorem: additive map multiplicative over rational field, division ring}
Аддитивное отображение
\ShowEq{map, division ring D1 D2}
тела $D_1$ в тело $D_2$
мультипликативно над полем рациональных чисел.
\end{theorem}
\begin{proof}
Следствие теоремы \ref{theorem: additive map, division ring, rational}.
\end{proof}

Мы не можем распространить утверждение теоремы
\ref{theorem: additive map multiplicative over rational field, division ring}
на произвольное подполе центра $Z(D)$ тела $D$.

\begin{theorem}
\label{theorem: exists additive map not multiplicative over complex field, division ring}
Пусть поле комплексных чисел $C$ является подполем
центра тела $D$.
Существует аддитивное отображение
\ShowEq{map, division ring D1 D2}
тела $D_1$ в тело $D_2$,
которое не мультипликативно над полем комплексных чисел.
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно рассмотреть поле
комплексных чисел $C$ так как $C=Z(C)$. Отображение
\[
z\rightarrow \overline z
\]
аддитивно. Однако равенство
\[
\overline{az}=a\overline z
\]
неверно.
\end{proof}

Теория комплексных векторных пространств настолько хорошо изучена, что из
доказательства теоремы
\ref{theorem: exists additive map not multiplicative over complex field, division ring}
легко вытекает следующая конструкция.
Пусть для некоторого тела $D$ существуют поля $F_1$, $F_2$ такие, что
$F_1\ne F_2$, $F_1\subset F_2\subset Z(D)$.
В этом случае существует отображение $I$ тела $D$, линейное над полем $F_1$,
но не линейное над полем $F_2$.\footnote{Например, в случае
комплексных чисел оператор $I$ является оператором комплексного
сопряжения. Множество операторов $I$ зависит от рассматриваемого
тела. Эти операторы представляют для нас интерес, когда мы рассматриваем
отображения тела, при которых меняется структура операции. Например,
отображение комплексных чисел $z\rightarrow\overline z$.}
Нетрудно видеть, что это отображение аддитивно.

Пусть $D_1$, $D_2$ - тела характеристики $0$.
Согласно теореме
\ref{theorem: additive map, ring, morphism}
аддитивное отображение
\ShowEq{additive map D1 D2}
имеет вид
\eqref{eq: additive map, ring, morphism}.
Выберем отображение $G_{(s)}(x)=G(x)$.
Аддитивное отображение
\ShowEq{additive map, ring, morphism G}
называется
\AddIndex{аддитивным отображением, порождённым отображением $G$}
{additive map generated by map, division ring}.
Отображение $G$ мы будем называть
\AddIndex{образующей аддитивного отображения}
{generator of additive map, division ring}.

\begin{theorem}
\label{theorem: additive map, division ring, center}
Пусть $F$, $F\subset Z(D_1)$, $F\subset Z(D_2)$, - поле.
Аддитивное отображение
\eqref{eq: additive map, ring, morphism G},
порождённое $F$\Hyph линейным отображением $G$, мультипликативно
над полем $F$.
\end{theorem}
\begin{proof}
Непосредственное следствие представления
\eqref{eq: additive map, ring, morphism G}
аддитивного отображения.
Для любого $a\in F$
\ShowEq{additive map, division ring, center}
\end{proof}

\begin{theorem}
\label{theorem: additive map based G, standard form, division ring}
Пусть $D_1$, $D_2$ - тела характеристики $0$.
Пусть $F$, $F\subset Z(D_1)$, $F\subset Z(D_2)$, - поле.
Пусть $G$ - $F$\Hyph линейное отображение.
Пусть $\Basis q$ - базис тела $D_2$ над полем $F$.
\symb{f^{\gi i\gi j}_G}0
{standard component of additive map, division ring}
\AddIndex{Стандартное представление аддитивного отображения
\eqref{eq: additive map, ring, morphism G}
над полем $F$}
{additive map, standard representation, division ring}
имеет вид\footnote{Представление аддитивного отображения с помощью
компонент аддитивного отображения
неоднозначно. Чисто алгебраическими методами мы можем
увеличить либо уменьшить число слагаемых.
Если размерность тела $D$ над полем $F$ конечна, то стандартное представление
аддитивного отображения гарантирует конечность множества
слагаемых в представлении отображения.}
\ShowEq{additive map, division ring, G, standard representation}
Выражение
$\ShowSymbol{standard component of additive map, division ring}$
в равенстве \eqref{eq: additive map, division ring, G, standard representation}
называется
\AddIndex{стандартной компонентой аддитивного отображения $f$ над полем $F$}
{standard component of additive map, division ring}.
\end{theorem}
\begin{proof}
Компоненты аддитивного отображения $f$
имеют разложение
\ShowEq{additive map, division ring, components extention}
относительно базиса $\Basis q$.
Если мы подставим \eqref{eq: additive map, division ring, components extention}
в \eqref{eq: additive map, ring, morphism G},
мы получим
\ShowEq{additive map, division ring, G, standard representation, 1}
Подставив в равенство \eqref{eq: additive map, division ring, G, standard representation, 1}
выражение
\ShowEq{additive map, division ring, G, standard representation, 2}
мы получим равенство \eqref{eq: additive map, division ring, G, standard representation}.
\end{proof}

\begin{theorem}
\label{theorem: additive multiplicative map over field, G, division ring}
Пусть $D_1$, $D_2$ - тела характеристики $0$.
Пусть $F$, $F\subset Z(D_1)$, $F\subset Z(D_2)$, - поле.
Пусть $G$ - $F$\Hyph линейное отображение.
Пусть $\Basis p$ - базис тела $D_1$ над полем $F$.
Пусть $\Basis q$ - базис тела $D_2$ над полем $F$.
Пусть ${}_{\gi{kl}}B^{\gi p}$ - структурные константы тела $D_2$.
Тогда аддитивное отображение
\eqref{eq: additive map, ring, morphism G},
порождённое $F$\Hyph линейным отображением $G$,
можно записать в виде
\ShowEq{additive multiplicative map over field, G, division ring}
\end{theorem}
\begin{proof}
Согласно теореме \ref{theorem: additive map, division ring, center}
аддитивное отображение тела $D$ линейно над полем $F$.
Выберем отображение
\ShowEq{additive map D1 D2 generator}
Согласно теореме \xRef{0701.238}{theorem: drc linear map of drc vector space}
аддитивное отображение $f(a)$ в базисе $\Basis e$
принимает вид
\eqref{eq: additive multiplicative map over field, G, division ring}.
Из равенств \eqref{eq: additive map, division ring, G, standard representation}
и \eqref{eq: additive map D1 D2 generator}
следует
\ShowEq{additive map, division ring, F linear map G, standard representation}
Из равенств \eqref{eq: additive multiplicative map over field, G, division ring}
и \eqref{eq: additive map, division ring, F linear map G, standard representation}
следует
\ShowEq{additive multiplicative map over field, G, division ring, 1}
Так как векторы ${}_{\gi r}\Vector e$ линейно независимы над полем $F$ и величины
$a^{\gi k}$ произвольны, то из равенства
\eqref{eq: additive multiplicative map over field, G, division ring, 1}
следует равенство \eqref{eq: additive multiplicative map over field, G, division ring, relation}.
\end{proof}

\begin{theorem}
\label{theorem: additive generator is regular map, division ring}
Пусть поле $F$ является подкольцом центра $Z(D)$ тела $D$ характеристики $0$.
$F$\Hyph линейное отображение, порождающее аддитивное отображение, является невырожденным 
отображением.
\end{theorem}
\begin{proof}
Согласно теореме об изоморфизмах аддитивное отображение
\eqref{eq: linear map, division ring} можно представить в виде композиции
\[
f(x)=f_1(x+H)
\]
канонического отображения $x\rightarrow x+H$ и изоморфизма $f_1$.
$H$ - идеал аддитивной группы тела $D$.
Допустим идеал $H$ нетривиален. Тогда
существуют $x_1\ne x_2$, $f(x_1)=f(x_2)$.
Следовательно, образ при отображении $f$ содержит
циклическую подгруппу.
Это противоречит утверждению, что характеристика тела $D$ равна $0$.
Следовательно, $H=\{0\}$ и каноническое отображение является невырожденным $F$\Hyph линейным
отображением либо $H=D$ и каноническое отображение является вырожденным
отображением.
\end{proof}

\begin{definition}
\label{definition: linear map, division ring}
Аддитивное отображение, линейное над
центром тела, называется \AddIndex{линейным отображением тела}
{linear map, division ring}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: linear map, division ring, canonical morphism}
Пусть $D$ является телом характеристики $0$.
Линейное отображение
\ShowEq{linear map, division ring}
имеет вид
\ShowEq{linear map, division ring, canonical morphism}
Выражение
\symb{\pC{s}{p}f}1
{component of linear map, division ring}, $p=0$, $1$,
в равенстве \eqref{eq: linear map, division ring, canonical morphism}
называется \AddIndex{компонентой линейного отображения $f$}
{component of linear map, division ring}.
\end{theorem}

\begin{theorem}
\label{theorem: linear map, standard form, division ring}
Пусть $D$ - тело характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над центром $Z(D)$.
\symb{f^{\gi i\gi j}}0
{standard component of linear map, division ring}
\AddIndex{Стандартное представление линейного отображения
\eqref{eq: linear map, division ring, canonical morphism}
тела}
{linear map, standard representation, division ring}
имеет вид\footnote{Представление линейного отображения тела с помощью
компонент линейного отображения
неоднозначно. Чисто алгебраическими методами мы можем
увеличить либо уменьшить число слагаемых.
Если размерность тела $D$ над полем $Z(D)$ конечна, то стандартное представление
линейного отображения гарантирует конечность множества
слагаемых в представлении отображения.}
\ShowEq{linear map, division ring, standard representation}
Выражение
$\ShowSymbol{standard component of linear map, division ring}$
в равенстве \eqref{eq: linear map, division ring, standard representation}
называется \AddIndex{стандартной компонентой линейного отображения $f$}
{standard component of linear map, division ring}.
\end{theorem}

\begin{theorem}
\label{theorem: linear map over field, division ring}
Пусть $D$ является телом характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над полем $Z(D)$.
Тогда линейное отображение
\eqref{eq: linear map, division ring}
можно записать в виде
\ShowEq{linear map over field, division ring}
\end{theorem}
\begin{proof}
Равенство
\eqref{eq: linear map, division ring, canonical morphism}
является частным случаем равенства
\eqref{eq: additive map, ring, morphism G}
при условии $G(x)=x$.
Теорема
\ref{theorem: linear map, standard form, division ring}
является частным случаем теоремы
\ref{theorem: additive map based G, standard form, division ring}
при условии $G(x)=x$.
Теорема
\ref{theorem: linear map over field, division ring}
является частным случаем теоремы
\ref{theorem: additive multiplicative map over field, G, division ring}
при условии $G(x)=x$.
Наша задача - показать, что мы можем положить $G(x)=x$.

Равенство
\eqref{eq: linear map over field, division ring, relation}
связывает координаты линейного преобразования $f$ относительно заданного
базиса $\Basis e$ тела $D$ над центром $Z(D)$
со стандартными компонентами этого преобразования, рассматриваемого как
линейное преобразование тела.
Для заданных координат линейного преобразования
мы можем рассматривать равенство
\eqref{eq: linear map over field, division ring, relation}
как систему линейных уравнений относительно
стандартных компонент.
Из теоремы \ref{theorem: linear map over field, division ring}
следует, что если определитель системы линейных уравнений
\eqref{eq: linear map over field, division ring, relation}
отличен от $0$, то для любого линейного преобразования тела $D$ над полем $Z(D)$
существует соответствующее линейное преобразование тела.

Если определитель системы линейных уравнений
\eqref{eq: linear map over field, division ring, relation}
равен $0$, то существуют отображения, отличные от отображения $G(x)=x$.
Если размерность тела конечна, то эти отображения порождают
конечно мерную алгебру. Структура этой алгебры будет рассмотрена в отдельной статье.
Не нарушая общности, мы будем полагать и в этом случае $G(x)=x$.
%Мы будем предполагать, что для заданного тела нам известно
%множество образующих. Мы также будем предполагать,
%что ни одна из образующих не выражается аддитивно через остальные образующие.
\end{proof}

\begin{theorem}
\label{theorem: linear map, division ring}
Пусть поле $F$ является подкольцом центра $Z(D)$ тела $D$ характеристики $0$.
Линейное отображение тела
мультипликативно
над полем $F$.
\end{theorem}
\begin{proof}
Непосредственное следствие определения
\ref{definition: linear map, division ring}.
\end{proof}

%Линейное отображение поля имеет вид
%\[
%y=ax
%\]
%и является многочленом первой степени относительно $x$.
%Аналогично, мы определякм скалярное произведение векторов,
%опираясь на квадратичные формы, которые либо симметричны,
%либо эрмитовы. Но в обоих случаях мы выбираем какой оператор $I$
%мы используем для заданного аргумента.

\begin{theorem}
Выражение
\[
{}_{\gi k}f^{\gi r}=f^{\gi i\gi j}
\ {}_{\gi{ik}}B^{\gi p}\ {}_{\gi{pj}}B^{\gi r}
\]
является тензором над полем $F$
\begin{equation}
{}_{\gi i}f'^{\gi j}={}_{\gi i}A^{\gi k}
\ {}_{\gi k}f^{\gi l}\ {}_{\gi l}A^{-1}{}^{\gi j}
\label{eq: standard component of additive map, division ring, transformation}
\end{equation}
\end{theorem}
\begin{proof}
$D$\Hyph линейное отображение относительно базиса $\Basis e$ имеет вид
\eqref{eq: linear map over field, division ring}.
Пусть $\Basis e{}'$ - другой базис. Пусть
\begin{equation}
{}_{\gi i}\Vector e{}'={}_{\gi i}A^{\gi j}\ {}_{\gi j}\Vector e
\label{eq: standard component of additive map, division ring, change basis}
\end{equation}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e{}'$.
Так как аддитивное отображение $f$ не меняется, то
\begin{equation}
f(x)=x'^{\gi k}\ {}_{\gi k}f'^{\gi l}\ {}_{\gi l}\Vector e{}'
\label{eq: standard component of additive map, division ring, transformation, 1}
\end{equation}
Подставим \xEqRef{0701.238}{eq: division ring over field, change basis, 3},
\eqref{eq: standard component of additive map, division ring, change basis}
в равенство \eqref{eq: standard component of additive map, division ring, transformation, 1}
\begin{equation}
f(x)
=x^{\gi i}\ {}_{\gi i}A^{-1}{}^{\gi k}\ {}_{\gi k}f'^{\gi l}
\ {}_{\gi l}A^{\gi j}\ {}_{\gi j}\Vector e
\label{eq: standard component of additive map, division ring, transformation, 2}
\end{equation}
Так как векторы ${}_{\gi j}\Vector e$ линейно независимы и
компоненты вектора $x^{\gi i}$ произвольны, то равенство
\eqref{eq: standard component of additive map, division ring, transformation}
следует
из равенства
\eqref{eq: standard component of additive map, division ring, transformation, 2}.
Следовательно, выражение
${}_kf^r$
является тензором над полем $F$.
\end{proof}

\ifx\EprintCalculus\undefined
\begin{definition}
Множество
\symb{\text{ker}f}
0{kernel of additive map, division ring}
\[
\ShowSymbol{kernel of additive map, division ring}=\{x\in D_1:f(x)=0\}
\]
называется
\AddIndex{ядром аддитивного отображения}{kernel of additive map, division ring}
\[f:D_1\rightarrow D_2\]
тела $D_1$
в тело $D_2$.
\qed
\end{definition}

\begin{theorem}
Ядро аддитивного отображения
\[f:D_1\rightarrow D_2\]
является подгруппой аддитивной группы тела $D_1$.
\end{theorem}
\begin{proof}
Пусть $a$, $b\in\text{ker}f$. Тогда
\begin{align*}
f(a)&=0
\\
f(b)&=0
\\
f(a+b)=f(a)+f(b)&=0
\end{align*}
Следовательно, $a+b\in\text{ker}f$.
\end{proof}

\begin{definition}
Аддитивное отображение
\[f:D_1\rightarrow D_2\]
тела $D_1$
в тело $D_2$
называется
\AddIndex{вырожденным}{singular additive map, division ring},
если
\[\text{ker}f\ne\{0\}\]
\qed
\end{definition}
\fi

\begin{theorem}
\label{theorem: product of additive map, D D D}
Пусть $D$ - тело характеристики $0$.
Пусть $\Basis e$ - базис тела $D$ над центром $Z(D)$ тела $D$.
Пусть
\ShowEq{product of additive map, D D D}
линейные отображения тела $D$.
Отображение
\begin{equation}
h(x)=gf(x)=g(f(x))
\label{eq: D linear map, division ring, h1}
\end{equation}
является линейным отображением
\ShowEq{D linear map, division ring, h2}
где
\ShowEq{D linear map, division ring, h gf}
\end{theorem}
\begin{proof}
Отображение \eqref{eq: D linear map, division ring, h1}
аддитивно так как
\ShowEq{product of additive map, D D D, 1}
Отображение \eqref{eq: D linear map, division ring, h1}
мультипликативно над $Z(D)$ так как
\ShowEq{product of additive map, D D D, 2}

Если мы подставим
\eqref{eq: D linear map, division ring, f} и
\eqref{eq: D linear map, division ring, g} в
\eqref{eq: D linear map, division ring, h1},
то мы получим
\begin{equation}
h(x)=\pC{t}{0}g\ f(x)\ \pC{t}{1}g
=\pC{t}{0}g\ \pC{s}{0}f\ x\ \pC{s}{1}f\ \pC{t}{1}g
\label{eq: additive map, division ring, h3}
\end{equation}
Сравнивая \eqref{eq: additive map, division ring, h3}
и \eqref{eq: D linear map, division ring, h2},
мы получим \eqref{eq: D linear map, division ring, h gf, 0},
\eqref{eq: D linear map, division ring, h gf, 1}.

Если мы подставим
\eqref{eq: D linear map, division ring, standard representation, f} и
\eqref{eq: D linear map, division ring, standard representation, g} в
\eqref{eq: D linear map, division ring, h1},
то мы получим
\begin{align}
h(x)=&g^{\gi{ij}}\ {}_{\gi i}\Vector e\ f(x)\ {}_{\gi j}\Vector e
\nonumber
\\
=&g^{\gi{ij}}\ {}_{\gi i}\Vector e\ f^{\gi{kl}}\ {}_{\gi k}\Vector e
\ x\ {}_{\gi l}\Vector e\ {}_{\gi j}\Vector e
\label{eq: D linear map, division ring, standard representation, h3}
\\
=&g^{\gi{ij}}\ f^{\gi{kl}}\ {}_{\gi{ik}}B^{\gi p}
\ {}_{\gi{lj}}B^{\gi r}\ {}_{\gi p}e\ x\ {}_{\gi r}\Vector e
\nonumber
\end{align}
Сравнивая \eqref{eq: D linear map, division ring, standard representation, h3}
и \eqref{eq: D linear map, division ring, standard representation, h2},
мы получим \eqref{eq: D linear map, division ring, standard representation, h gf}.
\end{proof}

\section{Полилинейное отображение тела}

\begin{definition}
\label{definition: polyadditive map of division rings}
Пусть $R_1$, ..., $R_n$ -
кольца и $S$ - модуль.
Мы будем называть отображение
\begin{equation}
f:R_1\times...\times R_n\rightarrow
S
\label{eq: polyadditive map of rings}
\end{equation}
\AddIndex{полиаддитивным отображением колец}
{polyadditive map of rings}
$R_1$, ..., $R_n$
в модуль $S$,
если
\[
f(
p_1, ...,
p_i+ q_i, ...,
p_n)
=
f(
p_1, ...,
p_i, ...,
p_n)
+
f(
p_1, ...,
q_i, ...,
p_n)
\]
для любого $1\le i\le n$ и
для любых $p_i$, $q_i \in R_i$.
Обозначим
\symb{\mathcal A(R_1,...,R_n;
S)}1{set polyadditive maps, ring}
множество полиаддитивных отображений
колец
$R_1$, ..., $R_n$
в модуль
$S$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: map polylinear over commutative ring, ring}
Пусть $R_1$, ..., $R_n$, $P$ - кольца характеристики $0$.
Пусть $S$ - модуль над кольцом $P$.
Пусть
\[
f:R_1\times...\times R_n\rightarrow
S
\]
полиаддитивное отображение.
Существует коммутативное кольцо $F$, которое для любого $i$ является подкольцом центра
кольца $R_i$, и такое, что
для любого $i$ и $b\in F$
\[
f(a_1, ..., b a_i, ..., a_n)=bf(a_1, ..., a_i, ..., a_n)
\]
\end{theorem}
\begin{proof}
Для заданных $a_1$, ..., $a_{i-1}$, $a_{i+1}$, ..., $a_n$
отображение $f(a_1, ..., a_n)$ адитивно по $a_i$.
Согласно теореме
\ref{theorem: additive map, ring, integer},
мы можем выбрать кольцо целых чисел в качестве кольца $F$.
\end{proof}

\begin{definition}
\label{definition: map polylinear over commutative ring, ring}
Пусть $R_1$, ..., $R_n$, $P$ - кольца характеристики $0$.
Пусть $S$ - модуль над кольцом $P$.
Пусть $F$ - коммутативное кольцо, которое для любого $i$ является подкольцом центра
кольца $R_i$.
Отображение
\[
f:R_1\times...\times R_n\rightarrow
S
\]
называется \AddIndex{полилинейным над коммутативным кольцом $F$}
{map polylinear over commutative ring, ring},
если отображение $f$
полиадитивно, и для любого $i$, $1\le i\le n$,
для заданных $a_1$, ..., $a_{i-1}$, $a_{i+1}$, ..., $a_n$
отображение $f(a_1, ..., a_n)$ мультипликативно по $a_i$.
Если кольцо $F$ - максимальное кольцо такое, что для любого $i$, $1\le i\le n$,
для заданных $a_1$, ..., $a_{i-1}$, $a_{i+1}$, ..., $a_n$
отображение $f(a_1, ..., a_n)$ линейно по $a_i$ над кольцом $F$,
то отображение $f$ называется
\AddIndex{полилинейным отображением колец}{polylinear map of rings}
$R_1$, ..., $R_n$
в модуль $S$.
Обозначим
\symb{\mathcal L(R_1,...,R_n;
S)}1{set polylinear maps, ring}
множество полилинейных отображений
колец
$R_1$, ..., $R_n$
в модуль
$S$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: polylinear map, division ring}
Пусть $D$ - тело характеристики $0$.
Полилинейное отображение
\ShowEq{polylinear map, division ring}
имеет вид
\ShowEq{polylinear map, division ring, canonical morphism}
$\sigma_s$ - перестановка множества переменных
$\{d_1,...,d_n\}$
\ShowEq{transposition of set of variables, division ring}
\end{theorem}
\begin{proof}
Мы докажем утверждение индукцией по $n$.

При $n=1$ доказываемое утверждение является следствием теоремы
\ref{theorem: linear map, division ring, canonical morphism}.
При этом мы можем отождествить\footnote{В представлении
\eqref{eq: polylinear map, division ring, canonical morphism}
мы будем пользоваться следующими правилами.
\begin{itemize}
\item Если область значений какого-либо индекса - это множество,
состоящее из одного элемента, мы будем опускать соответствующий
индекс.
\item Если $n=1$, то $\sigma_s$ - тождественное преобразование.
Это преобразование можно не указывать в выражении.
\end{itemize}} ($p=0$, $1$)
\ShowEq{polylinear map, division ring, 1, canonical morphism}

Допустим, что утверждение теоремы справедливо при $n=k-1$.
Тогда отображение
\eqref{eq: polylinear map, division ring}
можно представить в виде
\ShowEq{polylinear map, induction on n, 1, division ring}
Согласно предположению индукции полиаддитивное отображение
$h$ имеет вид
\ShowEq{polylinear map, induction on n, 2, division ring}
Согласно построению $h=g(d_k)$.
Следовательно, выражения $\pC{t}{p}h$
являются функциями $d_k$.
Поскольку $g(d_k)$ - аддитивная функция $d_k$,
то только одно выражение $\pC{t}{p}h$
является аддитивной функцией переменной $d_k$, и остальные выражения
$\pC{t}{q}h$
не зависят от $d_k$.

Не нарушая общности, положим $p=0$.
Согласно равенству
\eqref{eq: linear map, division ring, canonical morphism}
для заданного $t$
\ShowEq{polylinear map, induction on n, 3, division ring}
Положим $s=tr$ и определим перестановку $\sigma_s$ согласно правилу
\ShowEq{polylinear map, induction on n, 4, division ring}
Положим
\ShowEq{polylinear map, induction on n, 5, division ring}
для $q=1$, ..., $k-1$.
\ShowEq{polylinear map, induction on n, 6, division ring}
для $q=0$, $1$.
Мы доказали шаг индукции.
\end{proof}

\begin{definition}
\begin{sloppypar}
Выражение
\symb{\pC{s}{p}f^n}1
{component of polylinear map, division ring}
в равенстве \eqref{eq: polylinear map, division ring, canonical morphism}
называется \AddIndex{компонентой полилинейного отображения $f$}
{component of polylinear map, division ring}.
\qed
\end{sloppypar}
\end{definition}

\begin{theorem}
\label{theorem: standard representation of polylinear map, division ring}
Пусть $D$ - тело характеристики $0$.
Допустим $\Basis e$
- базис тела $D$ над полем $Z(D)$.
\symb{\pC{t}{}f^{\gi{i_0...i_n}}}0
{standard component of polylinear map, division ring}
\AddIndex{Стандартное представление полилинейного отображения тела}
{polylinear map, standard representation, division ring}
имеет вид
\ShowEq{polylinear map, division ring, standard representation}
Индекс $t$ нумерует всевозможные перестановки
$\sigma_t$ множества переменных
$\{d_1,...,d_n\}$.
Выражение
$\ShowSymbol{standard component of polylinear map, division ring}$
в равенстве \eqref{eq: polylinear map, division ring, standard representation}
называется \AddIndex{стандартной компонентой полилинейного отображения $f$}
{standard component of polylinear map, division ring}.
\end{theorem}
\begin{proof}
Компоненты полилинейного отображения $f$
имеют разложение
\ShowEq{polylinear map, division ring, components extention}
относительно базиса $\Basis e$.
Если мы подставим \eqref{eq: polylinear map, division ring, components extention}
в \eqref{eq: polylinear map, division ring, canonical morphism},
мы получим
\ShowEq{polylinear map, division ring, standard representation, 1}
Рассмотрим выражение
\ShowEq{polylinear map, division ring, standard representation, 2}
В правой части подразумевается сумма тех слагаемых с индексом $s$,
для которых перестановка $\sigma_s$ совпадает. Каждая такая сумма
будет иметь уникальный индекс $t$.
Подставив в равенство
\eqref{eq: polylinear map, division ring, standard representation, 1}
выражение
\eqref{eq: polylinear map, division ring, standard representation, 2}
мы получим равенство \eqref{eq: polylinear map, division ring, standard representation}.
\end{proof}

\begin{theorem}
\label{theorem: polylinear map over field, division ring}
Пусть $\Basis e$ - базис тела $D$ над полем $Z(D)$.
Полиаддитивное отображение
\eqref{eq: polylinear map, division ring}
можно представить в виде $D$-значной формы степени $n$
над полем $Z(D)$\footnote{Теорема доказана по аналогии
с теоремой в \citeBib{Rashevsky}, с. 107, 108}
\ShowEq{polylinear map over field, division ring}
где
\ShowEq{polylinear map over field, coordinates, division ring}
и величины ${}_{\gi{i_1...i_n}}f$
являются координатами $D$-значного ковариантнго тензора над полем $F$.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: map polylinear over commutative ring, ring}
равенство
\eqref{eq: polylinear map over field, division ring}
следует из цепочки равенств
\ShowEq{polylinear map over field, 1, division ring}
Пусть $\Basis e'$ - другой базис. Пусть
\ShowEq{polylinear map over field, division ring, change basis}
преобразование, отображающее базис $\Basis e$ в
базис $\Basis e'$.
Из равенств \eqref{eq: polylinear map over field, division ring, change basis}
и \eqref{eq: polylinear map over field, coordinates, division ring}
следует
\ShowEq{polylinear map over field, division ring, change coordinates}
Из равенства \eqref{eq: polylinear map over field, division ring, change coordinates}
следует тензорный закон преобразования координат полилинейного отображения.
Из равенства \eqref{eq: polylinear map over field, division ring, change coordinates}
и теоремы \xRef{0701.238}{theorem: division ring over field, change basis}
следует, что значение отображения $f(\Vector a_1,...,\Vector a_n)$ не зависит от выбора
базиса.
\end{proof}

Полилинейное отображение
\eqref{eq: polylinear map, division ring}
\AddIndex{симметрично}
{polylinear map symmetric, division ring}, если
\[
f(d_1,...,d_n)=f(\sigma(d_1),...,\sigma(d_n))
\]
для любой перестановки $\sigma$ множества $\{d_1,...,d_n\}$.

\begin{theorem}
\label{theorem: polylinear map symmetric, division ring}
Если полилинейное отображение $f$ симметрично,
то
\ShowEq{polylinear map symmetric, division ring}
\end{theorem}
\begin{proof}
Равенство
\eqref{eq: polylinear map symmetric, division ring}
следует из равенства
\ShowEq{polylinear map symmetric, 1, division ring}
\end{proof}

Полилинейное отображение
\eqref{eq: polylinear map, division ring}
\AddIndex{косо симметрично}
{polylinear map skew symmetric, division ring}, если
\[
f(d_1,...,d_n)=|\sigma|f(\sigma(d_1),...,\sigma(d_n))
\]
для любой перестановки $\sigma$ множества $\{d_1,...,d_n\}$.
Здесь
\[
|\sigma|=
\left\{
\begin{matrix}
1&\textrm{перестановка }\sigma\textrm{ чётная}
\\
-1&\textrm{перестановка }\sigma\textrm{ нечётная}
\end{matrix}
\right.
\]

\begin{theorem}
\label{theorem: polylinear map skew symmetric, division ring}
Если полилинейное отображение $f$ косо симметрично,
то
\ShowEq{polylinear map skew symmetric, division ring}
\end{theorem}
\begin{proof}
Равенство
\eqref{eq: polylinear map skew symmetric, division ring}
следует из равенства
\ShowEq{polylinear map skew symmetric, 1, division ring}
\end{proof}

\begin{theorem}
\label{theorem: coordinates of polylinear map, division ring over field}
Отображение
\eqref{eq: polylinear map, division ring}
полилинейное над полем $F$
полилинейно тогда и только тогда, когда
\ShowEq{coordinates of polylinear map, division ring over field}
\end{theorem}
\begin{proof}
В равенстве \eqref{eq: polylinear map, division ring, standard representation}
положим
\ShowEq{coordinates of polylinear map, 1, division ring over field}
Тогда равенство \eqref{eq: polylinear map, division ring, standard representation}
примет вид
\ShowEq{polylinear map, division ring, standard representation, 1a}
Из равенства \eqref{eq: polylinear map over field, division ring}
следует
\ShowEq{polylinear map over field, division ring, 1a}
Равенство
\eqref{eq: coordinates of polylinear map, division ring over field}
следует из сравнения равенств
\eqref{eq: polylinear map, division ring, standard representation, 1a}
и
\eqref{eq: polylinear map over field, division ring}.
Равенство
\eqref{eq: coordinates of polylinear map, division ring over field, 1}
следует из сравнения равенств
\eqref{eq: polylinear map, division ring, standard representation, 1a}
и
\eqref{eq: polylinear map over field, division ring, 1a}.
\end{proof}


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%A 0
\Symb{texBiring}%
   {$(^a_b)$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb{texBiring}%
   {$(^a_b)$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant definition}%
\Symb{texBiring}%
   {минор}%
   {A from b a}%
\Symb{texBiring}%
   {минор}%
   {A from columns T}%
\Symb{texBiring}%
   {минор}%
   {A from rows S}%
\Symb{texBiring}%
   {минор}%
   {A without column a}%
\Symb{texBiring}%
   {минор}%
   {A without columns T}%
\Symb{texBiring}%
   {минор}%
   {A without row b}%
\Symb{texBiring}%
   {минор}%
   {A without rows S}%
\Symb{texAffineSpace}%
   {аффинное пространство}%
   {affine space}%
\Symb{texBasis}%
   {аффинное пространство}%
   {An}%
\Symb{texBiring}%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb{texAdditiveMap}%
   {компонента линейного отображения $\Vector{A}$ $D$\Hyph векторного пространства}%
   {component of linear map, D vector space}%
\Symb{texAdditiveMap}%
   {компонента $p$ полиаддитивного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb{texBiring}%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb{texBiring}%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb{texBiring}%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb{texVectorSpace}%
   {\dcr вектор}%
   {dcr vector}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb{texVectorSpace}%
   {\drc вектор}%
   {drc vector}%
\Symb{texSecondDifferential}%
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb{texAdditiveMap}%
   {частное аддитивное отображение переменной $v^i$}%
   {partial additive map of variable}%
\Symb{texBiring}%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb{texBiring}%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb{texBiring}%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb{texBiring}%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb{texBiring}%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb{texAdditiveMap}%
   {множество аддитивных отображений $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector{W}$}%
   {set additive maps, D vector space}%
\Symb{texRingAdditiveMap}%
   {множество аддитивных отображений кольца $R_1$ в кольцо $R_2$}%
   {set additive maps, ring}%
\Symb{texAdditiveMap}%
   {множество полиаддитивных отображений}%
   {set polyadditive maps, D vector space}%
\Symb{texRingAdditiveMap}%
   {множество полиаддитивных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polyadditive maps, ring}%
\Symb{texRingAdditiveMap}%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb{texPolyvector}%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb{texTstarRepresentation}%
   {правый сдвиг}%
   {starT shift}%
\Symb{texFiberedGroup}%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb{texTstarRepresentation}%
   {левый сдвиг}%
   {Tstar shift}%
\Symb{texFiberedGroup}%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb{texRefernceFrame}%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb{texRefernceFrame}%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B 0
\Symb{texBasis}%
   {многообразие базисов аффинного пространства}%
   {BAn}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства $\mathcal{V}$}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb{texBasis}%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb{texBundle}%
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power of bundle}%
\Symb{texBundle}%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb{texAffineSpace}%
   {многообразие базисов аффинного пространства}%
   {FAn}%
\Symb{texAffineSpace}%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb{texAffineSpace}%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb{texPolymodule}%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb{texDivisionRing}%
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%

\SetIndexSpace%C 0
\Symb{texBasis}%
   {центро-аффинное пространство}%
   {CAn}%
\Symb{texAffineSpace}%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb{texLie}%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb{texLie}%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%

\SetIndexSpace%D 0
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation, coordinates}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation, coordinates}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство \subs строк}%
   {c rows dcr vector space}%
\Symb{texSecondDifferential}%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Symb{texSecondDifferential}%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb{texDifferential}%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Symb{texSecondDifferential}%
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb{texDifferential}%
   {компонента производной Гато второго порядка отображения $f(x)$ тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Symb{texVectorField}%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb{texVectorSpace}%
   {координатное \drc векторное пространство}%
   {coordinate drc vector space}%
\Symb{texRefernceFrame}%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in bundle, 1}%
\Symb{texPolymodule}%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb{texFrechet}%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb{texSecondDifferential}%
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Symb{texSecondDifferential}%
   {производная Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Symb{texDifferential}%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Symb{texDifferential}%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction, division ring}%
\Symb{texSecondDifferential}%
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Symb{texSecondDifferential}%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb{texSecondDifferential}%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb{texSecondDifferential}%
   {производная Гато второго порядка отображения $\Vector f$}%
   {Gateaux derivative of Second Order, D vector space}%
\Symb{texDifferential}%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, division ring}%
\Symb{texDifferential}%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb{texSecondDifferential}%
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Symb{texDifferential}%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Symb{texSecondDifferential}%
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Symb{texDifferential}%
   {дифференциал Гато второго порядка отображения $f$ тела}%
   {Gateaux differential of Second Order, division ring}%
\Symb{texSecondDifferential}%
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Symb{texDifferential}%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb{texSecondDifferential}%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb{texSecondDifferential}%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 1, D vector space}%
\Symb{texSecondDifferential}%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 2, D vector space}%
\Symb{texSecondDifferential}%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 3, D vector space}%
\Symb{texSecondDifferential}%
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Symb{texSecondDifferential}%
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Symb{texSecondDifferential}%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 1, D vector space}%
\Symb{texSecondDifferential}%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 2, D vector space}%
\Symb{texSecondDifferential}%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 3, D vector space}%
\Symb{texDifferential}%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb{texVectorSpace}%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace D}%
\Symb{texAffine}%
   {производная}%
   {overline D}%
\Symb{texRefernceFrame}%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb{texVectorSpace}%
   {\drc векторное пространство \sups строк}%
   {r rows drc vector space}%
\Symb{texTidal}%
   {скорость отклонения}%
   {speed of deviation}%
\Symb{texDifferential}%
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Symb{texTensorProduct}%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb{texTensorProduct}%
   {тензорное произведение колец}%
   {tensor product of rings}%
\Symb{texVectorSpace}%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E 0
\Symb{texAffineSpace}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texAffineSpace}%
   {базис}%
   {basis}%
\Symb{texBasis}%
   {базис векторного пространства}%
   {Basis e}%
\Symb{texBasis}%
   {базис в векторном пространстве $\mathcal{V}$}%
   {basis in V}%
\Symb{texVectorSpace}%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb{texPolymodule}%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb{texCartesian}%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb{texBasis}%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb{texVectorField}%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb{texRefernceFrame}%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb{texBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texAffineSpace}%
   {евклидово пространство}%
   {En}%
\Symb{texAffineSpace}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texFiberedAlgebra}%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb{texBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texAdditiveMap}%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\mathcal{E}$}%
   {set of starT nonsingular transformations of bundle}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\mathcal{E}$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb{texBasis}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texRefernceFrame}%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb{texRefernceFrame}%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb{texBasis}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F 0
\Symb{texVectorSpace}%
   {координаты базиса в \dcr векторном пространстве \subs строк}%
   {basis coordinates, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {координаты базиса в \drc векторном пространстве \sups строк}%
   {basis coordinates, r rows drc vector space}%
\Symb{texVectorSpace}%
   {базис в \dcr векторном пространстве \subs строк}%
   {basis, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {базис в \drc векторного пространства \sups строк}%
   {basis, r rows drc vector space}%
\Symb{texDiffEq}%
   {центро-аффинный}%
   {Central Affine Basis}%
\Symb{texRingAdditiveMap}%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb{texRingAdditiveMap}%
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Symb{texBundle}%
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Symb{texBundleRelation}%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb{texFiberedAlgebra}%
   {гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb{texCartesian}%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb{texDifferential}%
   {норма отображения $f$  тела}%
   {norm of map, division ring}%
\Symb{texTstarRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%
\Symb{texAffineSpace}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texRefernceFrame}%
   {система отсчёта}%
   {reference frame}%
\Symb{texRefernceFrame}%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb{texRingAdditiveMap}%
   {стандартная компонента аддитивного отображения $f$ над полем $F$}%
   {standard component of additive map, division ring}%
\Symb{texBiadditiveMap}%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb{texRingAdditiveMap}%
   {стандартная компонента линейного отображения $f$ тела}%
   {standard component of linear map, division ring}%
\Symb{texRingAdditiveMap}%
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Symb{texBiadditiveMap}%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb{texTensorProduct}%
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%

\SetIndexSpace%G 0
\Symb{texVectorSpace}%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb{texFiberedMorphism}%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb{texFiberedMorphism}%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb{texLie}%
   {алгебра Ли группы Ли}%
   {g}%
\Symb{texLie}%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb{texAffineSpace}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texLie}%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb{texBasis}%
   {группа гомоморфизмов векторного пространства $\mathcal{V}$}%
   {GV}%
\Symb{texTstarRepresentation}%
   {малая группа элемента $x$}%
   {little group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective covariant starT representation of group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective covariant Tstar representation of group}%
\Symb{texPolymodule}%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb{texVectorSpace}%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb{texTstarRepresentation}%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H 0
\Symb{texBiring}%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%

\SetIndexSpace%I 0
\Symb{texLieRepresentation}%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb{texLinearLie}%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%K 0
\Symb{texAdditiveMap}%
   {ядро аддитивного отображения $D$\Hyph векторного пространства}%
   {kernel of additive map, D vector space}%
\Symb{texAdditiveMap}%
   {ядро аддитивного отображения тела}%
   {kernel of additive map, division ring}%

\SetIndexSpace%L 0
\Symb{texRepresentation}%
   {левый сдвиг}%
   {left shift}%
\Symb{texDiffProperty}%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb{texDiffProperty}%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb{texBundleRelation}%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb{texDifferential}%
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Symb{texBasis}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texLinearMap}%
   {\rcd векторное пространство \drc линейных отображений \drc векторного пространства $\Vector{V}$ в \drc векторное пространство $\Vector{W}$}%
   {set drc linear maps, drc vector space}%
\Symb{texAdditiveMap}%
   {множество линейных отображений $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector{W}$}%
   {set linear maps, D vector space}%
\Symb{texRepresentation}%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb{texLinearMap}%
   {\drc векторное пространство \rcd линейных отображений \rcd векторного пространства $\Vector{V}$ в \rcd векторное пространство $\Vector{W}$}%
   {set rcd linear maps, rcd vector space}%
\Symb{texLinearMap}%
   {множество \sT представлений тела $S$ в аддитивной группе тела $R$}%
   {set sT representations, division ring}%
\Symb{texLinearMap}%
   {множество \Ts представлений тела $S$ в аддитивной группе тела $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M 0
\Symb{texTstarMorphism}%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb{texTstarMorphism}%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb{texTstarMorphism}%
   {множество \Ts преобразований множества $M$}%
   {set of Tstar transformations}%
\Symb{texTstarRepresentation}%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb{texTstarRepresentation}%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb{texTstarRepresentation}%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%O 0
\Symb{texBasis}%
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Symb{texBasis}%
   {геометрический объект}%
   {geometrical object, vector space}%
\Symb{texFiberedGroup}%
   {орбита представления расслоенной группы $\mathcal{G}$}%
   {orbit of representation of fibered group}%
\Symb{texRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P 0
\Symb{texBundle}%
   {расслоение}%
   {bundle}%
\Symb{texFiberedMorphism}%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb{texFiberedMorphism}%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb{texCartesian}%
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R 0
\Symb{texBasis}%
   {активное преобразование}%
   {active transformation}%
\Symb{texAffine}%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb{texVectorSpace}%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in reduced bundle, 2}%
\Symb{texLinearMap}%
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Symb{texAffine}%
   {кривизна}%
   {GLn curvature_overline}%
\Symb{texVectorSpace}%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb{texRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texRepresentation}%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%
\Symb{texLinearMap}%
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%

\SetIndexSpace%S 0
\Symb{texBundleRelation}%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb{texVectorSpace}%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%

\SetIndexSpace%T 0
\Symb{texTstarMorphism}%
   {категория \Ts представлений $\mathfrak{F}$\Hyph алгебры $A$}%
   {category of Tstar representations of F algebra}%
\Symb{texTstarMorphism}%
   {категория \Ts представлений $\mathfrak{F}$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of F algebra from category}%
\Symb{texLie}%
   {касательная плоскость к группе $G$}%
   {TaG}%

\SetIndexSpace%V 0
\Symb{texBasis}%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb{texBasis}%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb{texPolymodule}%
   {прямое произведение $D_i\RCstar$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, drc vector space, 1 n}%
\Symb{texLinearMap}%
   {дуальное пространство к \drc векторному пространству $\Vector V$}%
   {dual space of drc vector space}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb{texVectorSpace}%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb{texVectorSpace}%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb{texVectorSpace}%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb{texTensorProduct}%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb{texTensorProduct}%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb{texBasis}%
   {векторное пространство}%
   {V}%

\SetIndexSpace%W 0
\Symb{texBasis}%
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%

\SetIndexSpace%X 0
\Symb{texRefernceFrame}%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z 0
\Symb{texDivisionRing}%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta 1
\Symb{texTidal}%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb{texRepresentation}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texTstarMorphism}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texBasis}%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb{texBiring}%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma 1
\Symb{texRefernceFrame}%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb{texAffine}%
   {символ Картана}%
   {Cartan symbol}%
\Symb{texAffine}%
   {связность}%
   {conection overline}%
\Symb{texRefernceFrame}%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb{texAffine}%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb{texBundle}%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda 1
\Symb{texLie}%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb{texLie}%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%Omega 1
\Symb{texRefernceFrame}%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi 1
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%

\SetIndexSpace%Fi 2
\Symb{texLie}%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla 2
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi 2
\Symb{texBundleRelation}%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi 2
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb{texPolymodule}%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb{texPolymodule}%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb{texPolymodule}%
   {прямое произведение $D_i\RCstar$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, drc vector space}%
\Symb{texPolymodule}%
   {прямое произведение $D_i\RCstar$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, drc vector space, i 1 n}%
\Symb{texPolymodule}%
   {произведение групп $G_i$, $i\in I$}%
   {product of groups}%
\Symb{texPolymodule}%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb{texPolymodule}%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb{texPolymodule}%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S 2
\Symb{texBundle}%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb{texBundle}%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

